Exclusive ${\pi}^0$ electroproduction at $W>2$ GeV with CLAS

Exclusive neutral-pion electroproduction ($ep\to e^\prime p^\prime \pi^0$) was measured at Jefferson Lab with a 5.75-GeV electron beam and the CLAS detector. Differential cross sections $d^4\sigma/dtdQ^2dx_Bd\phi_\pi$ and structure functions $\sigma_T+\epsilon\sigma_L, \sigma_{TT}$ and $\sigma_{LT}$ as functions of $t$ were obtained over a wide range of $Q^2$ and $x_B$. The data are compared with Regge and handbag theoretical calculations. Analyses in both frameworks find that a large dominance of transverse processes is necessary to explain the experimental results. For the Regge analysis it is found that the inclusion of vector meson rescattering processes is necessary to bring the magnitude of the calculated and measured structure functions into rough agreement. In the handbag framework, there are two independent calculations, both of which appear to roughly explain the magnitude of the structure functions in terms of transversity generalized parton distributions.

==> xs_table_long.tex <==

\section{Cross Section Table}
Differential cross sections for exclusive $\pi^0$  electroproduction 
$d^2\sigma/dtd\phi_\pi (\gamma^*p\to\pi^0p)$ 
at all measured values of $Q^2$,$x_B$,  $t$  and $\phi_\pi$ obtained in with the CLAS spectrometer at Jefferson Lab with electron beam energy  5.75 GeV. The errors on the cross sections in the last column are statistical and systematic, respectively.
\label{xs_table}

\begin{center}
\begin{longtable}{|c|c|c|c|c|}


\multicolumn{5}{c}%
{} \\
\hline
\multicolumn{1}{|c|}{$Q^2$, $GeV^2$} & 
\multicolumn{1}{|c|}{$x_B$} & 
\multicolumn{1}{|c|}{$t$, $GeV^2$} & 
\multicolumn{1}{|c|}{$\phi$, deg} &
\multicolumn{1}{|c|}{$\frac{d^2\sigma}{dt d\phi}$, $nb/GeV^2$}\\
\hline
\endhead

\hline
\endfoot

\hline
\endlastfoot


1.146 & 0.132 & 0.120 & 63 & 59.4 $\pm$ 15.3 $\pm$ 13.0  \\
\hline

1.145 & 0.132 & 0.120 & 81 & 66.4 $\pm$ 8.87 $\pm$ 13.8  \\
\hline

1.144 & 0.132 & 0.120 & 99 & 82.6 $\pm$ 7.63 $\pm$ 5.74  \\
\hline

1.146 & 0.132 & 0.120 & 117 & 84.0 $\pm$ 8.05 $\pm$ 10.3  \\
\hline

1.147 & 0.132 & 0.120 & 135 & 43.0 $\pm$ 5.96 $\pm$ 5.67  \\
\hline

1.147 & 0.132 & 0.119 & 153 & 43.8 $\pm$ 5.27 $\pm$ 6.78  \\
\hline

1.145 & 0.131 & 0.120 & 171 & 49.7 $\pm$ 6.17 $\pm$ 4.18  \\
\hline

1.146 & 0.132 & 0.120 & 189 & 57.4 $\pm$ 7.54 $\pm$ 9.67  \\
\hline

1.148 & 0.132 & 0.119 & 207 & 61.5 $\pm$ 6.21 $\pm$ 5.64  \\
\hline

1.146 & 0.132 & 0.119 & 225 & 44.8 $\pm$ 5.65 $\pm$ 3.08  \\
\hline

1.147 & 0.132 & 0.120 & 243 & 70.0 $\pm$ 8.43 $\pm$ 1.76  \\
\hline

1.146 & 0.132 & 0.120 & 261 & 65.9 $\pm$ 7.19 $\pm$ 5.83  \\
\hline

1.146 & 0.132 & 0.120 & 279 & 59.9 $\pm$ 7.93 $\pm$ 6.32  \\
\hline

1.146 & 0.132 & 0.120 & 297 & 55.2 $\pm$ 14.3 $\pm$ 15.8  \\
\hline

1.149 & 0.132 & 0.175 & 63 & 67.8 $\pm$ 16.0 $\pm$ 25.0  \\
\hline

1.146 & 0.132 & 0.174 & 81 & 54.3 $\pm$ 7.68 $\pm$ 6.80  \\
\hline

1.146 & 0.132 & 0.175 & 99 & 65.4 $\pm$ 6.97 $\pm$ 7.17  \\
\hline

1.145 & 0.132 & 0.175 & 117 & 74.2 $\pm$ 8.14 $\pm$ 4.39  \\
\hline

1.146 & 0.132 & 0.175 & 135 & 62.3 $\pm$ 6.92 $\pm$ 2.20  \\
\hline

1.144 & 0.132 & 0.175 & 153 & 55.2 $\pm$ 5.88 $\pm$ 4.36  \\
\hline

1.149 & 0.132 & 0.174 & 171 & 47.7 $\pm$ 6.49 $\pm$ 2.40  \\
\hline

1.147 & 0.132 & 0.174 & 189 & 37.6 $\pm$ 5.61 $\pm$ 2.39  \\
\hline

1.148 & 0.132 & 0.175 & 207 & 52.2 $\pm$ 5.70 $\pm$ 0.80  \\
\hline

1.145 & 0.132 & 0.174 & 225 & 64.0 $\pm$ 7.16 $\pm$ 6.23  \\
\hline

1.148 & 0.132 & 0.174 & 243 & 54.1 $\pm$ 7.23 $\pm$ 3.71  \\
\hline

1.148 & 0.132 & 0.175 & 261 & 67.3 $\pm$ 7.22 $\pm$ 1.25  \\
\hline

1.150 & 0.132 & 0.174 & 279 & 72.6 $\pm$ 9.23 $\pm$ 7.14  \\
\hline

1.145 & 0.132 & 0.175 & 297 & 55.5 $\pm$ 14.3 $\pm$ 6.82  \\
\hline

1.147 & 0.132 & 0.249 & 45 & 46.6 $\pm$ 19.0 $\pm$ 7.20  \\
\hline

1.146 & 0.132 & 0.248 & 63 & 51.9 $\pm$ 8.02 $\pm$ 2.19  \\
\hline

1.147 & 0.132 & 0.248 & 81 & 53.9 $\pm$ 5.05 $\pm$ 3.80  \\
\hline

1.145 & 0.132 & 0.249 & 99 & 56.4 $\pm$ 4.56 $\pm$ 2.19  \\
\hline

1.145 & 0.132 & 0.248 & 117 & 53.8 $\pm$ 4.82 $\pm$ 0.55  \\
\hline

1.147 & 0.132 & 0.248 & 135 & 50.4 $\pm$ 4.11 $\pm$ 1.77  \\
\hline

1.150 & 0.132 & 0.249 & 153 & 37.4 $\pm$ 3.30 $\pm$ 3.43  \\
\hline

1.146 & 0.132 & 0.247 & 171 & 37.1 $\pm$ 4.05 $\pm$ 5.84  \\
\hline

1.148 & 0.132 & 0.248 & 189 & 33.2 $\pm$ 3.46 $\pm$ 2.15  \\
\hline

1.150 & 0.132 & 0.248 & 207 & 48.8 $\pm$ 3.95 $\pm$ 0.78  \\
\hline

1.148 & 0.132 & 0.248 & 225 & 43.4 $\pm$ 4.03 $\pm$ 4.55  \\
\hline

1.148 & 0.132 & 0.248 & 243 & 56.3 $\pm$ 4.74 $\pm$ 4.18  \\
\hline

1.145 & 0.132 & 0.249 & 261 & 57.6 $\pm$ 4.50 $\pm$ 2.41  \\
\hline

1.148 & 0.132 & 0.248 & 279 & 45.0 $\pm$ 4.91 $\pm$ 2.16  \\
\hline

1.147 & 0.132 & 0.249 & 297 & 54.4 $\pm$ 8.21 $\pm$ 0.56  \\
\hline

1.146 & 0.132 & 0.248 & 315 & 35.6 $\pm$ 13.4 $\pm$ 7.27  \\
\hline

1.148 & 0.132 & 0.349 & 63 & 31.1 $\pm$ 4.81 $\pm$ 3.31  \\
\hline

1.147 & 0.132 & 0.348 & 81 & 37.3 $\pm$ 3.79 $\pm$ 4.09  \\
\hline

1.147 & 0.132 & 0.348 & 99 & 42.7 $\pm$ 3.82 $\pm$ 3.22  \\
\hline

1.147 & 0.132 & 0.348 & 117 & 36.1 $\pm$ 3.96 $\pm$ 1.27  \\
\hline

1.149 & 0.132 & 0.348 & 135 & 36.7 $\pm$ 3.41 $\pm$ 1.10  \\
\hline

1.149 & 0.132 & 0.347 & 153 & 34.5 $\pm$ 3.45 $\pm$ 3.04  \\
\hline

1.150 & 0.132 & 0.347 & 171 & 24.3 $\pm$ 3.37 $\pm$ 3.61  \\
\hline

1.148 & 0.132 & 0.348 & 189 & 29.9 $\pm$ 3.40 $\pm$ 1.33  \\
\hline

1.148 & 0.132 & 0.348 & 207 & 27.2 $\pm$ 2.96 $\pm$ 2.44  \\
\hline

1.148 & 0.132 & 0.348 & 225 & 42.2 $\pm$ 4.36 $\pm$ 2.41  \\
\hline

1.147 & 0.132 & 0.348 & 243 & 40.9 $\pm$ 3.80 $\pm$ 1.18  \\
\hline

1.147 & 0.132 & 0.349 & 261 & 40.5 $\pm$ 3.55 $\pm$ 0.51  \\
\hline

1.146 & 0.132 & 0.349 & 279 & 36.3 $\pm$ 3.96 $\pm$ 1.00  \\
\hline

1.147 & 0.132 & 0.348 & 297 & 30.0 $\pm$ 4.58 $\pm$ 4.09  \\
\hline

1.147 & 0.132 & 0.348 & 315 & 39.1 $\pm$ 9.22 $\pm$ 6.92  \\
\hline

1.150 & 0.132 & 0.492 & 27 & 43.9 $\pm$ 12.7 $\pm$ 9.56  \\
\hline

1.150 & 0.132 & 0.492 & 45 & 22.3 $\pm$ 3.37 $\pm$ 2.91  \\
\hline

1.149 & 0.132 & 0.492 & 63 & 17.8 $\pm$ 2.02 $\pm$ 1.62  \\
\hline

1.149 & 0.132 & 0.493 & 81 & 26.2 $\pm$ 2.01 $\pm$ 1.65  \\
\hline

1.149 & 0.132 & 0.492 & 99 & 24.2 $\pm$ 1.99 $\pm$ 0.79  \\
\hline

1.149 & 0.132 & 0.493 & 117 & 23.8 $\pm$ 2.35 $\pm$ 1.95  \\
\hline

1.150 & 0.132 & 0.493 & 135 & 23.6 $\pm$ 2.09 $\pm$ 2.98  \\
\hline

1.150 & 0.132 & 0.492 & 153 & 20.7 $\pm$ 2.20 $\pm$ 1.54  \\
\hline

1.150 & 0.132 & 0.492 & 171 & 18.5 $\pm$ 2.64 $\pm$ 0.57  \\
\hline

1.149 & 0.132 & 0.493 & 189 & 16.1 $\pm$ 2.03 $\pm$ 0.30  \\
\hline

1.149 & 0.132 & 0.493 & 207 & 18.6 $\pm$ 2.07 $\pm$ 1.67  \\
\hline

1.149 & 0.132 & 0.493 & 225 & 24.7 $\pm$ 2.56 $\pm$ 1.86  \\
\hline

1.150 & 0.132 & 0.494 & 243 & 22.4 $\pm$ 2.01 $\pm$ 2.33  \\
\hline

1.148 & 0.132 & 0.492 & 261 & 23.4 $\pm$ 1.89 $\pm$ 3.12  \\
\hline

1.148 & 0.132 & 0.493 & 279 & 30.3 $\pm$ 2.43 $\pm$ 1.45  \\
\hline

1.149 & 0.132 & 0.491 & 297 & 17.9 $\pm$ 1.98 $\pm$ 2.80  \\
\hline

1.151 & 0.133 & 0.493 & 315 & 18.7 $\pm$ 2.52 $\pm$ 2.82  \\
\hline

1.150 & 0.132 & 0.492 & 333 & 30.5 $\pm$ 10.2 $\pm$ 14.6  \\
\hline

1.151 & 0.132 & 0.770 & 9 & 7.41 $\pm$ 1.38 $\pm$ 4.71  \\
\hline

1.149 & 0.132 & 0.772 & 27 & 11.0 $\pm$ 1.16 $\pm$ 2.40  \\
\hline

1.151 & 0.132 & 0.771 & 45 & 9.03 $\pm$ 0.99 $\pm$ 1.64  \\
\hline

1.150 & 0.132 & 0.770 & 63 & 11.7 $\pm$ 1.01 $\pm$ 1.18  \\
\hline

1.151 & 0.133 & 0.768 & 81 & 13.0 $\pm$ 0.99 $\pm$ 1.25  \\
\hline

1.150 & 0.133 & 0.768 & 99 & 16.8 $\pm$ 1.33 $\pm$ 0.68  \\
\hline

1.151 & 0.132 & 0.770 & 117 & 11.8 $\pm$ 1.43 $\pm$ 1.79  \\
\hline

1.150 & 0.132 & 0.772 & 135 & 10.1 $\pm$ 1.60 $\pm$ 1.82  \\
\hline

1.152 & 0.133 & 0.772 & 153 & 7.61 $\pm$ 1.84 $\pm$ 0.82  \\
\hline

1.149 & 0.132 & 0.772 & 171 & 5.59 $\pm$ 1.98 $\pm$ 0.49  \\
\hline

1.150 & 0.132 & 0.772 & 189 & 8.99 $\pm$ 2.06 $\pm$ 0.73  \\
\hline

1.152 & 0.132 & 0.772 & 207 & 11.3 $\pm$ 2.09 $\pm$ 1.97  \\
\hline

1.151 & 0.132 & 0.769 & 225 & 7.80 $\pm$ 1.62 $\pm$ 0.15  \\
\hline

1.150 & 0.132 & 0.768 & 243 & 12.3 $\pm$ 1.30 $\pm$ 1.10  \\
\hline

1.149 & 0.132 & 0.767 & 261 & 11.1 $\pm$ 1.03 $\pm$ 0.23  \\
\hline

1.153 & 0.133 & 0.770 & 279 & 13.7 $\pm$ 1.19 $\pm$ 0.47  \\
\hline

1.150 & 0.133 & 0.770 & 297 & 10.9 $\pm$ 0.90 $\pm$ 0.65  \\
\hline

1.150 & 0.132 & 0.769 & 315 & 10.8 $\pm$ 0.89 $\pm$ 1.10  \\
\hline

1.151 & 0.133 & 0.770 & 333 & 12.1 $\pm$ 1.28 $\pm$ 1.86  \\
\hline

1.150 & 0.132 & 0.772 & 351 & 11.3 $\pm$ 2.00 $\pm$ 1.41  \\
\hline

1.153 & 0.133 & 1.204 & 9 & 3.11 $\pm$ 0.45 $\pm$ 0.70  \\
\hline

1.154 & 0.133 & 1.208 & 27 & 5.30 $\pm$ 0.58 $\pm$ 1.26  \\
\hline

1.153 & 0.133 & 1.206 & 45 & 7.61 $\pm$ 0.83 $\pm$ 1.07  \\
\hline

1.154 & 0.133 & 1.202 & 63 & 5.88 $\pm$ 0.67 $\pm$ 0.66  \\
\hline

1.155 & 0.133 & 1.199 & 81 & 6.11 $\pm$ 0.80 $\pm$ 0.61  \\
\hline

1.152 & 0.133 & 1.200 & 99 & 6.77 $\pm$ 1.35 $\pm$ 1.06  \\
\hline

1.155 & 0.133 & 1.204 & 117 & 12.7 $\pm$ 3.82 $\pm$ 1.44  \\
\hline

1.152 & 0.133 & 1.203 & 261 & 4.52 $\pm$ 1.10 $\pm$ 0.05  \\
\hline

1.154 & 0.133 & 1.201 & 279 & 6.82 $\pm$ 0.98 $\pm$ 0.49  \\
\hline

1.154 & 0.133 & 1.203 & 297 & 6.42 $\pm$ 0.66 $\pm$ 0.96  \\
\hline

1.154 & 0.133 & 1.207 & 315 & 5.82 $\pm$ 0.55 $\pm$ 0.95  \\
\hline

1.154 & 0.133 & 1.204 & 333 & 4.76 $\pm$ 0.57 $\pm$ 0.88  \\
\hline

1.152 & 0.133 & 1.208 & 351 & 4.03 $\pm$ 0.58 $\pm$ 0.53  \\
\hline

1.157 & 0.134 & 1.709 & 9 & 2.91 $\pm$ 0.44 $\pm$ 0.51  \\
\hline

1.157 & 0.133 & 1.708 & 27 & 2.55 $\pm$ 0.42 $\pm$ 0.10  \\
\hline

1.156 & 0.133 & 1.708 & 45 & 2.98 $\pm$ 0.68 $\pm$ 0.13  \\
\hline

1.159 & 0.133 & 1.706 & 63 & 3.50 $\pm$ 0.97 $\pm$ 0.49  \\
\hline

1.161 & 0.134 & 1.704 & 81 & 8.13 $\pm$ 3.64 $\pm$ 1.38  \\
\hline

1.156 & 0.133 & 1.711 & 171 & 1.74 $\pm$ 0.62 $\pm$ 0.41  \\
\hline

1.157 & 0.133 & 1.713 & 189 & 0.80 $\pm$ 0.33 $\pm$ 0.17  \\
\hline

1.158 & 0.133 & 1.716 & 297 & 3.05 $\pm$ 0.92 $\pm$ 1.06  \\
\hline

1.153 & 0.133 & 1.708 & 315 & 4.52 $\pm$ 0.70 $\pm$ 0.99  \\
\hline

1.158 & 0.133 & 1.704 & 333 & 2.87 $\pm$ 0.51 $\pm$ 0.18  \\
\hline

1.153 & 0.133 & 1.711 & 351 & 1.88 $\pm$ 0.39 $\pm$ 0.38  \\
\hline

1.377 & 0.169 & 0.120 & 27 & 40.2 $\pm$ 11.1 $\pm$ 9.82  \\
\hline

1.374 & 0.168 & 0.120 & 45 & 50.8 $\pm$ 7.84 $\pm$ 9.48  \\
\hline

1.376 & 0.169 & 0.120 & 63 & 65.5 $\pm$ 8.25 $\pm$ 12.3  \\
\hline

1.376 & 0.169 & 0.120 & 81 & 71.3 $\pm$ 7.16 $\pm$ 8.22  \\
\hline

1.376 & 0.169 & 0.120 & 99 & 73.9 $\pm$ 6.54 $\pm$ 4.55  \\
\hline

1.373 & 0.168 & 0.120 & 117 & 73.3 $\pm$ 7.60 $\pm$ 6.74  \\
\hline

1.377 & 0.169 & 0.120 & 135 & 66.0 $\pm$ 8.01 $\pm$ 6.91  \\
\hline

1.375 & 0.169 & 0.120 & 153 & 52.1 $\pm$ 5.97 $\pm$ 1.79  \\
\hline

1.376 & 0.169 & 0.120 & 171 & 44.2 $\pm$ 6.67 $\pm$ 5.89  \\
\hline

1.376 & 0.169 & 0.119 & 189 & 36.6 $\pm$ 5.78 $\pm$ 4.90  \\
\hline

1.376 & 0.169 & 0.119 & 207 & 43.7 $\pm$ 5.55 $\pm$ 4.47  \\
\hline

1.376 & 0.169 & 0.119 & 225 & 43.3 $\pm$ 6.18 $\pm$ 5.72  \\
\hline

1.376 & 0.169 & 0.119 & 243 & 63.9 $\pm$ 7.80 $\pm$ 7.23  \\
\hline

1.378 & 0.169 & 0.120 & 261 & 60.5 $\pm$ 6.08 $\pm$ 7.03  \\
\hline

1.377 & 0.169 & 0.120 & 279 & 66.0 $\pm$ 6.85 $\pm$ 1.43  \\
\hline

1.376 & 0.169 & 0.120 & 297 & 74.8 $\pm$ 9.00 $\pm$ 3.29  \\
\hline

1.376 & 0.169 & 0.120 & 315 & 61.1 $\pm$ 9.22 $\pm$ 9.05  \\
\hline

1.377 & 0.169 & 0.120 & 333 & 92.9 $\pm$ 16.4 $\pm$ 30.2  \\
\hline

1.377 & 0.169 & 0.175 & 27 & 36.6 $\pm$ 14.9 $\pm$ 0.51  \\
\hline

1.376 & 0.169 & 0.175 & 45 & 57.4 $\pm$ 9.84 $\pm$ 4.64  \\
\hline

1.373 & 0.169 & 0.174 & 63 & 56.5 $\pm$ 7.91 $\pm$ 9.06  \\
\hline

1.376 & 0.169 & 0.175 & 81 & 81.2 $\pm$ 7.38 $\pm$ 7.99  \\
\hline

1.376 & 0.169 & 0.174 & 99 & 83.2 $\pm$ 6.91 $\pm$ 6.81  \\
\hline

1.376 & 0.169 & 0.175 & 117 & 73.4 $\pm$ 7.87 $\pm$ 1.29  \\
\hline

1.377 & 0.169 & 0.175 & 135 & 63.7 $\pm$ 7.30 $\pm$ 7.64  \\
\hline

1.377 & 0.169 & 0.175 & 153 & 44.1 $\pm$ 5.79 $\pm$ 9.60  \\
\hline

1.377 & 0.169 & 0.174 & 171 & 45.0 $\pm$ 7.03 $\pm$ 1.47  \\
\hline

1.378 & 0.169 & 0.175 & 189 & 38.0 $\pm$ 5.93 $\pm$ 6.94  \\
\hline

1.375 & 0.169 & 0.175 & 207 & 59.5 $\pm$ 6.65 $\pm$ 9.98  \\
\hline

1.375 & 0.169 & 0.175 & 225 & 54.4 $\pm$ 7.15 $\pm$ 12.0  \\
\hline

1.378 & 0.169 & 0.175 & 243 & 50.2 $\pm$ 6.38 $\pm$ 5.03  \\
\hline

1.377 & 0.169 & 0.174 & 261 & 71.7 $\pm$ 6.52 $\pm$ 8.32  \\
\hline

1.375 & 0.169 & 0.175 & 279 & 76.8 $\pm$ 7.39 $\pm$ 8.51  \\
\hline

1.378 & 0.169 & 0.175 & 297 & 77.0 $\pm$ 9.01 $\pm$ 4.88  \\
\hline

1.376 & 0.169 & 0.174 & 315 & 68.7 $\pm$ 10.9 $\pm$ 3.86  \\
\hline

1.377 & 0.169 & 0.175 & 333 & 43.8 $\pm$ 19.6 $\pm$ 14.6  \\
\hline

1.375 & 0.169 & 0.248 & 45 & 50.6 $\pm$ 7.46 $\pm$ 5.02  \\
\hline

1.378 & 0.169 & 0.248 & 63 & 55.5 $\pm$ 5.29 $\pm$ 5.30  \\
\hline

1.376 & 0.169 & 0.248 & 81 & 69.4 $\pm$ 4.50 $\pm$ 4.51  \\
\hline

1.375 & 0.169 & 0.249 & 99 & 65.0 $\pm$ 4.24 $\pm$ 4.67  \\
\hline

1.376 & 0.169 & 0.249 & 117 & 68.1 $\pm$ 5.37 $\pm$ 3.21  \\
\hline

1.378 & 0.169 & 0.248 & 135 & 55.2 $\pm$ 4.42 $\pm$ 3.38  \\
\hline

1.376 & 0.169 & 0.248 & 153 & 45.5 $\pm$ 4.28 $\pm$ 3.14  \\
\hline

1.378 & 0.169 & 0.248 & 171 & 32.2 $\pm$ 4.42 $\pm$ 3.52  \\
\hline

1.376 & 0.169 & 0.248 & 189 & 34.0 $\pm$ 4.04 $\pm$ 1.13  \\
\hline

1.378 & 0.169 & 0.248 & 207 & 41.3 $\pm$ 4.05 $\pm$ 1.66  \\
\hline

1.379 & 0.169 & 0.248 & 225 & 49.4 $\pm$ 4.75 $\pm$ 2.50  \\
\hline

1.375 & 0.169 & 0.249 & 243 & 57.4 $\pm$ 4.43 $\pm$ 1.69  \\
\hline

1.374 & 0.169 & 0.249 & 261 & 57.8 $\pm$ 4.02 $\pm$ 5.46  \\
\hline

1.376 & 0.169 & 0.249 & 279 & 71.3 $\pm$ 4.98 $\pm$ 3.97  \\
\hline

1.377 & 0.169 & 0.248 & 297 & 60.3 $\pm$ 5.27 $\pm$ 2.33  \\
\hline

1.376 & 0.169 & 0.248 & 315 & 69.9 $\pm$ 7.86 $\pm$ 12.1  \\
\hline

1.376 & 0.169 & 0.349 & 45 & 35.6 $\pm$ 5.70 $\pm$ 9.62  \\
\hline

1.375 & 0.169 & 0.349 & 63 & 45.9 $\pm$ 4.32 $\pm$ 3.37  \\
\hline

1.375 & 0.169 & 0.349 & 81 & 51.5 $\pm$ 3.75 $\pm$ 3.88  \\
\hline

1.378 & 0.169 & 0.349 & 99 & 49.8 $\pm$ 3.88 $\pm$ 2.66  \\
\hline

1.375 & 0.169 & 0.349 & 117 & 47.6 $\pm$ 4.63 $\pm$ 1.79  \\
\hline

1.378 & 0.169 & 0.349 & 135 & 38.9 $\pm$ 4.12 $\pm$ 1.19  \\
\hline

1.377 & 0.169 & 0.348 & 153 & 24.6 $\pm$ 3.62 $\pm$ 1.68  \\
\hline

1.376 & 0.169 & 0.347 & 171 & 35.9 $\pm$ 5.83 $\pm$ 7.86  \\
\hline

1.378 & 0.169 & 0.348 & 189 & 29.3 $\pm$ 4.58 $\pm$ 3.82  \\
\hline

1.377 & 0.169 & 0.349 & 207 & 34.4 $\pm$ 4.27 $\pm$ 2.76  \\
\hline

1.378 & 0.169 & 0.349 & 225 & 34.8 $\pm$ 4.38 $\pm$ 2.23  \\
\hline

1.376 & 0.169 & 0.349 & 243 & 43.1 $\pm$ 3.78 $\pm$ 2.75  \\
\hline

1.376 & 0.169 & 0.349 & 261 & 57.9 $\pm$ 4.04 $\pm$ 2.40  \\
\hline

1.378 & 0.169 & 0.349 & 279 & 46.7 $\pm$ 3.95 $\pm$ 2.26  \\
\hline

1.377 & 0.169 & 0.349 & 297 & 48.2 $\pm$ 4.29 $\pm$ 2.44  \\
\hline

1.376 & 0.169 & 0.349 & 315 & 54.3 $\pm$ 6.27 $\pm$ 2.34  \\
\hline

1.378 & 0.169 & 0.492 & 27 & 21.9 $\pm$ 6.92 $\pm$ 9.97  \\
\hline

1.377 & 0.169 & 0.494 & 45 & 20.1 $\pm$ 2.40 $\pm$ 2.26  \\
\hline

1.377 & 0.169 & 0.495 & 63 & 29.9 $\pm$ 2.28 $\pm$ 3.21  \\
\hline

1.376 & 0.169 & 0.494 & 81 & 35.4 $\pm$ 2.18 $\pm$ 2.27  \\
\hline

1.377 & 0.169 & 0.494 & 99 & 35.5 $\pm$ 2.46 $\pm$ 4.00  \\
\hline

1.378 & 0.169 & 0.494 & 117 & 35.6 $\pm$ 3.27 $\pm$ 3.55  \\
\hline

1.378 & 0.169 & 0.493 & 135 & 25.6 $\pm$ 3.00 $\pm$ 1.85  \\
\hline

1.378 & 0.169 & 0.494 & 153 & 28.9 $\pm$ 4.08 $\pm$ 3.65  \\
\hline

1.377 & 0.169 & 0.494 & 171 & 21.5 $\pm$ 4.07 $\pm$ 0.27  \\
\hline

1.378 & 0.169 & 0.492 & 189 & 22.9 $\pm$ 3.76 $\pm$ 2.39  \\
\hline

1.379 & 0.169 & 0.492 & 207 & 23.6 $\pm$ 3.41 $\pm$ 1.99  \\
\hline

1.377 & 0.169 & 0.494 & 225 & 26.1 $\pm$ 3.46 $\pm$ 1.89  \\
\hline

1.378 & 0.169 & 0.493 & 243 & 31.9 $\pm$ 2.74 $\pm$ 1.45  \\
\hline

1.378 & 0.169 & 0.494 & 261 & 32.8 $\pm$ 2.25 $\pm$ 0.99  \\
\hline

1.378 & 0.169 & 0.494 & 279 & 31.2 $\pm$ 2.33 $\pm$ 2.17  \\
\hline

1.377 & 0.169 & 0.495 & 297 & 29.5 $\pm$ 2.11 $\pm$ 4.18  \\
\hline

1.378 & 0.169 & 0.494 & 315 & 26.9 $\pm$ 2.31 $\pm$ 2.24  \\
\hline

1.377 & 0.169 & 0.492 & 333 & 32.0 $\pm$ 8.87 $\pm$ 5.59  \\
\hline

1.379 & 0.170 & 0.775 & 9 & 20.0 $\pm$ 3.85 $\pm$ 8.43  \\
\hline

1.379 & 0.170 & 0.771 & 27 & 12.6 $\pm$ 1.36 $\pm$ 1.56  \\
\hline

1.379 & 0.170 & 0.770 & 45 & 14.4 $\pm$ 1.16 $\pm$ 1.80  \\
\hline

1.379 & 0.170 & 0.771 & 63 & 14.1 $\pm$ 1.05 $\pm$ 2.03  \\
\hline

1.378 & 0.170 & 0.771 & 81 & 18.2 $\pm$ 1.20 $\pm$ 0.58  \\
\hline

1.378 & 0.170 & 0.771 & 99 & 16.3 $\pm$ 1.56 $\pm$ 1.38  \\
\hline

1.378 & 0.169 & 0.770 & 117 & 14.0 $\pm$ 2.21 $\pm$ 1.02  \\
\hline

1.379 & 0.169 & 0.775 & 135 & 13.3 $\pm$ 3.14 $\pm$ 0.17  \\
\hline

1.378 & 0.169 & 0.773 & 153 & 16.3 $\pm$ 4.71 $\pm$ 5.12  \\
\hline

1.378 & 0.169 & 0.774 & 189 & 19.1 $\pm$ 4.49 $\pm$ 1.32  \\
\hline

1.378 & 0.169 & 0.775 & 207 & 5.13 $\pm$ 1.94 $\pm$ 1.07  \\
\hline

1.379 & 0.169 & 0.774 & 225 & 24.6 $\pm$ 4.73 $\pm$ 3.23  \\
\hline

1.379 & 0.170 & 0.773 & 243 & 12.7 $\pm$ 2.03 $\pm$ 0.40  \\
\hline

1.379 & 0.170 & 0.771 & 261 & 15.2 $\pm$ 1.47 $\pm$ 1.26  \\
\hline

1.379 & 0.170 & 0.773 & 279 & 17.7 $\pm$ 1.35 $\pm$ 0.76  \\
\hline

1.379 & 0.170 & 0.773 & 297 & 17.8 $\pm$ 1.08 $\pm$ 1.14  \\
\hline

1.379 & 0.170 & 0.773 & 315 & 13.6 $\pm$ 0.94 $\pm$ 2.15  \\
\hline

1.378 & 0.170 & 0.770 & 333 & 12.4 $\pm$ 1.39 $\pm$ 2.01  \\
\hline

1.379 & 0.169 & 0.774 & 351 & 17.4 $\pm$ 4.22 $\pm$ 6.25  \\
\hline

1.379 & 0.170 & 1.213 & 9 & 3.78 $\pm$ 0.50 $\pm$ 0.81  \\
\hline

1.381 & 0.170 & 1.209 & 27 & 6.12 $\pm$ 0.61 $\pm$ 1.11  \\
\hline

1.380 & 0.170 & 1.209 & 45 & 6.24 $\pm$ 0.68 $\pm$ 0.58  \\
\hline

1.381 & 0.170 & 1.206 & 63 & 8.52 $\pm$ 0.84 $\pm$ 0.51  \\
\hline

1.380 & 0.170 & 1.207 & 81 & 10.1 $\pm$ 1.25 $\pm$ 0.12  \\
\hline

1.380 & 0.170 & 1.209 & 99 & 9.53 $\pm$ 2.19 $\pm$ 1.15  \\
\hline

1.381 & 0.170 & 1.212 & 153 & 13.4 $\pm$ 5.47 $\pm$ 0.80  \\
\hline

1.380 & 0.169 & 1.207 & 171 & 2.45 $\pm$ 0.87 $\pm$ 0.53  \\
\hline

1.382 & 0.170 & 1.210 & 189 & 2.80 $\pm$ 0.70 $\pm$ 0.68  \\
\hline

1.380 & 0.169 & 1.212 & 207 & 4.89 $\pm$ 1.36 $\pm$ 0.68  \\
\hline

1.380 & 0.170 & 1.206 & 261 & 9.17 $\pm$ 2.37 $\pm$ 2.27  \\
\hline

1.380 & 0.170 & 1.210 & 279 & 8.75 $\pm$ 1.32 $\pm$ 1.14  \\
\hline

1.380 & 0.170 & 1.204 & 297 & 8.07 $\pm$ 0.73 $\pm$ 0.57  \\
\hline

1.380 & 0.170 & 1.206 & 315 & 6.40 $\pm$ 0.57 $\pm$ 0.90  \\
\hline

1.380 & 0.170 & 1.207 & 333 & 5.64 $\pm$ 0.63 $\pm$ 0.48  \\
\hline

1.379 & 0.170 & 1.209 & 351 & 4.70 $\pm$ 0.65 $\pm$ 0.78  \\
\hline

1.382 & 0.171 & 1.710 & 9 & 1.06 $\pm$ 0.24 $\pm$ 0.26  \\
\hline

1.385 & 0.170 & 1.712 & 27 & 3.98 $\pm$ 0.53 $\pm$ 0.41  \\
\hline

1.383 & 0.171 & 1.709 & 45 & 2.28 $\pm$ 0.55 $\pm$ 0.13  \\
\hline

1.384 & 0.171 & 1.705 & 63 & 6.10 $\pm$ 1.76 $\pm$ 4.58  \\
\hline

1.383 & 0.170 & 1.706 & 117 & 1.80 $\pm$ 0.74 $\pm$ 0.58  \\
\hline

1.380 & 0.170 & 1.713 & 135 & 1.72 $\pm$ 0.65 $\pm$ 0.30  \\
\hline

1.382 & 0.170 & 1.714 & 153 & 6.98 $\pm$ 2.47 $\pm$ 0.94  \\
\hline

1.382 & 0.170 & 1.713 & 171 & 1.54 $\pm$ 0.44 $\pm$ 0.42  \\
\hline

1.383 & 0.170 & 1.716 & 189 & 1.66 $\pm$ 0.36 $\pm$ 0.15  \\
\hline

1.382 & 0.170 & 1.710 & 207 & 1.29 $\pm$ 0.43 $\pm$ 0.32  \\
\hline

1.381 & 0.170 & 1.715 & 225 & 3.81 $\pm$ 1.70 $\pm$ 0.96  \\
\hline

1.381 & 0.170 & 1.710 & 243 & 4.21 $\pm$ 1.27 $\pm$ 1.90  \\
\hline

1.383 & 0.170 & 1.705 & 297 & 4.24 $\pm$ 1.41 $\pm$ 1.96  \\
\hline

1.383 & 0.170 & 1.713 & 315 & 2.39 $\pm$ 0.47 $\pm$ 0.38  \\
\hline

1.380 & 0.170 & 1.711 & 333 & 1.98 $\pm$ 0.43 $\pm$ 0.46  \\
\hline

1.381 & 0.170 & 1.710 & 351 & 2.45 $\pm$ 0.40 $\pm$ 0.79  \\
\hline

1.483 & 0.204 & 0.121 & 279 & 165. $\pm$ 74.0 $\pm$ 74.3  \\
\hline

1.483 & 0.204 & 0.119 & 315 & 89.7 $\pm$ 40.2 $\pm$ 67.4  \\
\hline

1.482 & 0.204 & 0.175 & 45 & 129. $\pm$ 58.0 $\pm$ 11.0  \\
\hline

1.482 & 0.203 & 0.177 & 81 & 171. $\pm$ 60.7 $\pm$ 53.3  \\
\hline

1.482 & 0.203 & 0.174 & 99 & 117. $\pm$ 52.6 $\pm$ 14.5  \\
\hline

1.482 & 0.204 & 0.173 & 297 & 137. $\pm$ 61.3 $\pm$ 24.0  \\
\hline

1.482 & 0.204 & 0.245 & 45 & 83.2 $\pm$ 34.0 $\pm$ 43.3  \\
\hline

1.481 & 0.204 & 0.249 & 63 & 61.0 $\pm$ 27.3 $\pm$ 8.49  \\
\hline

1.481 & 0.203 & 0.248 & 81 & 72.9 $\pm$ 27.6 $\pm$ 4.07  \\
\hline

1.482 & 0.203 & 0.248 & 99 & 153. $\pm$ 41.1 $\pm$ 22.9  \\
\hline

1.481 & 0.204 & 0.248 & 243 & 110. $\pm$ 41.6 $\pm$ 10.7  \\
\hline

1.483 & 0.204 & 0.251 & 261 & 105. $\pm$ 37.2 $\pm$ 5.65  \\
\hline

1.481 & 0.204 & 0.248 & 279 & 120. $\pm$ 45.5 $\pm$ 6.90  \\
\hline

1.482 & 0.204 & 0.248 & 297 & 137. $\pm$ 39.7 $\pm$ 7.13  \\
\hline

1.482 & 0.204 & 0.249 & 315 & 96.2 $\pm$ 36.4 $\pm$ 12.2  \\
\hline

1.482 & 0.204 & 0.352 & 81 & 93.4 $\pm$ 35.3 $\pm$ 3.08  \\
\hline

1.483 & 0.204 & 0.349 & 99 & 90.1 $\pm$ 36.8 $\pm$ 7.61  \\
\hline

1.482 & 0.204 & 0.351 & 279 & 79.7 $\pm$ 35.7 $\pm$ 9.73  \\
\hline

1.480 & 0.204 & 0.350 & 315 & 76.7 $\pm$ 31.3 $\pm$ 7.06  \\
\hline

1.481 & 0.204 & 0.496 & 45 & 40.1 $\pm$ 16.4 $\pm$ 1.82  \\
\hline

1.482 & 0.204 & 0.499 & 63 & 33.1 $\pm$ 12.5 $\pm$ 2.38  \\
\hline

1.481 & 0.204 & 0.499 & 81 & 21.5 $\pm$ 9.63 $\pm$ 6.37  \\
\hline

1.481 & 0.203 & 0.497 & 297 & 54.0 $\pm$ 18.0 $\pm$ 29.6  \\
\hline

1.483 & 0.204 & 0.495 & 315 & 50.6 $\pm$ 16.9 $\pm$ 11.4  \\
\hline

1.482 & 0.203 & 0.766 & 45 & 17.0 $\pm$ 7.61 $\pm$ 1.60  \\
\hline

1.481 & 0.204 & 0.767 & 315 & 19.9 $\pm$ 7.06 $\pm$ 2.59  \\
\hline

1.608 & 0.186 & 0.120 & 27 & 82.1 $\pm$ 29.0 $\pm$ 0.84  \\
\hline

1.606 & 0.187 & 0.120 & 45 & 30.9 $\pm$ 9.78 $\pm$ 9.17  \\
\hline

1.606 & 0.186 & 0.120 & 63 & 54.4 $\pm$ 11.1 $\pm$ 8.58  \\
\hline

1.606 & 0.187 & 0.120 & 81 & 58.7 $\pm$ 9.28 $\pm$ 9.67  \\
\hline

1.606 & 0.186 & 0.120 & 99 & 52.9 $\pm$ 7.33 $\pm$ 3.00  \\
\hline

1.606 & 0.186 & 0.120 & 117 & 59.7 $\pm$ 8.90 $\pm$ 5.27  \\
\hline

1.604 & 0.186 & 0.119 & 135 & 38.3 $\pm$ 7.37 $\pm$ 7.35  \\
\hline

1.608 & 0.186 & 0.120 & 153 & 31.1 $\pm$ 5.67 $\pm$ 2.10  \\
\hline

1.605 & 0.186 & 0.120 & 171 & 37.8 $\pm$ 7.15 $\pm$ 9.40  \\
\hline

1.606 & 0.186 & 0.119 & 189 & 31.1 $\pm$ 6.63 $\pm$ 4.81  \\
\hline

1.605 & 0.186 & 0.120 & 207 & 39.5 $\pm$ 6.58 $\pm$ 8.80  \\
\hline

1.605 & 0.186 & 0.119 & 225 & 38.4 $\pm$ 7.25 $\pm$ 5.99  \\
\hline

1.606 & 0.187 & 0.120 & 243 & 43.7 $\pm$ 7.99 $\pm$ 8.25  \\
\hline

1.607 & 0.187 & 0.120 & 261 & 49.8 $\pm$ 8.09 $\pm$ 3.53  \\
\hline

1.607 & 0.187 & 0.120 & 279 & 59.4 $\pm$ 9.05 $\pm$ 5.15  \\
\hline

1.608 & 0.186 & 0.120 & 297 & 67.3 $\pm$ 12.5 $\pm$ 14.4  \\
\hline

1.609 & 0.187 & 0.121 & 315 & 33.8 $\pm$ 9.76 $\pm$ 7.84  \\
\hline

1.603 & 0.186 & 0.119 & 333 & 80.3 $\pm$ 23.2 $\pm$ 17.4  \\
\hline

1.605 & 0.186 & 0.174 & 45 & 46.3 $\pm$ 14.0 $\pm$ 19.5  \\
\hline

1.608 & 0.187 & 0.175 & 63 & 66.2 $\pm$ 11.5 $\pm$ 14.3  \\
\hline

1.606 & 0.187 & 0.174 & 81 & 58.4 $\pm$ 8.35 $\pm$ 10.1  \\
\hline

1.608 & 0.187 & 0.175 & 99 & 54.4 $\pm$ 6.96 $\pm$ 8.47  \\
\hline

1.609 & 0.187 & 0.175 & 117 & 68.3 $\pm$ 9.97 $\pm$ 0.87  \\
\hline

1.606 & 0.186 & 0.175 & 135 & 49.2 $\pm$ 8.44 $\pm$ 11.9  \\
\hline

1.609 & 0.187 & 0.174 & 153 & 52.3 $\pm$ 8.37 $\pm$ 9.82  \\
\hline

1.607 & 0.186 & 0.175 & 171 & 33.2 $\pm$ 7.62 $\pm$ 4.94  \\
\hline

1.608 & 0.187 & 0.175 & 189 & 44.4 $\pm$ 8.11 $\pm$ 4.08  \\
\hline

1.605 & 0.187 & 0.175 & 207 & 52.1 $\pm$ 7.45 $\pm$ 9.77  \\
\hline

1.606 & 0.186 & 0.174 & 225 & 48.7 $\pm$ 8.60 $\pm$ 0.78  \\
\hline

1.609 & 0.187 & 0.175 & 243 & 58.4 $\pm$ 9.12 $\pm$ 3.51  \\
\hline

1.606 & 0.187 & 0.175 & 261 & 63.1 $\pm$ 8.08 $\pm$ 9.10  \\
\hline

1.605 & 0.187 & 0.175 & 279 & 52.9 $\pm$ 8.07 $\pm$ 1.16  \\
\hline

1.608 & 0.187 & 0.175 & 297 & 74.4 $\pm$ 11.8 $\pm$ 15.9  \\
\hline

1.604 & 0.186 & 0.174 & 315 & 74.0 $\pm$ 17.9 $\pm$ 13.2  \\
\hline

1.607 & 0.186 & 0.247 & 45 & 54.0 $\pm$ 11.3 $\pm$ 16.4  \\
\hline

1.609 & 0.187 & 0.249 & 63 & 37.8 $\pm$ 5.34 $\pm$ 9.44  \\
\hline

1.606 & 0.186 & 0.249 & 81 & 54.0 $\pm$ 5.19 $\pm$ 5.79  \\
\hline

1.608 & 0.187 & 0.248 & 99 & 51.2 $\pm$ 4.80 $\pm$ 3.43  \\
\hline

1.605 & 0.186 & 0.248 & 117 & 55.7 $\pm$ 5.90 $\pm$ 5.71  \\
\hline

1.605 & 0.186 & 0.249 & 135 & 41.5 $\pm$ 4.82 $\pm$ 6.15  \\
\hline

1.606 & 0.186 & 0.248 & 153 & 36.1 $\pm$ 4.48 $\pm$ 5.93  \\
\hline

1.607 & 0.187 & 0.248 & 171 & 35.2 $\pm$ 5.49 $\pm$ 0.41  \\
\hline

1.605 & 0.187 & 0.248 & 189 & 37.9 $\pm$ 4.93 $\pm$ 0.39  \\
\hline

1.606 & 0.187 & 0.249 & 207 & 33.0 $\pm$ 4.20 $\pm$ 1.05  \\
\hline

1.605 & 0.186 & 0.248 & 225 & 48.4 $\pm$ 5.44 $\pm$ 5.13  \\
\hline

1.606 & 0.186 & 0.248 & 243 & 54.0 $\pm$ 5.48 $\pm$ 6.04  \\
\hline

1.609 & 0.187 & 0.249 & 261 & 60.4 $\pm$ 5.07 $\pm$ 2.08  \\
\hline

1.604 & 0.186 & 0.247 & 279 & 44.8 $\pm$ 5.11 $\pm$ 3.11  \\
\hline

1.606 & 0.186 & 0.249 & 297 & 56.5 $\pm$ 6.36 $\pm$ 0.83  \\
\hline

1.611 & 0.187 & 0.248 & 315 & 62.7 $\pm$ 10.6 $\pm$ 4.67  \\
\hline

1.610 & 0.187 & 0.350 & 45 & 37.1 $\pm$ 8.30 $\pm$ 3.69  \\
\hline

1.607 & 0.187 & 0.348 & 63 & 39.5 $\pm$ 5.06 $\pm$ 4.65  \\
\hline

1.605 & 0.186 & 0.348 & 81 & 41.3 $\pm$ 4.20 $\pm$ 2.48  \\
\hline

1.607 & 0.187 & 0.350 & 99 & 49.1 $\pm$ 4.73 $\pm$ 0.56  \\
\hline

1.606 & 0.187 & 0.349 & 117 & 34.0 $\pm$ 4.54 $\pm$ 5.07  \\
\hline

1.606 & 0.187 & 0.348 & 135 & 45.6 $\pm$ 5.16 $\pm$ 6.93  \\
\hline

1.609 & 0.187 & 0.348 & 153 & 32.7 $\pm$ 4.58 $\pm$ 1.39  \\
\hline

1.608 & 0.187 & 0.347 & 171 & 27.7 $\pm$ 5.05 $\pm$ 2.35  \\
\hline

1.607 & 0.187 & 0.348 & 189 & 39.7 $\pm$ 5.45 $\pm$ 3.09  \\
\hline

1.607 & 0.187 & 0.347 & 207 & 29.8 $\pm$ 4.22 $\pm$ 0.38  \\
\hline

1.607 & 0.187 & 0.349 & 225 & 28.0 $\pm$ 4.22 $\pm$ 0.60  \\
\hline

1.606 & 0.187 & 0.350 & 243 & 45.2 $\pm$ 4.84 $\pm$ 5.01  \\
\hline

1.609 & 0.187 & 0.349 & 261 & 48.6 $\pm$ 4.70 $\pm$ 3.32  \\
\hline

1.607 & 0.186 & 0.349 & 279 & 46.7 $\pm$ 4.92 $\pm$ 1.30  \\
\hline

1.610 & 0.187 & 0.348 & 297 & 32.2 $\pm$ 4.19 $\pm$ 0.75  \\
\hline

1.608 & 0.187 & 0.349 & 315 & 42.4 $\pm$ 7.74 $\pm$ 2.10  \\
\hline

1.608 & 0.187 & 0.493 & 45 & 28.2 $\pm$ 3.83 $\pm$ 8.14  \\
\hline

1.605 & 0.187 & 0.494 & 63 & 26.7 $\pm$ 2.72 $\pm$ 2.79  \\
\hline

1.607 & 0.187 & 0.495 & 81 & 29.7 $\pm$ 2.50 $\pm$ 2.21  \\
\hline

1.608 & 0.187 & 0.495 & 99 & 29.7 $\pm$ 2.73 $\pm$ 1.15  \\
\hline

1.608 & 0.187 & 0.495 & 117 & 27.5 $\pm$ 2.97 $\pm$ 3.58  \\
\hline

1.607 & 0.187 & 0.492 & 135 & 19.7 $\pm$ 2.57 $\pm$ 1.88  \\
\hline

1.608 & 0.187 & 0.494 & 153 & 20.7 $\pm$ 3.06 $\pm$ 0.39  \\
\hline

1.607 & 0.187 & 0.493 & 171 & 21.6 $\pm$ 3.81 $\pm$ 1.59  \\
\hline

1.608 & 0.187 & 0.494 & 189 & 19.3 $\pm$ 3.12 $\pm$ 1.98  \\
\hline

1.608 & 0.187 & 0.494 & 207 & 20.4 $\pm$ 2.94 $\pm$ 4.62  \\
\hline

1.607 & 0.187 & 0.493 & 225 & 26.5 $\pm$ 3.29 $\pm$ 0.76  \\
\hline

1.608 & 0.187 & 0.494 & 243 & 23.0 $\pm$ 2.56 $\pm$ 1.81  \\
\hline

1.607 & 0.187 & 0.494 & 261 & 29.9 $\pm$ 2.64 $\pm$ 2.23  \\
\hline

1.607 & 0.187 & 0.493 & 279 & 29.6 $\pm$ 2.65 $\pm$ 1.98  \\
\hline

1.607 & 0.187 & 0.494 & 297 & 27.4 $\pm$ 2.57 $\pm$ 2.34  \\
\hline

1.606 & 0.187 & 0.494 & 315 & 29.6 $\pm$ 3.26 $\pm$ 3.91  \\
\hline

1.608 & 0.187 & 0.773 & 9 & 17.4 $\pm$ 6.15 $\pm$ 3.25  \\
\hline

1.607 & 0.187 & 0.774 & 27 & 12.5 $\pm$ 1.90 $\pm$ 2.09  \\
\hline

1.608 & 0.187 & 0.774 & 45 & 14.7 $\pm$ 1.43 $\pm$ 1.62  \\
\hline

1.605 & 0.187 & 0.773 & 63 & 12.3 $\pm$ 1.26 $\pm$ 1.89  \\
\hline

1.608 & 0.187 & 0.775 & 81 & 16.9 $\pm$ 1.38 $\pm$ 0.44  \\
\hline

1.608 & 0.187 & 0.775 & 99 & 17.3 $\pm$ 1.71 $\pm$ 0.66  \\
\hline

1.606 & 0.187 & 0.776 & 117 & 13.4 $\pm$ 1.95 $\pm$ 1.45  \\
\hline

1.608 & 0.187 & 0.774 & 135 & 12.9 $\pm$ 2.44 $\pm$ 1.60  \\
\hline

1.609 & 0.187 & 0.776 & 153 & 12.7 $\pm$ 3.40 $\pm$ 1.71  \\
\hline

1.608 & 0.187 & 0.775 & 171 & 11.7 $\pm$ 4.43 $\pm$ 2.24  \\
\hline

1.610 & 0.187 & 0.773 & 189 & 5.50 $\pm$ 2.46 $\pm$ 0.18  \\
\hline

1.609 & 0.187 & 0.774 & 207 & 13.0 $\pm$ 3.36 $\pm$ 3.72  \\
\hline

1.609 & 0.187 & 0.774 & 225 & 15.9 $\pm$ 3.07 $\pm$ 0.66  \\
\hline

1.608 & 0.187 & 0.774 & 243 & 14.1 $\pm$ 1.81 $\pm$ 0.69  \\
\hline

1.608 & 0.187 & 0.776 & 261 & 14.8 $\pm$ 1.50 $\pm$ 0.95  \\
\hline

1.606 & 0.187 & 0.773 & 279 & 13.2 $\pm$ 1.32 $\pm$ 1.06  \\
\hline

1.607 & 0.187 & 0.775 & 297 & 13.7 $\pm$ 1.17 $\pm$ 1.11  \\
\hline

1.608 & 0.187 & 0.774 & 315 & 14.0 $\pm$ 1.21 $\pm$ 1.61  \\
\hline

1.605 & 0.186 & 0.772 & 333 & 13.4 $\pm$ 2.09 $\pm$ 2.90  \\
\hline

1.608 & 0.187 & 0.774 & 351 & 31.7 $\pm$ 8.19 $\pm$ 8.30  \\
\hline

1.609 & 0.187 & 1.208 & 9 & 5.06 $\pm$ 0.75 $\pm$ 1.12  \\
\hline

1.606 & 0.187 & 1.209 & 27 & 5.40 $\pm$ 0.74 $\pm$ 0.41  \\
\hline

1.609 & 0.187 & 1.209 & 45 & 5.85 $\pm$ 0.79 $\pm$ 0.29  \\
\hline

1.607 & 0.187 & 1.210 & 63 & 7.07 $\pm$ 0.87 $\pm$ 1.00  \\
\hline

1.610 & 0.187 & 1.210 & 81 & 7.77 $\pm$ 1.05 $\pm$ 0.12  \\
\hline

1.607 & 0.187 & 1.209 & 99 & 7.83 $\pm$ 1.90 $\pm$ 0.19  \\
\hline

1.608 & 0.187 & 1.214 & 171 & 4.26 $\pm$ 1.90 $\pm$ 0.25  \\
\hline

1.611 & 0.187 & 1.218 & 189 & 4.33 $\pm$ 1.37 $\pm$ 0.44  \\
\hline

1.609 & 0.187 & 1.211 & 207 & 7.82 $\pm$ 2.61 $\pm$ 1.75  \\
\hline

1.607 & 0.187 & 1.212 & 243 & 12.4 $\pm$ 5.07 $\pm$ 2.93  \\
\hline

1.608 & 0.187 & 1.208 & 261 & 3.18 $\pm$ 1.12 $\pm$ 0.24  \\
\hline

1.610 & 0.187 & 1.210 & 279 & 5.96 $\pm$ 1.07 $\pm$ 0.92  \\
\hline

1.608 & 0.187 & 1.210 & 297 & 7.20 $\pm$ 0.84 $\pm$ 0.61  \\
\hline

1.607 & 0.187 & 1.208 & 315 & 5.23 $\pm$ 0.64 $\pm$ 0.67  \\
\hline

1.608 & 0.187 & 1.214 & 333 & 5.37 $\pm$ 0.77 $\pm$ 0.96  \\
\hline

1.608 & 0.187 & 1.214 & 351 & 2.55 $\pm$ 0.59 $\pm$ 0.51  \\
\hline

1.609 & 0.187 & 1.716 & 9 & 2.06 $\pm$ 0.41 $\pm$ 0.09  \\
\hline

1.607 & 0.187 & 1.713 & 27 & 2.83 $\pm$ 0.50 $\pm$ 0.31  \\
\hline

1.608 & 0.187 & 1.714 & 45 & 3.01 $\pm$ 0.67 $\pm$ 0.32  \\
\hline

1.610 & 0.187 & 1.710 & 63 & 3.71 $\pm$ 1.07 $\pm$ 0.47  \\
\hline

1.611 & 0.188 & 1.710 & 117 & 5.24 $\pm$ 1.98 $\pm$ 0.71  \\
\hline

1.612 & 0.187 & 1.710 & 189 & 1.42 $\pm$ 0.50 $\pm$ 0.66  \\
\hline

1.608 & 0.187 & 1.712 & 243 & 3.99 $\pm$ 1.79 $\pm$ 0.87  \\
\hline

1.612 & 0.187 & 1.713 & 297 & 1.88 $\pm$ 0.77 $\pm$ 0.30  \\
\hline

1.612 & 0.188 & 1.716 & 315 & 2.61 $\pm$ 0.57 $\pm$ 0.48  \\
\hline

1.609 & 0.188 & 1.716 & 333 & 2.83 $\pm$ 0.56 $\pm$ 0.26  \\
\hline

1.613 & 0.187 & 1.715 & 351 & 2.10 $\pm$ 0.51 $\pm$ 0.25  \\
\hline

1.748 & 0.223 & 0.121 & 9 & 42.6 $\pm$ 6.91 $\pm$ 2.10  \\
\hline

1.740 & 0.223 & 0.120 & 27 & 47.9 $\pm$ 5.54 $\pm$ 8.25  \\
\hline

1.742 & 0.223 & 0.120 & 45 & 55.3 $\pm$ 5.70 $\pm$ 13.3  \\
\hline

1.745 & 0.223 & 0.120 & 63 & 51.7 $\pm$ 5.78 $\pm$ 11.1  \\
\hline

1.743 & 0.223 & 0.120 & 81 & 51.4 $\pm$ 5.22 $\pm$ 0.81  \\
\hline

1.743 & 0.223 & 0.120 & 99 & 54.0 $\pm$ 4.57 $\pm$ 7.36  \\
\hline

1.745 & 0.223 & 0.120 & 117 & 47.1 $\pm$ 4.78 $\pm$ 7.74  \\
\hline

1.741 & 0.223 & 0.119 & 135 & 51.3 $\pm$ 6.01 $\pm$ 5.00  \\
\hline

1.745 & 0.223 & 0.120 & 153 & 43.2 $\pm$ 5.05 $\pm$ 1.62  \\
\hline

1.746 & 0.223 & 0.120 & 171 & 52.4 $\pm$ 7.49 $\pm$ 6.78  \\
\hline

1.743 & 0.223 & 0.120 & 189 & 29.7 $\pm$ 5.83 $\pm$ 3.92  \\
\hline

1.746 & 0.223 & 0.120 & 207 & 35.3 $\pm$ 4.94 $\pm$ 1.84  \\
\hline

1.741 & 0.223 & 0.120 & 225 & 56.0 $\pm$ 7.05 $\pm$ 4.43  \\
\hline

1.742 & 0.223 & 0.120 & 243 & 40.9 $\pm$ 4.70 $\pm$ 3.22  \\
\hline

1.742 & 0.223 & 0.120 & 261 & 53.0 $\pm$ 4.90 $\pm$ 5.36  \\
\hline

1.745 & 0.223 & 0.120 & 279 & 46.3 $\pm$ 5.45 $\pm$ 3.95  \\
\hline

1.741 & 0.223 & 0.120 & 297 & 54.6 $\pm$ 6.30 $\pm$ 9.23  \\
\hline

1.741 & 0.223 & 0.120 & 315 & 49.1 $\pm$ 5.12 $\pm$ 8.34  \\
\hline

1.746 & 0.223 & 0.120 & 333 & 45.4 $\pm$ 5.43 $\pm$ 4.67  \\
\hline

1.745 & 0.223 & 0.120 & 351 & 39.3 $\pm$ 6.55 $\pm$ 7.97  \\
\hline

1.745 & 0.223 & 0.175 & 9 & 55.8 $\pm$ 9.04 $\pm$ 12.0  \\
\hline

1.746 & 0.223 & 0.175 & 27 & 45.5 $\pm$ 6.08 $\pm$ 0.68  \\
\hline

1.741 & 0.223 & 0.175 & 45 & 56.7 $\pm$ 5.88 $\pm$ 5.99  \\
\hline

1.743 & 0.223 & 0.175 & 63 & 62.0 $\pm$ 6.32 $\pm$ 6.62  \\
\hline

1.745 & 0.223 & 0.175 & 81 & 70.8 $\pm$ 6.07 $\pm$ 11.1  \\
\hline

1.742 & 0.223 & 0.174 & 99 & 85.2 $\pm$ 6.51 $\pm$ 7.03  \\
\hline

1.744 & 0.223 & 0.175 & 117 & 61.7 $\pm$ 6.36 $\pm$ 5.78  \\
\hline

1.742 & 0.223 & 0.175 & 135 & 41.2 $\pm$ 5.95 $\pm$ 4.58  \\
\hline

1.749 & 0.223 & 0.175 & 153 & 35.7 $\pm$ 5.51 $\pm$ 3.62  \\
\hline

1.746 & 0.223 & 0.175 & 171 & 44.8 $\pm$ 7.80 $\pm$ 0.50  \\
\hline

1.741 & 0.223 & 0.174 & 189 & 30.8 $\pm$ 5.94 $\pm$ 3.56  \\
\hline

1.742 & 0.223 & 0.175 & 207 & 41.0 $\pm$ 5.86 $\pm$ 5.65  \\
\hline

1.745 & 0.223 & 0.175 & 225 & 42.9 $\pm$ 6.46 $\pm$ 2.84  \\
\hline

1.742 & 0.223 & 0.175 & 243 & 51.8 $\pm$ 5.76 $\pm$ 8.76  \\
\hline

1.741 & 0.223 & 0.175 & 261 & 69.2 $\pm$ 6.00 $\pm$ 2.36  \\
\hline

1.742 & 0.223 & 0.174 & 279 & 82.3 $\pm$ 7.30 $\pm$ 3.57  \\
\hline

1.743 & 0.223 & 0.175 & 297 & 77.5 $\pm$ 7.07 $\pm$ 4.17  \\
\hline

1.743 & 0.223 & 0.175 & 315 & 57.8 $\pm$ 5.51 $\pm$ 9.82  \\
\hline

1.743 & 0.223 & 0.175 & 333 & 48.7 $\pm$ 6.18 $\pm$ 4.43  \\
\hline

1.743 & 0.223 & 0.175 & 351 & 37.3 $\pm$ 7.78 $\pm$ 8.22  \\
\hline

1.746 & 0.223 & 0.248 & 9 & 23.0 $\pm$ 6.39 $\pm$ 4.75  \\
\hline

1.745 & 0.224 & 0.249 & 27 & 45.5 $\pm$ 5.09 $\pm$ 8.48  \\
\hline

1.745 & 0.223 & 0.249 & 45 & 49.2 $\pm$ 3.96 $\pm$ 3.07  \\
\hline

1.744 & 0.223 & 0.248 & 63 & 75.5 $\pm$ 4.59 $\pm$ 8.16  \\
\hline

1.743 & 0.223 & 0.248 & 81 & 72.1 $\pm$ 3.90 $\pm$ 3.85  \\
\hline

1.743 & 0.223 & 0.249 & 99 & 63.9 $\pm$ 3.79 $\pm$ 2.79  \\
\hline

1.745 & 0.223 & 0.248 & 117 & 53.0 $\pm$ 4.63 $\pm$ 3.91  \\
\hline

1.744 & 0.223 & 0.249 & 135 & 41.7 $\pm$ 4.66 $\pm$ 0.60  \\
\hline

1.746 & 0.223 & 0.249 & 153 & 34.9 $\pm$ 4.54 $\pm$ 2.18  \\
\hline

1.743 & 0.223 & 0.248 & 171 & 42.0 $\pm$ 6.32 $\pm$ 1.68  \\
\hline

1.744 & 0.223 & 0.249 & 189 & 40.8 $\pm$ 5.61 $\pm$ 2.67  \\
\hline

1.744 & 0.223 & 0.248 & 207 & 41.4 $\pm$ 4.75 $\pm$ 1.12  \\
\hline

1.749 & 0.223 & 0.249 & 225 & 50.1 $\pm$ 5.41 $\pm$ 4.98  \\
\hline

1.748 & 0.223 & 0.249 & 243 & 50.3 $\pm$ 4.16 $\pm$ 2.87  \\
\hline

1.744 & 0.223 & 0.249 & 261 & 63.0 $\pm$ 3.89 $\pm$ 2.38  \\
\hline

1.744 & 0.223 & 0.248 & 279 & 69.3 $\pm$ 4.41 $\pm$ 4.49  \\
\hline

1.747 & 0.223 & 0.249 & 297 & 69.8 $\pm$ 4.16 $\pm$ 7.94  \\
\hline

1.743 & 0.223 & 0.248 & 315 & 54.6 $\pm$ 3.73 $\pm$ 5.28  \\
\hline

1.744 & 0.223 & 0.249 & 333 & 35.6 $\pm$ 4.56 $\pm$ 9.40  \\
\hline

1.745 & 0.223 & 0.248 & 351 & 35.8 $\pm$ 8.69 $\pm$ 8.69  \\
\hline

1.743 & 0.223 & 0.349 & 27 & 35.0 $\pm$ 5.84 $\pm$ 4.89  \\
\hline

1.744 & 0.223 & 0.350 & 45 & 41.7 $\pm$ 3.70 $\pm$ 5.53  \\
\hline

1.743 & 0.223 & 0.349 & 63 & 51.3 $\pm$ 3.61 $\pm$ 4.00  \\
\hline

1.745 & 0.223 & 0.350 & 81 & 62.6 $\pm$ 3.49 $\pm$ 4.98  \\
\hline

1.745 & 0.223 & 0.350 & 99 & 48.6 $\pm$ 3.39 $\pm$ 2.45  \\
\hline

1.745 & 0.223 & 0.349 & 117 & 42.5 $\pm$ 4.51 $\pm$ 3.07  \\
\hline

1.744 & 0.223 & 0.348 & 135 & 41.9 $\pm$ 5.70 $\pm$ 12.2  \\
\hline

1.744 & 0.223 & 0.348 & 153 & 20.5 $\pm$ 4.28 $\pm$ 2.94  \\
\hline

1.748 & 0.224 & 0.349 & 171 & 31.4 $\pm$ 6.16 $\pm$ 4.00  \\
\hline

1.748 & 0.223 & 0.348 & 189 & 33.3 $\pm$ 5.89 $\pm$ 0.81  \\
\hline

1.743 & 0.223 & 0.349 & 207 & 29.1 $\pm$ 4.92 $\pm$ 7.44  \\
\hline

1.746 & 0.223 & 0.350 & 225 & 33.1 $\pm$ 4.78 $\pm$ 0.62  \\
\hline

1.745 & 0.223 & 0.350 & 243 & 42.5 $\pm$ 3.95 $\pm$ 0.53  \\
\hline

1.744 & 0.223 & 0.349 & 261 & 55.5 $\pm$ 3.80 $\pm$ 2.26  \\
\hline

1.744 & 0.223 & 0.349 & 279 & 61.0 $\pm$ 3.93 $\pm$ 3.39  \\
\hline

1.745 & 0.223 & 0.349 & 297 & 53.0 $\pm$ 3.31 $\pm$ 3.36  \\
\hline

1.746 & 0.223 & 0.349 & 315 & 46.3 $\pm$ 3.37 $\pm$ 3.80  \\
\hline

1.744 & 0.223 & 0.349 & 333 & 41.7 $\pm$ 6.29 $\pm$ 4.76  \\
\hline

1.746 & 0.224 & 0.495 & 27 & 24.0 $\pm$ 3.85 $\pm$ 2.30  \\
\hline

1.744 & 0.223 & 0.496 & 45 & 27.6 $\pm$ 2.03 $\pm$ 1.55  \\
\hline

1.744 & 0.223 & 0.496 & 63 & 36.2 $\pm$ 2.03 $\pm$ 1.23  \\
\hline

1.745 & 0.223 & 0.496 & 81 & 44.4 $\pm$ 2.12 $\pm$ 0.92  \\
\hline

1.746 & 0.223 & 0.497 & 99 & 34.6 $\pm$ 2.28 $\pm$ 0.78  \\
\hline

1.744 & 0.223 & 0.497 & 117 & 31.8 $\pm$ 3.39 $\pm$ 2.45  \\
\hline

1.744 & 0.224 & 0.494 & 135 & 37.0 $\pm$ 4.86 $\pm$ 2.05  \\
\hline

1.744 & 0.223 & 0.495 & 153 & 31.3 $\pm$ 5.29 $\pm$ 2.23  \\
\hline

1.748 & 0.224 & 0.492 & 171 & 21.1 $\pm$ 4.98 $\pm$ 4.43  \\
\hline

1.749 & 0.223 & 0.494 & 189 & 18.9 $\pm$ 3.95 $\pm$ 1.67  \\
\hline

1.746 & 0.223 & 0.493 & 207 & 21.7 $\pm$ 4.09 $\pm$ 3.43  \\
\hline

1.744 & 0.223 & 0.494 & 225 & 25.9 $\pm$ 4.00 $\pm$ 5.75  \\
\hline

1.745 & 0.223 & 0.496 & 243 & 34.0 $\pm$ 3.13 $\pm$ 2.70  \\
\hline

1.744 & 0.223 & 0.498 & 261 & 35.6 $\pm$ 2.41 $\pm$ 2.80  \\
\hline

1.744 & 0.223 & 0.497 & 279 & 38.1 $\pm$ 2.21 $\pm$ 2.52  \\
\hline

1.744 & 0.223 & 0.496 & 297 & 32.2 $\pm$ 1.75 $\pm$ 1.43  \\
\hline

1.744 & 0.223 & 0.495 & 315 & 31.2 $\pm$ 1.85 $\pm$ 1.07  \\
\hline

1.742 & 0.223 & 0.495 & 333 & 27.1 $\pm$ 4.29 $\pm$ 8.64  \\
\hline

1.749 & 0.224 & 0.775 & 27 & 16.6 $\pm$ 1.55 $\pm$ 0.90  \\
\hline

1.744 & 0.224 & 0.776 & 45 & 16.7 $\pm$ 1.05 $\pm$ 0.90  \\
\hline

1.745 & 0.224 & 0.777 & 63 & 23.0 $\pm$ 1.15 $\pm$ 1.07  \\
\hline

1.745 & 0.224 & 0.776 & 81 & 22.6 $\pm$ 1.20 $\pm$ 1.00  \\
\hline

1.741 & 0.224 & 0.777 & 99 & 18.7 $\pm$ 1.70 $\pm$ 1.62  \\
\hline

1.744 & 0.224 & 0.776 & 117 & 18.2 $\pm$ 3.13 $\pm$ 0.78  \\
\hline

1.746 & 0.224 & 0.778 & 135 & 18.1 $\pm$ 4.39 $\pm$ 0.48  \\
\hline

1.748 & 0.224 & 0.778 & 153 & 12.0 $\pm$ 3.10 $\pm$ 1.70  \\
\hline

1.752 & 0.224 & 0.778 & 171 & 14.4 $\pm$ 2.08 $\pm$ 1.93  \\
\hline

1.752 & 0.223 & 0.777 & 189 & 10.1 $\pm$ 1.34 $\pm$ 1.44  \\
\hline

1.749 & 0.224 & 0.778 & 207 & 9.83 $\pm$ 1.83 $\pm$ 2.20  \\
\hline

1.745 & 0.224 & 0.777 & 225 & 12.8 $\pm$ 3.69 $\pm$ 1.20  \\
\hline

1.745 & 0.224 & 0.775 & 243 & 15.8 $\pm$ 2.59 $\pm$ 0.64  \\
\hline

1.744 & 0.224 & 0.777 & 261 & 18.4 $\pm$ 1.79 $\pm$ 0.80  \\
\hline

1.744 & 0.224 & 0.777 & 279 & 20.6 $\pm$ 1.31 $\pm$ 1.20  \\
\hline

1.745 & 0.224 & 0.777 & 297 & 18.9 $\pm$ 0.93 $\pm$ 0.62  \\
\hline

1.744 & 0.224 & 0.776 & 315 & 17.5 $\pm$ 0.89 $\pm$ 1.14  \\
\hline

1.747 & 0.224 & 0.777 & 333 & 13.2 $\pm$ 1.43 $\pm$ 2.09  \\
\hline

1.747 & 0.224 & 1.215 & 9 & 7.35 $\pm$ 0.80 $\pm$ 1.21  \\
\hline

1.747 & 0.224 & 1.215 & 27 & 6.63 $\pm$ 0.55 $\pm$ 1.00  \\
\hline

1.746 & 0.224 & 1.215 & 45 & 8.12 $\pm$ 0.65 $\pm$ 0.42  \\
\hline

1.748 & 0.224 & 1.212 & 63 & 9.42 $\pm$ 0.77 $\pm$ 0.50  \\
\hline

1.745 & 0.224 & 1.212 & 81 & 8.39 $\pm$ 1.07 $\pm$ 0.28  \\
\hline

1.747 & 0.224 & 1.211 & 99 & 9.11 $\pm$ 2.15 $\pm$ 1.65  \\
\hline

1.748 & 0.224 & 1.214 & 117 & 8.57 $\pm$ 2.38 $\pm$ 1.45  \\
\hline

1.749 & 0.224 & 1.217 & 135 & 6.19 $\pm$ 1.60 $\pm$ 0.99  \\
\hline

1.746 & 0.224 & 1.217 & 153 & 4.26 $\pm$ 1.14 $\pm$ 0.48  \\
\hline

1.748 & 0.224 & 1.218 & 171 & 4.56 $\pm$ 0.71 $\pm$ 0.41  \\
\hline

1.752 & 0.224 & 1.219 & 189 & 5.44 $\pm$ 0.60 $\pm$ 0.46  \\
\hline

1.750 & 0.224 & 1.216 & 207 & 3.78 $\pm$ 0.67 $\pm$ 1.05  \\
\hline

1.750 & 0.224 & 1.213 & 225 & 5.01 $\pm$ 1.59 $\pm$ 1.56  \\
\hline

1.745 & 0.224 & 1.214 & 243 & 8.60 $\pm$ 2.72 $\pm$ 1.40  \\
\hline

1.745 & 0.224 & 1.213 & 261 & 10.7 $\pm$ 3.23 $\pm$ 0.36  \\
\hline

1.745 & 0.224 & 1.213 & 279 & 7.26 $\pm$ 1.13 $\pm$ 1.26  \\
\hline

1.746 & 0.224 & 1.214 & 297 & 9.37 $\pm$ 0.71 $\pm$ 0.84  \\
\hline

1.747 & 0.224 & 1.215 & 315 & 7.66 $\pm$ 0.54 $\pm$ 0.47  \\
\hline

1.745 & 0.224 & 1.215 & 333 & 7.34 $\pm$ 0.64 $\pm$ 0.65  \\
\hline

1.747 & 0.224 & 1.218 & 351 & 6.54 $\pm$ 0.82 $\pm$ 1.58  \\
\hline

1.749 & 0.224 & 1.719 & 9 & 2.03 $\pm$ 0.28 $\pm$ 0.25  \\
\hline

1.750 & 0.224 & 1.718 & 27 & 3.38 $\pm$ 0.40 $\pm$ 0.49  \\
\hline

1.746 & 0.225 & 1.716 & 45 & 4.35 $\pm$ 0.63 $\pm$ 0.36  \\
\hline

1.749 & 0.225 & 1.716 & 63 & 5.31 $\pm$ 1.33 $\pm$ 0.40  \\
\hline

1.749 & 0.224 & 1.711 & 81 & 6.71 $\pm$ 2.37 $\pm$ 1.60  \\
\hline

1.749 & 0.224 & 1.711 & 99 & 4.21 $\pm$ 0.71 $\pm$ 0.88  \\
\hline

1.748 & 0.224 & 1.712 & 117 & 2.79 $\pm$ 0.70 $\pm$ 0.42  \\
\hline

1.747 & 0.224 & 1.714 & 135 & 0.86 $\pm$ 0.38 $\pm$ 0.23  \\
\hline

1.753 & 0.224 & 1.714 & 153 & 1.90 $\pm$ 0.78 $\pm$ 1.02  \\
\hline

1.751 & 0.224 & 1.715 & 171 & 2.67 $\pm$ 0.60 $\pm$ 0.47  \\
\hline

1.753 & 0.224 & 1.719 & 189 & 2.61 $\pm$ 0.47 $\pm$ 0.64  \\
\hline

1.748 & 0.224 & 1.716 & 207 & 3.19 $\pm$ 0.71 $\pm$ 0.31  \\
\hline

1.750 & 0.224 & 1.715 & 225 & 3.24 $\pm$ 1.08 $\pm$ 1.29  \\
\hline

1.750 & 0.224 & 1.714 & 243 & 4.28 $\pm$ 0.86 $\pm$ 0.53  \\
\hline

1.747 & 0.224 & 1.710 & 261 & 4.06 $\pm$ 0.96 $\pm$ 0.20  \\
\hline

1.751 & 0.225 & 1.712 & 297 & 3.46 $\pm$ 1.00 $\pm$ 0.62  \\
\hline

1.748 & 0.225 & 1.718 & 315 & 4.19 $\pm$ 0.56 $\pm$ 0.95  \\
\hline

1.749 & 0.224 & 1.716 & 333 & 3.40 $\pm$ 0.45 $\pm$ 0.61  \\
\hline

1.750 & 0.224 & 1.717 & 351 & 2.19 $\pm$ 0.33 $\pm$ 0.03  \\
\hline

1.867 & 0.269 & 0.121 & 9 & 44.1 $\pm$ 8.19 $\pm$ 15.1  \\
\hline

1.868 & 0.270 & 0.121 & 27 & 39.3 $\pm$ 6.46 $\pm$ 4.77  \\
\hline

1.867 & 0.270 & 0.121 & 45 & 62.6 $\pm$ 8.15 $\pm$ 4.60  \\
\hline

1.867 & 0.269 & 0.121 & 63 & 62.3 $\pm$ 9.73 $\pm$ 3.37  \\
\hline

1.867 & 0.269 & 0.121 & 81 & 72.4 $\pm$ 11.8 $\pm$ 11.4  \\
\hline

1.865 & 0.269 & 0.121 & 99 & 61.2 $\pm$ 12.2 $\pm$ 2.98  \\
\hline

1.867 & 0.270 & 0.121 & 243 & 73.4 $\pm$ 26.0 $\pm$ 22.4  \\
\hline

1.868 & 0.270 & 0.121 & 261 & 72.7 $\pm$ 15.5 $\pm$ 11.2  \\
\hline

1.867 & 0.269 & 0.121 & 279 & 65.4 $\pm$ 12.6 $\pm$ 12.3  \\
\hline

1.871 & 0.270 & 0.121 & 297 & 57.3 $\pm$ 8.45 $\pm$ 13.2  \\
\hline

1.868 & 0.270 & 0.121 & 315 & 60.2 $\pm$ 7.59 $\pm$ 4.69  \\
\hline

1.869 & 0.270 & 0.122 & 333 & 44.4 $\pm$ 6.93 $\pm$ 9.53  \\
\hline

1.866 & 0.269 & 0.121 & 351 & 43.5 $\pm$ 8.70 $\pm$ 23.5  \\
\hline

1.869 & 0.271 & 0.174 & 9 & 72.3 $\pm$ 10.3 $\pm$ 24.6  \\
\hline

1.868 & 0.271 & 0.174 & 27 & 64.3 $\pm$ 8.60 $\pm$ 3.66  \\
\hline

1.871 & 0.271 & 0.175 & 45 & 70.6 $\pm$ 9.26 $\pm$ 5.96  \\
\hline

1.868 & 0.271 & 0.175 & 63 & 59.2 $\pm$ 10.2 $\pm$ 2.76  \\
\hline

1.868 & 0.271 & 0.175 & 81 & 77.2 $\pm$ 11.5 $\pm$ 2.13  \\
\hline

1.867 & 0.270 & 0.175 & 99 & 62.6 $\pm$ 10.2 $\pm$ 7.11  \\
\hline

1.870 & 0.270 & 0.175 & 117 & 67.8 $\pm$ 20.4 $\pm$ 17.1  \\
\hline

1.869 & 0.271 & 0.175 & 243 & 66.0 $\pm$ 18.3 $\pm$ 14.2  \\
\hline

1.867 & 0.271 & 0.175 & 261 & 73.3 $\pm$ 12.6 $\pm$ 13.7  \\
\hline

1.871 & 0.271 & 0.175 & 279 & 70.5 $\pm$ 12.1 $\pm$ 7.59  \\
\hline

1.867 & 0.271 & 0.176 & 297 & 70.6 $\pm$ 9.61 $\pm$ 16.5  \\
\hline

1.871 & 0.271 & 0.174 & 315 & 72.7 $\pm$ 9.09 $\pm$ 3.46  \\
\hline

1.866 & 0.271 & 0.175 & 333 & 80.7 $\pm$ 10.2 $\pm$ 8.53  \\
\hline

1.868 & 0.271 & 0.175 & 351 & 75.4 $\pm$ 11.4 $\pm$ 15.7  \\
\hline

1.869 & 0.271 & 0.249 & 9 & 51.6 $\pm$ 5.81 $\pm$ 5.53  \\
\hline

1.870 & 0.271 & 0.248 & 27 & 64.1 $\pm$ 5.46 $\pm$ 3.71  \\
\hline

1.869 & 0.271 & 0.248 & 45 & 69.4 $\pm$ 6.11 $\pm$ 8.12  \\
\hline

1.868 & 0.271 & 0.249 & 63 & 96.3 $\pm$ 8.45 $\pm$ 2.57  \\
\hline

1.868 & 0.270 & 0.249 & 81 & 87.3 $\pm$ 7.97 $\pm$ 2.75  \\
\hline

1.868 & 0.271 & 0.248 & 99 & 75.8 $\pm$ 8.93 $\pm$ 1.44  \\
\hline

1.869 & 0.271 & 0.249 & 117 & 76.8 $\pm$ 18.6 $\pm$ 2.93  \\
\hline

1.870 & 0.270 & 0.249 & 153 & 57.5 $\pm$ 20.3 $\pm$ 7.61  \\
\hline

1.867 & 0.270 & 0.250 & 189 & 39.4 $\pm$ 12.4 $\pm$ 9.66  \\
\hline

1.870 & 0.270 & 0.249 & 207 & 69.7 $\pm$ 24.6 $\pm$ 26.8  \\
\hline

1.870 & 0.271 & 0.249 & 225 & 97.2 $\pm$ 34.4 $\pm$ 54.7  \\
\hline

1.871 & 0.271 & 0.248 & 243 & 72.4 $\pm$ 15.4 $\pm$ 1.87  \\
\hline

1.869 & 0.270 & 0.250 & 261 & 73.1 $\pm$ 10.3 $\pm$ 8.62  \\
\hline

1.868 & 0.270 & 0.249 & 279 & 87.6 $\pm$ 9.14 $\pm$ 3.27  \\
\hline

1.871 & 0.271 & 0.249 & 297 & 92.2 $\pm$ 7.11 $\pm$ 9.88  \\
\hline

1.870 & 0.271 & 0.249 & 315 & 57.9 $\pm$ 5.02 $\pm$ 5.80  \\
\hline

1.871 & 0.271 & 0.249 & 333 & 60.1 $\pm$ 5.92 $\pm$ 6.63  \\
\hline

1.868 & 0.271 & 0.249 & 351 & 38.8 $\pm$ 5.60 $\pm$ 9.42  \\
\hline

1.871 & 0.271 & 0.349 & 9 & 43.5 $\pm$ 7.05 $\pm$ 4.85  \\
\hline

1.869 & 0.271 & 0.349 & 27 & 45.6 $\pm$ 5.06 $\pm$ 4.95  \\
\hline

1.868 & 0.271 & 0.350 & 45 & 63.5 $\pm$ 5.95 $\pm$ 2.66  \\
\hline

1.869 & 0.271 & 0.349 & 63 & 88.4 $\pm$ 7.39 $\pm$ 12.7  \\
\hline

1.868 & 0.271 & 0.349 & 81 & 74.1 $\pm$ 7.13 $\pm$ 3.98  \\
\hline

1.871 & 0.271 & 0.349 & 99 & 89.3 $\pm$ 12.6 $\pm$ 8.06  \\
\hline

1.870 & 0.271 & 0.349 & 117 & 49.7 $\pm$ 20.3 $\pm$ 11.7  \\
\hline

1.870 & 0.270 & 0.349 & 153 & 45.1 $\pm$ 14.3 $\pm$ 0.90  \\
\hline

1.871 & 0.271 & 0.348 & 171 & 27.3 $\pm$ 9.64 $\pm$ 4.27  \\
\hline

1.871 & 0.271 & 0.349 & 189 & 26.2 $\pm$ 6.77 $\pm$ 4.24  \\
\hline

1.873 & 0.271 & 0.349 & 207 & 59.2 $\pm$ 15.3 $\pm$ 8.28  \\
\hline

1.869 & 0.270 & 0.349 & 243 & 33.2 $\pm$ 14.9 $\pm$ 12.9  \\
\hline

1.870 & 0.271 & 0.349 & 261 & 104. $\pm$ 15.4 $\pm$ 4.35  \\
\hline

1.868 & 0.271 & 0.349 & 279 & 99.2 $\pm$ 9.92 $\pm$ 6.55  \\
\hline

1.868 & 0.271 & 0.349 & 297 & 74.7 $\pm$ 6.10 $\pm$ 5.24  \\
\hline

1.870 & 0.271 & 0.349 & 315 & 78.2 $\pm$ 5.84 $\pm$ 4.90  \\
\hline

1.871 & 0.271 & 0.350 & 333 & 41.5 $\pm$ 5.15 $\pm$ 1.65  \\
\hline

1.869 & 0.270 & 0.349 & 351 & 36.1 $\pm$ 6.95 $\pm$ 4.66  \\
\hline

1.870 & 0.271 & 0.496 & 9 & 24.6 $\pm$ 7.41 $\pm$ 3.25  \\
\hline

1.866 & 0.271 & 0.497 & 27 & 40.7 $\pm$ 3.89 $\pm$ 3.60  \\
\hline

1.870 & 0.271 & 0.498 & 45 & 51.8 $\pm$ 3.93 $\pm$ 3.53  \\
\hline

1.869 & 0.271 & 0.497 & 63 & 50.8 $\pm$ 3.88 $\pm$ 2.99  \\
\hline

1.870 & 0.271 & 0.498 & 81 & 50.1 $\pm$ 4.44 $\pm$ 2.77  \\
\hline

1.870 & 0.271 & 0.498 & 99 & 55.2 $\pm$ 9.33 $\pm$ 1.58  \\
\hline

1.871 & 0.271 & 0.497 & 135 & 34.1 $\pm$ 12.0 $\pm$ 9.14  \\
\hline

1.870 & 0.271 & 0.495 & 153 & 27.0 $\pm$ 5.52 $\pm$ 11.6  \\
\hline

1.872 & 0.271 & 0.493 & 171 & 14.4 $\pm$ 3.48 $\pm$ 1.51  \\
\hline

1.869 & 0.271 & 0.493 & 189 & 27.9 $\pm$ 3.60 $\pm$ 4.38  \\
\hline

1.870 & 0.271 & 0.495 & 207 & 27.6 $\pm$ 4.61 $\pm$ 3.29  \\
\hline

1.871 & 0.271 & 0.497 & 225 & 37.0 $\pm$ 11.2 $\pm$ 6.58  \\
\hline

1.871 & 0.271 & 0.500 & 261 & 54.3 $\pm$ 11.6 $\pm$ 3.11  \\
\hline

1.869 & 0.271 & 0.498 & 279 & 58.9 $\pm$ 5.81 $\pm$ 3.79  \\
\hline

1.870 & 0.271 & 0.497 & 297 & 58.8 $\pm$ 3.63 $\pm$ 1.35  \\
\hline

1.870 & 0.271 & 0.496 & 315 & 43.8 $\pm$ 3.07 $\pm$ 1.94  \\
\hline

1.871 & 0.271 & 0.497 & 333 & 31.8 $\pm$ 3.89 $\pm$ 4.92  \\
\hline

1.869 & 0.271 & 0.496 & 351 & 28.5 $\pm$ 9.49 $\pm$ 5.72  \\
\hline

1.870 & 0.271 & 0.777 & 27 & 21.6 $\pm$ 2.11 $\pm$ 1.04  \\
\hline

1.868 & 0.271 & 0.779 & 45 & 26.3 $\pm$ 1.97 $\pm$ 0.89  \\
\hline

1.870 & 0.271 & 0.783 & 63 & 31.1 $\pm$ 2.31 $\pm$ 1.41  \\
\hline

1.869 & 0.271 & 0.781 & 81 & 24.5 $\pm$ 3.02 $\pm$ 3.20  \\
\hline

1.869 & 0.271 & 0.783 & 99 & 32.6 $\pm$ 7.49 $\pm$ 6.17  \\
\hline

1.870 & 0.271 & 0.781 & 117 & 37.9 $\pm$ 12.6 $\pm$ 8.12  \\
\hline

1.870 & 0.271 & 0.780 & 135 & 23.9 $\pm$ 4.98 $\pm$ 2.61  \\
\hline

1.871 & 0.271 & 0.778 & 153 & 26.1 $\pm$ 3.38 $\pm$ 3.70  \\
\hline

1.871 & 0.271 & 0.779 & 171 & 20.2 $\pm$ 2.47 $\pm$ 3.43  \\
\hline

1.870 & 0.271 & 0.778 & 189 & 15.1 $\pm$ 1.52 $\pm$ 1.82  \\
\hline

1.871 & 0.271 & 0.779 & 207 & 18.9 $\pm$ 2.21 $\pm$ 3.51  \\
\hline

1.870 & 0.271 & 0.777 & 225 & 27.0 $\pm$ 4.16 $\pm$ 3.55  \\
\hline

1.870 & 0.271 & 0.779 & 243 & 38.8 $\pm$ 11.2 $\pm$ 4.68  \\
\hline

1.869 & 0.271 & 0.781 & 261 & 41.1 $\pm$ 13.7 $\pm$ 4.80  \\
\hline

1.870 & 0.271 & 0.784 & 279 & 22.7 $\pm$ 3.42 $\pm$ 1.39  \\
\hline

1.868 & 0.271 & 0.782 & 297 & 28.9 $\pm$ 1.93 $\pm$ 0.72  \\
\hline

1.870 & 0.271 & 0.781 & 315 & 25.2 $\pm$ 1.64 $\pm$ 1.53  \\
\hline

1.869 & 0.271 & 0.780 & 333 & 20.8 $\pm$ 2.51 $\pm$ 2.79  \\
\hline

1.870 & 0.272 & 1.220 & 9 & 5.27 $\pm$ 1.52 $\pm$ 1.26  \\
\hline

1.870 & 0.271 & 1.215 & 27 & 10.7 $\pm$ 1.16 $\pm$ 1.27  \\
\hline

1.869 & 0.272 & 1.218 & 45 & 12.9 $\pm$ 1.34 $\pm$ 1.31  \\
\hline

1.872 & 0.272 & 1.215 & 63 & 14.5 $\pm$ 2.03 $\pm$ 0.82  \\
\hline

1.870 & 0.272 & 1.217 & 81 & 15.0 $\pm$ 4.34 $\pm$ 1.64  \\
\hline

1.870 & 0.272 & 1.213 & 99 & 19.5 $\pm$ 3.40 $\pm$ 2.10  \\
\hline

1.870 & 0.271 & 1.214 & 117 & 13.4 $\pm$ 2.49 $\pm$ 0.99  \\
\hline

1.871 & 0.272 & 1.216 & 135 & 12.0 $\pm$ 2.74 $\pm$ 1.30  \\
\hline

1.870 & 0.271 & 1.216 & 153 & 13.7 $\pm$ 2.42 $\pm$ 2.55  \\
\hline

1.870 & 0.271 & 1.219 & 171 & 9.15 $\pm$ 1.55 $\pm$ 1.39  \\
\hline

1.871 & 0.271 & 1.221 & 189 & 11.9 $\pm$ 1.35 $\pm$ 0.99  \\
\hline

1.872 & 0.272 & 1.217 & 207 & 10.1 $\pm$ 1.73 $\pm$ 1.37  \\
\hline

1.870 & 0.271 & 1.218 & 225 & 13.3 $\pm$ 2.31 $\pm$ 2.54  \\
\hline

1.870 & 0.271 & 1.215 & 243 & 11.4 $\pm$ 3.05 $\pm$ 2.67  \\
\hline

1.870 & 0.272 & 1.217 & 261 & 23.8 $\pm$ 7.17 $\pm$ 6.44  \\
\hline

1.872 & 0.272 & 1.217 & 279 & 11.7 $\pm$ 3.90 $\pm$ 2.74  \\
\hline

1.870 & 0.272 & 1.215 & 297 & 11.5 $\pm$ 1.59 $\pm$ 1.37  \\
\hline

1.871 & 0.271 & 1.215 & 315 & 13.5 $\pm$ 1.23 $\pm$ 1.28  \\
\hline

1.870 & 0.271 & 1.218 & 333 & 7.62 $\pm$ 1.05 $\pm$ 0.48  \\
\hline

1.872 & 0.272 & 1.218 & 351 & 9.60 $\pm$ 2.48 $\pm$ 0.87  \\
\hline

1.871 & 0.272 & 1.723 & 9 & 2.50 $\pm$ 0.52 $\pm$ 0.32  \\
\hline

1.870 & 0.272 & 1.717 & 27 & 2.93 $\pm$ 0.55 $\pm$ 0.14  \\
\hline

1.869 & 0.272 & 1.720 & 45 & 4.33 $\pm$ 1.20 $\pm$ 0.38  \\
\hline

1.872 & 0.272 & 1.717 & 81 & 5.80 $\pm$ 1.67 $\pm$ 0.64  \\
\hline

1.869 & 0.272 & 1.718 & 99 & 9.45 $\pm$ 1.10 $\pm$ 1.39  \\
\hline

1.872 & 0.272 & 1.716 & 117 & 7.83 $\pm$ 1.43 $\pm$ 1.08  \\
\hline

1.874 & 0.272 & 1.718 & 135 & 5.63 $\pm$ 2.13 $\pm$ 1.31  \\
\hline

1.870 & 0.272 & 1.721 & 153 & 8.44 $\pm$ 1.99 $\pm$ 0.33  \\
\hline

1.871 & 0.272 & 1.722 & 171 & 6.99 $\pm$ 1.87 $\pm$ 0.55  \\
\hline

1.872 & 0.272 & 1.726 & 189 & 4.48 $\pm$ 1.20 $\pm$ 0.63  \\
\hline

1.876 & 0.273 & 1.724 & 207 & 6.24 $\pm$ 2.08 $\pm$ 1.14  \\
\hline

1.869 & 0.272 & 1.718 & 225 & 9.36 $\pm$ 2.09 $\pm$ 1.87  \\
\hline

1.872 & 0.272 & 1.716 & 243 & 7.07 $\pm$ 1.89 $\pm$ 1.56  \\
\hline

1.871 & 0.272 & 1.712 & 261 & 9.07 $\pm$ 1.66 $\pm$ 0.72  \\
\hline

1.874 & 0.272 & 1.715 & 279 & 9.78 $\pm$ 2.24 $\pm$ 2.88  \\
\hline

1.871 & 0.273 & 1.721 & 315 & 5.86 $\pm$ 1.28 $\pm$ 0.36  \\
\hline

1.870 & 0.272 & 1.717 & 333 & 4.81 $\pm$ 0.84 $\pm$ 1.20  \\
\hline

1.871 & 0.272 & 1.721 & 351 & 2.99 $\pm$ 0.61 $\pm$ 0.35  \\
\hline

1.948 & 0.311 & 0.133 & 27 & 90.1 $\pm$ 36.8 $\pm$ 28.1  \\
\hline

1.953 & 0.313 & 0.175 & 9 & 69.7 $\pm$ 23.3 $\pm$ 8.24  \\
\hline

1.951 & 0.313 & 0.175 & 27 & 51.8 $\pm$ 19.6 $\pm$ 9.66  \\
\hline

1.950 & 0.313 & 0.176 & 45 & 104. $\pm$ 28.7 $\pm$ 12.3  \\
\hline

1.951 & 0.312 & 0.176 & 63 & 88.6 $\pm$ 33.5 $\pm$ 17.9  \\
\hline

1.954 & 0.313 & 0.176 & 297 & 49.8 $\pm$ 20.4 $\pm$ 16.5  \\
\hline

1.951 & 0.313 & 0.176 & 315 & 61.0 $\pm$ 21.6 $\pm$ 4.35  \\
\hline

1.957 & 0.313 & 0.176 & 333 & 59.7 $\pm$ 22.6 $\pm$ 5.28  \\
\hline

1.952 & 0.313 & 0.174 & 351 & 75.5 $\pm$ 28.5 $\pm$ 10.2  \\
\hline

1.952 & 0.313 & 0.249 & 9 & 43.7 $\pm$ 11.3 $\pm$ 12.0  \\
\hline

1.954 & 0.313 & 0.249 & 27 & 54.6 $\pm$ 12.5 $\pm$ 24.8  \\
\hline

1.954 & 0.313 & 0.250 & 45 & 107. $\pm$ 19.6 $\pm$ 5.97  \\
\hline

1.953 & 0.313 & 0.248 & 63 & 99.3 $\pm$ 23.4 $\pm$ 25.9  \\
\hline

1.953 & 0.313 & 0.248 & 81 & 96.8 $\pm$ 36.6 $\pm$ 6.60  \\
\hline

1.951 & 0.313 & 0.249 & 297 & 103. $\pm$ 21.9 $\pm$ 8.32  \\
\hline

1.950 & 0.312 & 0.248 & 315 & 57.3 $\pm$ 13.2 $\pm$ 12.8  \\
\hline

1.952 & 0.313 & 0.248 & 333 & 57.4 $\pm$ 14.4 $\pm$ 4.89  \\
\hline

1.952 & 0.313 & 0.250 & 351 & 45.0 $\pm$ 13.6 $\pm$ 8.43  \\
\hline

1.953 & 0.314 & 0.348 & 9 & 50.1 $\pm$ 11.8 $\pm$ 5.06  \\
\hline

1.952 & 0.313 & 0.349 & 27 & 59.0 $\pm$ 12.3 $\pm$ 2.18  \\
\hline

1.953 & 0.313 & 0.350 & 45 & 99.5 $\pm$ 16.1 $\pm$ 16.1  \\
\hline

1.949 & 0.312 & 0.347 & 63 & 107. $\pm$ 24.0 $\pm$ 9.62  \\
\hline

1.956 & 0.313 & 0.349 & 153 & 92.5 $\pm$ 30.9 $\pm$ 14.1  \\
\hline

1.952 & 0.312 & 0.349 & 189 & 50.9 $\pm$ 18.0 $\pm$ 5.37  \\
\hline

1.952 & 0.312 & 0.349 & 225 & 75.0 $\pm$ 30.6 $\pm$ 7.17  \\
\hline

1.955 & 0.313 & 0.350 & 243 & 109. $\pm$ 48.7 $\pm$ 42.7  \\
\hline

1.954 & 0.313 & 0.351 & 279 & 87.6 $\pm$ 39.2 $\pm$ 11.6  \\
\hline

1.954 & 0.313 & 0.351 & 297 & 65.3 $\pm$ 14.3 $\pm$ 22.6  \\
\hline

1.952 & 0.313 & 0.347 & 315 & 71.5 $\pm$ 13.8 $\pm$ 9.44  \\
\hline

1.953 & 0.313 & 0.349 & 333 & 55.4 $\pm$ 12.7 $\pm$ 5.35  \\
\hline

1.954 & 0.313 & 0.350 & 351 & 56.7 $\pm$ 13.4 $\pm$ 14.0  \\
\hline

1.953 & 0.313 & 0.495 & 9 & 36.7 $\pm$ 9.19 $\pm$ 5.62  \\
\hline

1.956 & 0.313 & 0.498 & 27 & 56.3 $\pm$ 8.40 $\pm$ 7.23  \\
\hline

1.955 & 0.313 & 0.496 & 45 & 72.3 $\pm$ 10.5 $\pm$ 1.09  \\
\hline

1.955 & 0.313 & 0.495 & 63 & 76.8 $\pm$ 15.4 $\pm$ 21.3  \\
\hline

1.952 & 0.313 & 0.497 & 135 & 51.1 $\pm$ 16.2 $\pm$ 10.3  \\
\hline

1.954 & 0.313 & 0.493 & 153 & 32.1 $\pm$ 10.2 $\pm$ 11.8  \\
\hline

1.954 & 0.313 & 0.494 & 171 & 102. $\pm$ 23.3 $\pm$ 21.5  \\
\hline

1.954 & 0.313 & 0.494 & 189 & 30.6 $\pm$ 7.90 $\pm$ 6.94  \\
\hline

1.952 & 0.313 & 0.499 & 225 & 60.3 $\pm$ 15.1 $\pm$ 33.0  \\
\hline

1.953 & 0.313 & 0.495 & 243 & 46.3 $\pm$ 18.9 $\pm$ 10.3  \\
\hline

1.952 & 0.313 & 0.497 & 279 & 70.0 $\pm$ 31.3 $\pm$ 9.67  \\
\hline

1.953 & 0.313 & 0.496 & 297 & 58.4 $\pm$ 10.9 $\pm$ 6.86  \\
\hline

1.953 & 0.313 & 0.495 & 315 & 51.5 $\pm$ 7.68 $\pm$ 4.53  \\
\hline

1.953 & 0.313 & 0.494 & 333 & 48.0 $\pm$ 9.07 $\pm$ 3.38  \\
\hline

1.953 & 0.313 & 0.496 & 351 & 45.4 $\pm$ 11.4 $\pm$ 5.42  \\
\hline

1.953 & 0.313 & 0.780 & 27 & 19.5 $\pm$ 3.82 $\pm$ 6.14  \\
\hline

1.953 & 0.313 & 0.783 & 45 & 26.8 $\pm$ 4.53 $\pm$ 2.00  \\
\hline

1.952 & 0.313 & 0.789 & 63 & 39.2 $\pm$ 8.18 $\pm$ 5.63  \\
\hline

1.954 & 0.313 & 0.787 & 81 & 26.2 $\pm$ 10.7 $\pm$ 1.91  \\
\hline

1.954 & 0.313 & 0.783 & 117 & 27.1 $\pm$ 10.3 $\pm$ 4.75  \\
\hline

1.953 & 0.313 & 0.776 & 135 & 39.6 $\pm$ 11.4 $\pm$ 6.64  \\
\hline

1.954 & 0.313 & 0.779 & 153 & 34.4 $\pm$ 7.69 $\pm$ 11.2  \\
\hline

1.953 & 0.313 & 0.778 & 171 & 25.3 $\pm$ 7.01 $\pm$ 2.08  \\
\hline

1.953 & 0.312 & 0.778 & 189 & 25.5 $\pm$ 5.10 $\pm$ 0.35  \\
\hline

1.953 & 0.313 & 0.782 & 207 & 33.6 $\pm$ 8.67 $\pm$ 11.2  \\
\hline

1.954 & 0.313 & 0.785 & 225 & 39.4 $\pm$ 7.88 $\pm$ 2.27  \\
\hline

1.953 & 0.313 & 0.783 & 243 & 41.5 $\pm$ 12.5 $\pm$ 8.82  \\
\hline

1.953 & 0.313 & 0.789 & 297 & 32.6 $\pm$ 6.53 $\pm$ 1.66  \\
\hline

1.953 & 0.314 & 0.784 & 315 & 39.6 $\pm$ 5.03 $\pm$ 3.50  \\
\hline

1.953 & 0.313 & 0.788 & 333 & 36.8 $\pm$ 6.32 $\pm$ 4.98  \\
\hline

1.951 & 0.313 & 1.217 & 27 & 15.2 $\pm$ 3.10 $\pm$ 1.95  \\
\hline

1.953 & 0.313 & 1.216 & 45 & 23.8 $\pm$ 4.67 $\pm$ 2.09  \\
\hline

1.954 & 0.313 & 1.219 & 63 & 34.6 $\pm$ 10.9 $\pm$ 4.13  \\
\hline

1.953 & 0.314 & 1.216 & 99 & 24.9 $\pm$ 5.58 $\pm$ 6.07  \\
\hline

1.953 & 0.313 & 1.217 & 117 & 43.0 $\pm$ 8.61 $\pm$ 1.74  \\
\hline

1.952 & 0.313 & 1.221 & 135 & 30.1 $\pm$ 11.4 $\pm$ 6.05  \\
\hline

1.953 & 0.313 & 1.223 & 153 & 30.8 $\pm$ 7.97 $\pm$ 1.94  \\
\hline

1.955 & 0.313 & 1.221 & 171 & 26.2 $\pm$ 9.27 $\pm$ 5.53  \\
\hline

1.955 & 0.313 & 1.223 & 189 & 15.0 $\pm$ 5.01 $\pm$ 0.97  \\
\hline

1.954 & 0.313 & 1.223 & 225 & 24.0 $\pm$ 6.41 $\pm$ 3.12  \\
\hline

1.952 & 0.313 & 1.219 & 243 & 49.1 $\pm$ 16.3 $\pm$ 4.61  \\
\hline

1.955 & 0.314 & 1.222 & 261 & 22.9 $\pm$ 7.63 $\pm$ 1.93  \\
\hline

1.954 & 0.313 & 1.220 & 297 & 13.1 $\pm$ 4.96 $\pm$ 3.40  \\
\hline

1.952 & 0.313 & 1.220 & 315 & 11.5 $\pm$ 2.79 $\pm$ 0.93  \\
\hline

1.953 & 0.313 & 1.216 & 333 & 13.7 $\pm$ 3.43 $\pm$ 1.02  \\
\hline

1.954 & 0.313 & 1.731 & 27 & 5.86 $\pm$ 1.95 $\pm$ 0.61  \\
\hline

1.955 & 0.313 & 1.707 & 81 & 13.7 $\pm$ 3.97 $\pm$ 3.05  \\
\hline

1.954 & 0.313 & 1.720 & 99 & 13.4 $\pm$ 2.86 $\pm$ 1.29  \\
\hline

1.952 & 0.314 & 1.725 & 117 & 15.9 $\pm$ 4.58 $\pm$ 2.35  \\
\hline

1.954 & 0.313 & 1.721 & 261 & 9.41 $\pm$ 3.14 $\pm$ 2.68  \\
\hline

1.954 & 0.314 & 1.725 & 279 & 10.2 $\pm$ 3.40 $\pm$ 1.43  \\
\hline

1.954 & 0.314 & 1.718 & 333 & 12.7 $\pm$ 3.83 $\pm$ 1.63  \\
\hline

2.099 & 0.238 & 0.120 & 27 & 61.1 $\pm$ 23.1 $\pm$ 4.57  \\
\hline

2.103 & 0.238 & 0.120 & 63 & 32.1 $\pm$ 11.4 $\pm$ 5.24  \\
\hline

2.097 & 0.238 & 0.119 & 81 & 32.9 $\pm$ 9.92 $\pm$ 8.80  \\
\hline

2.094 & 0.238 & 0.120 & 99 & 39.6 $\pm$ 8.85 $\pm$ 4.55  \\
\hline

2.102 & 0.239 & 0.120 & 117 & 24.8 $\pm$ 7.48 $\pm$ 7.78  \\
\hline

2.098 & 0.238 & 0.120 & 135 & 26.6 $\pm$ 10.1 $\pm$ 7.03  \\
\hline

2.102 & 0.238 & 0.120 & 189 & 35.7 $\pm$ 16.0 $\pm$ 4.90  \\
\hline

2.104 & 0.238 & 0.120 & 207 & 50.3 $\pm$ 16.8 $\pm$ 4.74  \\
\hline

2.100 & 0.238 & 0.120 & 243 & 36.9 $\pm$ 11.1 $\pm$ 3.28  \\
\hline

2.103 & 0.238 & 0.120 & 261 & 31.9 $\pm$ 7.73 $\pm$ 5.18  \\
\hline

2.099 & 0.238 & 0.121 & 279 & 32.8 $\pm$ 9.89 $\pm$ 7.87  \\
\hline

2.095 & 0.238 & 0.119 & 297 & 41.3 $\pm$ 11.9 $\pm$ 6.84  \\
\hline

2.096 & 0.238 & 0.120 & 333 & 70.9 $\pm$ 26.8 $\pm$ 20.0  \\
\hline

2.096 & 0.238 & 0.174 & 45 & 39.7 $\pm$ 16.2 $\pm$ 9.78  \\
\hline

2.099 & 0.239 & 0.175 & 63 & 22.4 $\pm$ 10.0 $\pm$ 9.84  \\
\hline

2.105 & 0.238 & 0.174 & 81 & 67.7 $\pm$ 14.8 $\pm$ 10.5  \\
\hline

2.099 & 0.238 & 0.175 & 99 & 31.0 $\pm$ 8.59 $\pm$ 9.60  \\
\hline

2.098 & 0.238 & 0.174 & 117 & 30.1 $\pm$ 8.69 $\pm$ 7.69  \\
\hline

2.094 & 0.237 & 0.173 & 135 & 42.8 $\pm$ 10.7 $\pm$ 6.40  \\
\hline

2.096 & 0.238 & 0.175 & 153 & 28.3 $\pm$ 8.53 $\pm$ 3.92  \\
\hline

2.102 & 0.239 & 0.175 & 171 & 58.1 $\pm$ 16.8 $\pm$ 5.73  \\
\hline

2.098 & 0.238 & 0.174 & 189 & 39.2 $\pm$ 17.5 $\pm$ 8.72  \\
\hline

2.094 & 0.238 & 0.174 & 225 & 39.4 $\pm$ 13.1 $\pm$ 14.0  \\
\hline

2.098 & 0.238 & 0.175 & 243 & 54.5 $\pm$ 13.6 $\pm$ 14.0  \\
\hline

2.105 & 0.238 & 0.174 & 261 & 46.6 $\pm$ 11.0 $\pm$ 2.94  \\
\hline

2.105 & 0.238 & 0.176 & 279 & 37.2 $\pm$ 11.8 $\pm$ 13.3  \\
\hline

2.100 & 0.238 & 0.175 & 297 & 24.6 $\pm$ 10.0 $\pm$ 0.49  \\
\hline

2.106 & 0.239 & 0.177 & 315 & 88.7 $\pm$ 24.6 $\pm$ 3.66  \\
\hline

2.098 & 0.238 & 0.249 & 45 & 53.4 $\pm$ 14.3 $\pm$ 7.34  \\
\hline

2.100 & 0.238 & 0.249 & 63 & 42.5 $\pm$ 8.34 $\pm$ 2.00  \\
\hline

2.101 & 0.238 & 0.248 & 81 & 47.5 $\pm$ 7.24 $\pm$ 4.97  \\
\hline

2.098 & 0.238 & 0.248 & 99 & 43.5 $\pm$ 7.15 $\pm$ 1.61  \\
\hline

2.097 & 0.237 & 0.250 & 117 & 33.7 $\pm$ 6.89 $\pm$ 1.87  \\
\hline

2.097 & 0.238 & 0.248 & 135 & 40.1 $\pm$ 7.32 $\pm$ 0.51  \\
\hline

2.100 & 0.238 & 0.249 & 153 & 26.6 $\pm$ 5.81 $\pm$ 4.87  \\
\hline

2.103 & 0.239 & 0.249 & 171 & 29.1 $\pm$ 7.79 $\pm$ 6.37  \\
\hline

2.097 & 0.238 & 0.249 & 207 & 34.2 $\pm$ 7.66 $\pm$ 3.00  \\
\hline

2.102 & 0.238 & 0.249 & 225 & 31.9 $\pm$ 7.31 $\pm$ 2.17  \\
\hline

2.098 & 0.238 & 0.249 & 243 & 43.5 $\pm$ 8.23 $\pm$ 9.64  \\
\hline

2.105 & 0.238 & 0.249 & 261 & 32.7 $\pm$ 6.08 $\pm$ 4.90  \\
\hline

2.098 & 0.238 & 0.249 & 279 & 21.8 $\pm$ 5.29 $\pm$ 0.53  \\
\hline

2.099 & 0.238 & 0.250 & 297 & 39.1 $\pm$ 7.67 $\pm$ 3.84  \\
\hline

2.097 & 0.238 & 0.250 & 315 & 53.9 $\pm$ 12.1 $\pm$ 6.07  \\
\hline

2.098 & 0.238 & 0.349 & 45 & 49.5 $\pm$ 13.2 $\pm$ 11.0  \\
\hline

2.094 & 0.238 & 0.350 & 63 & 45.3 $\pm$ 7.46 $\pm$ 0.46  \\
\hline

2.101 & 0.238 & 0.350 & 81 & 27.5 $\pm$ 5.01 $\pm$ 0.82  \\
\hline

2.100 & 0.238 & 0.350 & 99 & 43.7 $\pm$ 6.92 $\pm$ 3.92  \\
\hline

2.100 & 0.238 & 0.350 & 117 & 27.8 $\pm$ 6.55 $\pm$ 12.0  \\
\hline

2.097 & 0.238 & 0.349 & 135 & 12.4 $\pm$ 4.14 $\pm$ 1.03  \\
\hline

2.100 & 0.238 & 0.347 & 153 & 32.7 $\pm$ 6.83 $\pm$ 5.43  \\
\hline

2.098 & 0.238 & 0.350 & 171 & 37.2 $\pm$ 9.02 $\pm$ 2.24  \\
\hline

2.101 & 0.238 & 0.348 & 189 & 21.1 $\pm$ 6.68 $\pm$ 3.42  \\
\hline

2.100 & 0.238 & 0.349 & 207 & 34.5 $\pm$ 7.36 $\pm$ 3.85  \\
\hline

2.098 & 0.238 & 0.350 & 225 & 25.2 $\pm$ 6.51 $\pm$ 9.23  \\
\hline

2.097 & 0.238 & 0.350 & 243 & 34.8 $\pm$ 7.11 $\pm$ 1.18  \\
\hline

2.101 & 0.238 & 0.350 & 261 & 28.2 $\pm$ 5.16 $\pm$ 3.25  \\
\hline

2.096 & 0.238 & 0.348 & 279 & 28.8 $\pm$ 5.76 $\pm$ 8.07  \\
\hline

2.101 & 0.238 & 0.349 & 297 & 40.7 $\pm$ 7.10 $\pm$ 16.8  \\
\hline

2.098 & 0.238 & 0.350 & 315 & 35.3 $\pm$ 10.2 $\pm$ 5.44  \\
\hline

2.099 & 0.238 & 0.493 & 45 & 15.9 $\pm$ 4.26 $\pm$ 2.01  \\
\hline

2.098 & 0.238 & 0.497 & 63 & 20.1 $\pm$ 3.35 $\pm$ 2.75  \\
\hline

2.099 & 0.238 & 0.499 & 81 & 30.8 $\pm$ 3.58 $\pm$ 1.92  \\
\hline

2.096 & 0.238 & 0.497 & 99 & 21.6 $\pm$ 3.30 $\pm$ 1.76  \\
\hline

2.100 & 0.238 & 0.496 & 117 & 24.0 $\pm$ 4.24 $\pm$ 0.33  \\
\hline

2.098 & 0.238 & 0.495 & 135 & 37.3 $\pm$ 5.70 $\pm$ 3.19  \\
\hline

2.099 & 0.238 & 0.495 & 153 & 17.9 $\pm$ 4.78 $\pm$ 1.24  \\
\hline

2.099 & 0.238 & 0.494 & 171 & 36.9 $\pm$ 9.22 $\pm$ 8.27  \\
\hline

2.098 & 0.238 & 0.495 & 189 & 33.3 $\pm$ 8.33 $\pm$ 3.83  \\
\hline

2.099 & 0.238 & 0.496 & 207 & 19.0 $\pm$ 5.07 $\pm$ 2.97  \\
\hline

2.098 & 0.238 & 0.495 & 225 & 30.4 $\pm$ 5.97 $\pm$ 0.40  \\
\hline

2.099 & 0.238 & 0.496 & 243 & 27.2 $\pm$ 4.19 $\pm$ 5.49  \\
\hline

2.100 & 0.238 & 0.494 & 261 & 32.3 $\pm$ 4.04 $\pm$ 2.74  \\
\hline

2.097 & 0.238 & 0.497 & 279 & 26.3 $\pm$ 3.80 $\pm$ 1.28  \\
\hline

2.099 & 0.238 & 0.496 & 297 & 18.5 $\pm$ 3.13 $\pm$ 1.37  \\
\hline

2.097 & 0.238 & 0.494 & 315 & 15.8 $\pm$ 3.73 $\pm$ 4.22  \\
\hline

2.102 & 0.239 & 0.778 & 27 & 12.5 $\pm$ 4.15 $\pm$ 0.13  \\
\hline

2.096 & 0.238 & 0.774 & 45 & 11.7 $\pm$ 1.89 $\pm$ 1.93  \\
\hline

2.098 & 0.238 & 0.776 & 63 & 12.3 $\pm$ 1.77 $\pm$ 0.13  \\
\hline

2.099 & 0.238 & 0.779 & 81 & 14.9 $\pm$ 1.82 $\pm$ 0.41  \\
\hline

2.098 & 0.238 & 0.777 & 99 & 13.7 $\pm$ 2.16 $\pm$ 1.20  \\
\hline

2.098 & 0.238 & 0.782 & 117 & 14.5 $\pm$ 3.25 $\pm$ 2.35  \\
\hline

2.100 & 0.238 & 0.776 & 135 & 12.1 $\pm$ 4.04 $\pm$ 2.07  \\
\hline

2.098 & 0.238 & 0.778 & 225 & 18.0 $\pm$ 6.00 $\pm$ 2.14  \\
\hline

2.098 & 0.239 & 0.778 & 243 & 18.1 $\pm$ 3.43 $\pm$ 2.13  \\
\hline

2.100 & 0.238 & 0.776 & 261 & 12.5 $\pm$ 2.03 $\pm$ 2.16  \\
\hline

2.098 & 0.238 & 0.782 & 279 & 15.3 $\pm$ 2.14 $\pm$ 1.51  \\
\hline

2.100 & 0.239 & 0.778 & 297 & 12.8 $\pm$ 1.70 $\pm$ 0.30  \\
\hline

2.101 & 0.239 & 0.779 & 315 & 16.2 $\pm$ 2.07 $\pm$ 0.99  \\
\hline

2.100 & 0.238 & 0.778 & 333 & 27.4 $\pm$ 6.13 $\pm$ 2.22  \\
\hline

2.101 & 0.239 & 1.220 & 9 & 3.35 $\pm$ 1.12 $\pm$ 0.25  \\
\hline

2.099 & 0.239 & 1.217 & 27 & 5.66 $\pm$ 1.13 $\pm$ 0.82  \\
\hline

2.100 & 0.238 & 1.218 & 45 & 4.80 $\pm$ 0.98 $\pm$ 0.47  \\
\hline

2.099 & 0.239 & 1.212 & 63 & 5.40 $\pm$ 1.13 $\pm$ 0.43  \\
\hline

2.097 & 0.239 & 1.209 & 81 & 8.41 $\pm$ 1.65 $\pm$ 0.56  \\
\hline

2.100 & 0.239 & 1.215 & 99 & 6.91 $\pm$ 3.09 $\pm$ 0.87  \\
\hline

2.097 & 0.239 & 1.211 & 279 & 6.99 $\pm$ 1.75 $\pm$ 2.58  \\
\hline

2.101 & 0.239 & 1.218 & 297 & 7.89 $\pm$ 1.26 $\pm$ 0.69  \\
\hline

2.102 & 0.239 & 1.216 & 315 & 6.72 $\pm$ 1.08 $\pm$ 1.23  \\
\hline

2.098 & 0.238 & 1.220 & 333 & 4.52 $\pm$ 1.10 $\pm$ 1.23  \\
\hline

2.102 & 0.239 & 1.218 & 351 & 6.03 $\pm$ 1.67 $\pm$ 1.20  \\
\hline

2.096 & 0.238 & 1.718 & 9 & 2.09 $\pm$ 0.63 $\pm$ 0.24  \\
\hline

2.098 & 0.239 & 1.729 & 27 & 2.10 $\pm$ 0.70 $\pm$ 0.39  \\
\hline

2.103 & 0.239 & 1.723 & 45 & 2.09 $\pm$ 0.85 $\pm$ 0.03  \\
\hline

2.099 & 0.238 & 1.712 & 63 & 5.01 $\pm$ 2.24 $\pm$ 0.74  \\
\hline

2.101 & 0.238 & 1.722 & 297 & 6.54 $\pm$ 2.67 $\pm$ 0.74  \\
\hline

2.104 & 0.238 & 1.728 & 333 & 3.29 $\pm$ 0.99 $\pm$ 0.53  \\
\hline

2.100 & 0.238 & 1.724 & 351 & 2.19 $\pm$ 0.77 $\pm$ 0.26  \\
\hline

2.205 & 0.275 & 0.122 & 9 & 34.1 $\pm$ 7.11 $\pm$ 7.95  \\
\hline

2.209 & 0.274 & 0.121 & 27 & 39.3 $\pm$ 6.07 $\pm$ 6.12  \\
\hline

2.206 & 0.275 & 0.122 & 45 & 31.7 $\pm$ 5.01 $\pm$ 0.32  \\
\hline

2.208 & 0.275 & 0.122 & 63 & 29.9 $\pm$ 6.23 $\pm$ 0.67  \\
\hline

2.206 & 0.275 & 0.122 & 81 & 59.0 $\pm$ 9.84 $\pm$ 9.96  \\
\hline

2.211 & 0.274 & 0.122 & 99 & 40.4 $\pm$ 9.27 $\pm$ 12.2  \\
\hline

2.209 & 0.275 & 0.122 & 117 & 32.8 $\pm$ 11.6 $\pm$ 4.79  \\
\hline

2.208 & 0.274 & 0.122 & 153 & 45.5 $\pm$ 18.6 $\pm$ 7.34  \\
\hline

2.213 & 0.274 & 0.122 & 207 & 50.9 $\pm$ 22.8 $\pm$ 24.2  \\
\hline

2.212 & 0.275 & 0.122 & 225 & 88.8 $\pm$ 33.6 $\pm$ 13.1  \\
\hline

2.205 & 0.274 & 0.122 & 261 & 32.5 $\pm$ 8.40 $\pm$ 6.69  \\
\hline

2.204 & 0.274 & 0.122 & 279 & 27.8 $\pm$ 6.94 $\pm$ 1.83  \\
\hline

2.211 & 0.275 & 0.122 & 297 & 32.8 $\pm$ 6.19 $\pm$ 3.44  \\
\hline

2.203 & 0.274 & 0.122 & 315 & 38.6 $\pm$ 5.95 $\pm$ 4.83  \\
\hline

2.208 & 0.274 & 0.122 & 333 & 27.8 $\pm$ 5.26 $\pm$ 2.97  \\
\hline

2.212 & 0.274 & 0.122 & 351 & 28.4 $\pm$ 6.19 $\pm$ 5.44  \\
\hline

2.212 & 0.276 & 0.175 & 9 & 39.7 $\pm$ 8.27 $\pm$ 8.02  \\
\hline

2.204 & 0.276 & 0.175 & 27 & 49.0 $\pm$ 7.57 $\pm$ 6.17  \\
\hline

2.210 & 0.276 & 0.175 & 45 & 37.7 $\pm$ 6.04 $\pm$ 8.09  \\
\hline

2.214 & 0.276 & 0.175 & 63 & 35.6 $\pm$ 6.11 $\pm$ 3.32  \\
\hline

2.209 & 0.276 & 0.176 & 81 & 48.3 $\pm$ 6.57 $\pm$ 7.38  \\
\hline

2.207 & 0.276 & 0.175 & 99 & 40.6 $\pm$ 6.43 $\pm$ 0.80  \\
\hline

2.202 & 0.276 & 0.175 & 117 & 35.3 $\pm$ 9.12 $\pm$ 8.93  \\
\hline

2.211 & 0.276 & 0.174 & 135 & 59.8 $\pm$ 14.9 $\pm$ 4.24  \\
\hline

2.211 & 0.276 & 0.175 & 153 & 34.2 $\pm$ 9.15 $\pm$ 6.33  \\
\hline

2.213 & 0.276 & 0.175 & 171 & 26.0 $\pm$ 10.6 $\pm$ 1.84  \\
\hline

2.214 & 0.276 & 0.175 & 189 & 49.8 $\pm$ 12.9 $\pm$ 3.29  \\
\hline

2.214 & 0.276 & 0.175 & 207 & 38.3 $\pm$ 11.0 $\pm$ 6.65  \\
\hline

2.213 & 0.276 & 0.175 & 225 & 73.0 $\pm$ 18.8 $\pm$ 7.79  \\
\hline

2.211 & 0.276 & 0.176 & 243 & 55.1 $\pm$ 10.8 $\pm$ 16.4  \\
\hline

2.204 & 0.276 & 0.175 & 261 & 52.8 $\pm$ 7.96 $\pm$ 5.26  \\
\hline

2.210 & 0.276 & 0.175 & 279 & 37.2 $\pm$ 6.29 $\pm$ 5.44  \\
\hline

2.212 & 0.276 & 0.175 & 297 & 41.9 $\pm$ 6.46 $\pm$ 4.02  \\
\hline

2.209 & 0.276 & 0.175 & 315 & 30.3 $\pm$ 5.36 $\pm$ 3.73  \\
\hline

2.212 & 0.277 & 0.175 & 333 & 38.9 $\pm$ 6.89 $\pm$ 3.47  \\
\hline

2.212 & 0.276 & 0.175 & 351 & 60.6 $\pm$ 11.1 $\pm$ 11.6  \\
\hline

2.208 & 0.276 & 0.248 & 9 & 42.3 $\pm$ 6.70 $\pm$ 5.43  \\
\hline

2.210 & 0.276 & 0.248 & 27 & 40.0 $\pm$ 4.92 $\pm$ 4.09  \\
\hline

2.208 & 0.276 & 0.248 & 45 & 44.9 $\pm$ 4.76 $\pm$ 3.48  \\
\hline

2.208 & 0.276 & 0.248 & 63 & 37.8 $\pm$ 4.15 $\pm$ 4.23  \\
\hline

2.207 & 0.276 & 0.249 & 81 & 45.6 $\pm$ 4.20 $\pm$ 1.59  \\
\hline

2.211 & 0.276 & 0.248 & 99 & 47.3 $\pm$ 4.45 $\pm$ 5.46  \\
\hline

2.212 & 0.276 & 0.248 & 117 & 41.3 $\pm$ 6.53 $\pm$ 3.45  \\
\hline

2.210 & 0.276 & 0.249 & 135 & 61.8 $\pm$ 11.3 $\pm$ 0.83  \\
\hline

2.209 & 0.276 & 0.249 & 153 & 49.1 $\pm$ 10.2 $\pm$ 7.49  \\
\hline

2.208 & 0.276 & 0.248 & 171 & 40.7 $\pm$ 10.9 $\pm$ 2.31  \\
\hline

2.212 & 0.276 & 0.248 & 189 & 28.6 $\pm$ 9.04 $\pm$ 4.28  \\
\hline

2.209 & 0.276 & 0.250 & 207 & 57.8 $\pm$ 12.3 $\pm$ 14.5  \\
\hline

2.212 & 0.276 & 0.248 & 225 & 32.8 $\pm$ 8.22 $\pm$ 1.90  \\
\hline

2.212 & 0.276 & 0.249 & 243 & 47.7 $\pm$ 6.56 $\pm$ 2.77  \\
\hline

2.207 & 0.276 & 0.250 & 261 & 44.4 $\pm$ 4.68 $\pm$ 1.46  \\
\hline

2.210 & 0.276 & 0.248 & 279 & 59.7 $\pm$ 5.64 $\pm$ 6.05  \\
\hline

2.208 & 0.276 & 0.248 & 297 & 41.6 $\pm$ 4.31 $\pm$ 5.89  \\
\hline

2.207 & 0.276 & 0.249 & 315 & 43.4 $\pm$ 4.30 $\pm$ 1.42  \\
\hline

2.212 & 0.276 & 0.249 & 333 & 40.1 $\pm$ 5.35 $\pm$ 15.4  \\
\hline

2.212 & 0.276 & 0.249 & 351 & 33.6 $\pm$ 6.47 $\pm$ 6.99  \\
\hline

2.212 & 0.276 & 0.349 & 9 & 24.9 $\pm$ 8.31 $\pm$ 5.23  \\
\hline

2.211 & 0.276 & 0.349 & 27 & 46.5 $\pm$ 6.44 $\pm$ 7.13  \\
\hline

2.213 & 0.276 & 0.349 & 45 & 39.2 $\pm$ 4.28 $\pm$ 0.40  \\
\hline

2.207 & 0.276 & 0.349 & 63 & 47.9 $\pm$ 4.36 $\pm$ 1.32  \\
\hline

2.209 & 0.276 & 0.350 & 81 & 48.3 $\pm$ 4.09 $\pm$ 2.36  \\
\hline

2.210 & 0.276 & 0.349 & 99 & 44.5 $\pm$ 4.32 $\pm$ 3.39  \\
\hline

2.210 & 0.276 & 0.350 & 117 & 35.5 $\pm$ 5.47 $\pm$ 1.06  \\
\hline

2.211 & 0.276 & 0.348 & 135 & 37.4 $\pm$ 8.16 $\pm$ 2.86  \\
\hline

2.209 & 0.276 & 0.349 & 153 & 34.3 $\pm$ 10.3 $\pm$ 11.5  \\
\hline

2.206 & 0.276 & 0.349 & 189 & 20.7 $\pm$ 9.25 $\pm$ 4.93  \\
\hline

2.210 & 0.276 & 0.349 & 207 & 38.1 $\pm$ 13.5 $\pm$ 18.0  \\
\hline

2.210 & 0.276 & 0.349 & 225 & 41.8 $\pm$ 10.8 $\pm$ 7.03  \\
\hline

2.210 & 0.276 & 0.349 & 243 & 37.3 $\pm$ 5.63 $\pm$ 2.15  \\
\hline

2.210 & 0.276 & 0.350 & 261 & 44.5 $\pm$ 4.72 $\pm$ 4.36  \\
\hline

2.209 & 0.276 & 0.350 & 279 & 46.3 $\pm$ 4.74 $\pm$ 3.37  \\
\hline

2.212 & 0.276 & 0.349 & 297 & 44.2 $\pm$ 3.91 $\pm$ 2.93  \\
\hline

2.209 & 0.276 & 0.349 & 315 & 41.0 $\pm$ 3.74 $\pm$ 2.37  \\
\hline

2.210 & 0.276 & 0.350 & 333 & 47.5 $\pm$ 6.66 $\pm$ 4.85  \\
\hline

2.209 & 0.276 & 0.498 & 27 & 42.1 $\pm$ 5.68 $\pm$ 2.45  \\
\hline

2.214 & 0.276 & 0.496 & 45 & 38.2 $\pm$ 3.04 $\pm$ 2.29  \\
\hline

2.209 & 0.276 & 0.495 & 63 & 36.2 $\pm$ 2.53 $\pm$ 1.24  \\
\hline

2.212 & 0.276 & 0.498 & 81 & 33.3 $\pm$ 2.37 $\pm$ 1.98  \\
\hline

2.208 & 0.276 & 0.497 & 99 & 32.3 $\pm$ 2.91 $\pm$ 1.71  \\
\hline

2.209 & 0.276 & 0.496 & 117 & 29.6 $\pm$ 4.32 $\pm$ 1.56  \\
\hline

2.211 & 0.276 & 0.496 & 135 & 20.5 $\pm$ 6.20 $\pm$ 5.25  \\
\hline

2.212 & 0.276 & 0.495 & 153 & 41.2 $\pm$ 11.0 $\pm$ 11.1  \\
\hline

2.210 & 0.276 & 0.493 & 171 & 13.4 $\pm$ 6.00 $\pm$ 4.25  \\
\hline

2.211 & 0.276 & 0.493 & 189 & 29.5 $\pm$ 6.78 $\pm$ 6.13  \\
\hline

2.210 & 0.277 & 0.494 & 207 & 16.1 $\pm$ 5.71 $\pm$ 6.14  \\
\hline

2.210 & 0.277 & 0.495 & 225 & 29.7 $\pm$ 7.94 $\pm$ 6.12  \\
\hline

2.213 & 0.276 & 0.498 & 243 & 29.7 $\pm$ 4.33 $\pm$ 3.28  \\
\hline

2.209 & 0.276 & 0.497 & 261 & 36.8 $\pm$ 3.30 $\pm$ 2.40  \\
\hline

2.210 & 0.276 & 0.497 & 279 & 38.0 $\pm$ 2.83 $\pm$ 2.26  \\
\hline

2.212 & 0.276 & 0.497 & 297 & 37.0 $\pm$ 2.34 $\pm$ 1.85  \\
\hline

2.209 & 0.276 & 0.497 & 315 & 34.4 $\pm$ 2.40 $\pm$ 3.06  \\
\hline

2.210 & 0.276 & 0.496 & 333 & 30.7 $\pm$ 4.80 $\pm$ 3.42  \\
\hline

2.209 & 0.277 & 0.779 & 27 & 13.2 $\pm$ 1.99 $\pm$ 1.01  \\
\hline

2.207 & 0.276 & 0.780 & 45 & 17.0 $\pm$ 1.28 $\pm$ 0.73  \\
\hline

2.207 & 0.277 & 0.780 & 63 & 22.9 $\pm$ 1.41 $\pm$ 0.32  \\
\hline

2.206 & 0.277 & 0.781 & 81 & 20.6 $\pm$ 1.43 $\pm$ 0.66  \\
\hline

2.209 & 0.277 & 0.781 & 99 & 20.7 $\pm$ 2.29 $\pm$ 0.66  \\
\hline

2.208 & 0.277 & 0.780 & 117 & 12.1 $\pm$ 3.82 $\pm$ 1.29  \\
\hline

2.212 & 0.277 & 0.780 & 135 & 18.7 $\pm$ 5.65 $\pm$ 3.25  \\
\hline

2.210 & 0.277 & 0.779 & 153 & 21.4 $\pm$ 4.47 $\pm$ 2.21  \\
\hline

2.211 & 0.276 & 0.778 & 171 & 9.64 $\pm$ 2.27 $\pm$ 1.92  \\
\hline

2.214 & 0.277 & 0.779 & 189 & 8.07 $\pm$ 1.55 $\pm$ 2.49  \\
\hline

2.211 & 0.277 & 0.778 & 207 & 16.1 $\pm$ 2.80 $\pm$ 2.40  \\
\hline

2.208 & 0.276 & 0.778 & 225 & 24.2 $\pm$ 5.87 $\pm$ 0.50  \\
\hline

2.208 & 0.277 & 0.778 & 243 & 23.6 $\pm$ 5.14 $\pm$ 2.76  \\
\hline

2.207 & 0.277 & 0.782 & 261 & 21.6 $\pm$ 2.62 $\pm$ 0.95  \\
\hline

2.209 & 0.277 & 0.781 & 279 & 20.2 $\pm$ 1.69 $\pm$ 0.78  \\
\hline

2.206 & 0.276 & 0.781 & 297 & 17.7 $\pm$ 1.11 $\pm$ 0.75  \\
\hline

2.208 & 0.277 & 0.780 & 315 & 17.1 $\pm$ 1.10 $\pm$ 0.28  \\
\hline

2.210 & 0.277 & 0.779 & 333 & 17.1 $\pm$ 2.44 $\pm$ 2.76  \\
\hline

2.207 & 0.277 & 1.218 & 9 & 7.34 $\pm$ 1.60 $\pm$ 1.28  \\
\hline

2.207 & 0.277 & 1.220 & 27 & 7.38 $\pm$ 0.80 $\pm$ 0.40  \\
\hline

2.212 & 0.277 & 1.218 & 45 & 8.31 $\pm$ 0.79 $\pm$ 0.32  \\
\hline

2.211 & 0.277 & 1.217 & 63 & 9.77 $\pm$ 0.98 $\pm$ 0.18  \\
\hline

2.208 & 0.277 & 1.217 & 81 & 10.2 $\pm$ 1.63 $\pm$ 0.88  \\
\hline

2.210 & 0.277 & 1.215 & 99 & 12.0 $\pm$ 3.32 $\pm$ 2.54  \\
\hline

2.211 & 0.277 & 1.218 & 117 & 6.79 $\pm$ 1.96 $\pm$ 1.41  \\
\hline

2.211 & 0.277 & 1.218 & 135 & 6.83 $\pm$ 1.97 $\pm$ 0.79  \\
\hline

2.210 & 0.276 & 1.223 & 153 & 9.35 $\pm$ 2.14 $\pm$ 1.25  \\
\hline

2.211 & 0.277 & 1.222 & 171 & 4.37 $\pm$ 1.26 $\pm$ 0.40  \\
\hline

2.218 & 0.277 & 1.221 & 189 & 5.48 $\pm$ 1.14 $\pm$ 1.05  \\
\hline

2.211 & 0.277 & 1.223 & 207 & 6.41 $\pm$ 1.47 $\pm$ 1.64  \\
\hline

2.211 & 0.277 & 1.217 & 225 & 7.66 $\pm$ 2.05 $\pm$ 1.66  \\
\hline

2.207 & 0.277 & 1.220 & 243 & 7.48 $\pm$ 2.64 $\pm$ 0.60  \\
\hline

2.204 & 0.277 & 1.219 & 279 & 10.4 $\pm$ 1.96 $\pm$ 0.59  \\
\hline

2.210 & 0.277 & 1.217 & 297 & 9.16 $\pm$ 0.91 $\pm$ 0.51  \\
\hline

2.209 & 0.277 & 1.216 & 315 & 8.51 $\pm$ 0.72 $\pm$ 0.53  \\
\hline

2.212 & 0.277 & 1.217 & 333 & 8.68 $\pm$ 1.00 $\pm$ 0.70  \\
\hline

2.210 & 0.277 & 1.214 & 351 & 10.8 $\pm$ 2.20 $\pm$ 1.33  \\
\hline

2.211 & 0.277 & 1.723 & 9 & 2.27 $\pm$ 0.43 $\pm$ 0.10  \\
\hline

2.209 & 0.277 & 1.718 & 27 & 2.38 $\pm$ 0.41 $\pm$ 0.17  \\
\hline

2.210 & 0.278 & 1.721 & 45 & 4.28 $\pm$ 0.87 $\pm$ 0.81  \\
\hline

2.211 & 0.277 & 1.713 & 81 & 6.39 $\pm$ 2.02 $\pm$ 0.44  \\
\hline

2.210 & 0.277 & 1.718 & 99 & 4.10 $\pm$ 0.84 $\pm$ 0.67  \\
\hline

2.215 & 0.278 & 1.721 & 117 & 2.15 $\pm$ 0.72 $\pm$ 0.13  \\
\hline

2.214 & 0.277 & 1.723 & 135 & 5.22 $\pm$ 1.31 $\pm$ 0.36  \\
\hline

2.211 & 0.277 & 1.721 & 189 & 2.92 $\pm$ 0.81 $\pm$ 0.53  \\
\hline

2.214 & 0.277 & 1.720 & 207 & 2.40 $\pm$ 0.98 $\pm$ 0.86  \\
\hline

2.209 & 0.277 & 1.715 & 243 & 5.93 $\pm$ 1.48 $\pm$ 0.80  \\
\hline

2.208 & 0.277 & 1.715 & 261 & 5.41 $\pm$ 1.50 $\pm$ 0.88  \\
\hline

2.209 & 0.277 & 1.714 & 279 & 3.78 $\pm$ 1.54 $\pm$ 1.67  \\
\hline

2.212 & 0.278 & 1.716 & 315 & 2.85 $\pm$ 0.64 $\pm$ 0.82  \\
\hline

2.215 & 0.277 & 1.720 & 333 & 3.64 $\pm$ 0.60 $\pm$ 0.15  \\
\hline

2.212 & 0.277 & 1.722 & 351 & 3.42 $\pm$ 0.59 $\pm$ 0.38  \\
\hline

2.219 & 0.316 & 0.136 & 27 & 66.1 $\pm$ 17.1 $\pm$ 7.94  \\
\hline

2.233 & 0.316 & 0.136 & 45 & 44.7 $\pm$ 16.9 $\pm$ 3.60  \\
\hline

2.222 & 0.315 & 0.136 & 315 & 75.7 $\pm$ 22.8 $\pm$ 18.8  \\
\hline

2.224 & 0.315 & 0.135 & 333 & 53.6 $\pm$ 17.9 $\pm$ 12.3  \\
\hline

2.238 & 0.332 & 0.177 & 9 & 45.4 $\pm$ 7.36 $\pm$ 2.89  \\
\hline

2.235 & 0.332 & 0.177 & 27 & 42.8 $\pm$ 6.69 $\pm$ 4.64  \\
\hline

2.236 & 0.332 & 0.177 & 45 & 60.8 $\pm$ 8.97 $\pm$ 4.69  \\
\hline

2.237 & 0.332 & 0.177 & 63 & 61.8 $\pm$ 12.6 $\pm$ 10.6  \\
\hline

2.241 & 0.332 & 0.177 & 81 & 64.8 $\pm$ 18.7 $\pm$ 11.4  \\
\hline

2.236 & 0.331 & 0.176 & 99 & 50.4 $\pm$ 15.9 $\pm$ 19.7  \\
\hline

2.237 & 0.332 & 0.176 & 117 & 39.8 $\pm$ 13.3 $\pm$ 2.41  \\
\hline

2.234 & 0.333 & 0.177 & 135 & 84.0 $\pm$ 34.3 $\pm$ 8.23  \\
\hline

2.238 & 0.332 & 0.177 & 243 & 69.4 $\pm$ 18.5 $\pm$ 17.5  \\
\hline

2.237 & 0.332 & 0.177 & 261 & 102. $\pm$ 26.4 $\pm$ 7.86  \\
\hline

2.233 & 0.332 & 0.177 & 279 & 75.1 $\pm$ 18.2 $\pm$ 32.0  \\
\hline

2.237 & 0.333 & 0.176 & 297 & 74.1 $\pm$ 12.0 $\pm$ 16.1  \\
\hline

2.235 & 0.332 & 0.177 & 315 & 41.9 $\pm$ 7.19 $\pm$ 1.74  \\
\hline

2.237 & 0.332 & 0.176 & 333 & 56.0 $\pm$ 8.75 $\pm$ 9.86  \\
\hline

2.235 & 0.331 & 0.177 & 351 & 51.5 $\pm$ 8.35 $\pm$ 1.84  \\
\hline

2.242 & 0.337 & 0.249 & 9 & 57.6 $\pm$ 4.72 $\pm$ 5.02  \\
\hline

2.242 & 0.337 & 0.249 & 27 & 61.5 $\pm$ 4.61 $\pm$ 4.72  \\
\hline

2.239 & 0.337 & 0.249 & 45 & 64.7 $\pm$ 5.32 $\pm$ 7.02  \\
\hline

2.241 & 0.336 & 0.249 & 63 & 70.7 $\pm$ 7.14 $\pm$ 3.36  \\
\hline

2.243 & 0.336 & 0.249 & 81 & 79.3 $\pm$ 9.92 $\pm$ 4.88  \\
\hline

2.243 & 0.337 & 0.249 & 99 & 96.7 $\pm$ 15.5 $\pm$ 5.48  \\
\hline

2.244 & 0.337 & 0.250 & 117 & 49.7 $\pm$ 12.4 $\pm$ 11.3  \\
\hline

2.241 & 0.337 & 0.250 & 135 & 64.9 $\pm$ 15.7 $\pm$ 9.36  \\
\hline

2.243 & 0.337 & 0.249 & 153 & 55.7 $\pm$ 15.4 $\pm$ 6.52  \\
\hline

2.244 & 0.337 & 0.250 & 207 & 51.3 $\pm$ 18.1 $\pm$ 10.9  \\
\hline

2.243 & 0.337 & 0.249 & 225 & 72.3 $\pm$ 13.0 $\pm$ 7.59  \\
\hline

2.243 & 0.337 & 0.249 & 243 & 72.2 $\pm$ 11.7 $\pm$ 10.3  \\
\hline

2.240 & 0.337 & 0.249 & 261 & 87.4 $\pm$ 17.5 $\pm$ 8.64  \\
\hline

2.245 & 0.337 & 0.249 & 279 & 49.8 $\pm$ 8.08 $\pm$ 2.77  \\
\hline

2.241 & 0.337 & 0.249 & 297 & 62.1 $\pm$ 5.82 $\pm$ 7.57  \\
\hline

2.239 & 0.337 & 0.249 & 315 & 56.5 $\pm$ 4.65 $\pm$ 4.36  \\
\hline

2.241 & 0.336 & 0.249 & 333 & 52.1 $\pm$ 4.79 $\pm$ 4.38  \\
\hline

2.243 & 0.337 & 0.249 & 351 & 56.0 $\pm$ 5.03 $\pm$ 4.93  \\
\hline

2.244 & 0.337 & 0.349 & 9 & 50.8 $\pm$ 3.92 $\pm$ 6.94  \\
\hline

2.241 & 0.337 & 0.349 & 27 & 48.6 $\pm$ 3.50 $\pm$ 3.78  \\
\hline

2.238 & 0.337 & 0.350 & 45 & 63.2 $\pm$ 4.65 $\pm$ 2.78  \\
\hline

2.239 & 0.337 & 0.349 & 63 & 67.4 $\pm$ 5.78 $\pm$ 3.20  \\
\hline

2.244 & 0.337 & 0.349 & 81 & 63.5 $\pm$ 7.43 $\pm$ 13.5  \\
\hline

2.240 & 0.337 & 0.349 & 99 & 55.4 $\pm$ 13.1 $\pm$ 5.44  \\
\hline

2.245 & 0.337 & 0.349 & 117 & 62.6 $\pm$ 19.8 $\pm$ 8.37  \\
\hline

2.240 & 0.337 & 0.349 & 135 & 65.8 $\pm$ 13.2 $\pm$ 8.29  \\
\hline

2.246 & 0.337 & 0.349 & 153 & 39.5 $\pm$ 9.30 $\pm$ 4.96  \\
\hline

2.245 & 0.337 & 0.350 & 171 & 29.7 $\pm$ 13.3 $\pm$ 4.86  \\
\hline

2.245 & 0.337 & 0.349 & 189 & 30.1 $\pm$ 8.68 $\pm$ 0.84  \\
\hline

2.248 & 0.337 & 0.349 & 207 & 29.0 $\pm$ 8.73 $\pm$ 3.27  \\
\hline

2.241 & 0.337 & 0.349 & 225 & 61.5 $\pm$ 9.28 $\pm$ 3.26  \\
\hline

2.244 & 0.336 & 0.350 & 243 & 56.0 $\pm$ 9.75 $\pm$ 7.51  \\
\hline

2.244 & 0.338 & 0.349 & 261 & 90.0 $\pm$ 18.4 $\pm$ 28.6  \\
\hline

2.241 & 0.337 & 0.349 & 279 & 62.9 $\pm$ 8.18 $\pm$ 3.87  \\
\hline

2.241 & 0.337 & 0.349 & 297 & 71.9 $\pm$ 5.42 $\pm$ 4.17  \\
\hline

2.242 & 0.337 & 0.349 & 315 & 66.4 $\pm$ 4.45 $\pm$ 4.36  \\
\hline

2.240 & 0.337 & 0.350 & 333 & 55.7 $\pm$ 4.38 $\pm$ 2.05  \\
\hline

2.242 & 0.337 & 0.349 & 351 & 51.9 $\pm$ 4.48 $\pm$ 2.46  \\
\hline

2.243 & 0.337 & 0.498 & 9 & 38.0 $\pm$ 2.77 $\pm$ 1.97  \\
\hline

2.243 & 0.338 & 0.497 & 27 & 48.3 $\pm$ 2.57 $\pm$ 2.13  \\
\hline

2.242 & 0.337 & 0.498 & 45 & 54.1 $\pm$ 2.94 $\pm$ 2.10  \\
\hline

2.239 & 0.337 & 0.497 & 63 & 55.7 $\pm$ 3.65 $\pm$ 1.49  \\
\hline

2.241 & 0.337 & 0.498 & 81 & 55.7 $\pm$ 4.94 $\pm$ 1.72  \\
\hline

2.241 & 0.337 & 0.497 & 99 & 50.1 $\pm$ 10.2 $\pm$ 3.18  \\
\hline

2.241 & 0.337 & 0.497 & 117 & 22.7 $\pm$ 8.57 $\pm$ 4.43  \\
\hline

2.245 & 0.337 & 0.496 & 135 & 49.2 $\pm$ 6.01 $\pm$ 8.58  \\
\hline

2.242 & 0.338 & 0.496 & 153 & 28.1 $\pm$ 3.79 $\pm$ 5.13  \\
\hline

2.244 & 0.338 & 0.494 & 171 & 38.0 $\pm$ 6.43 $\pm$ 4.27  \\
\hline

2.245 & 0.338 & 0.493 & 189 & 23.7 $\pm$ 3.50 $\pm$ 4.68  \\
\hline

2.243 & 0.338 & 0.495 & 207 & 36.7 $\pm$ 5.14 $\pm$ 5.07  \\
\hline

2.244 & 0.337 & 0.497 & 225 & 56.8 $\pm$ 5.39 $\pm$ 14.6  \\
\hline

2.243 & 0.338 & 0.497 & 243 & 64.1 $\pm$ 6.95 $\pm$ 9.08  \\
\hline

2.242 & 0.337 & 0.497 & 261 & 58.5 $\pm$ 11.7 $\pm$ 15.6  \\
\hline

2.239 & 0.337 & 0.497 & 279 & 60.2 $\pm$ 6.31 $\pm$ 4.79  \\
\hline

2.241 & 0.337 & 0.497 & 297 & 54.5 $\pm$ 3.20 $\pm$ 2.42  \\
\hline

2.242 & 0.337 & 0.498 & 315 & 52.8 $\pm$ 2.57 $\pm$ 1.05  \\
\hline

2.240 & 0.337 & 0.497 & 333 & 43.8 $\pm$ 2.74 $\pm$ 2.16  \\
\hline

2.242 & 0.337 & 0.497 & 351 & 35.2 $\pm$ 3.03 $\pm$ 5.47  \\
\hline

2.243 & 0.338 & 0.780 & 9 & 21.0 $\pm$ 2.64 $\pm$ 2.77  \\
\hline

2.241 & 0.338 & 0.783 & 27 & 27.0 $\pm$ 1.50 $\pm$ 2.02  \\
\hline

2.241 & 0.338 & 0.784 & 45 & 34.0 $\pm$ 1.63 $\pm$ 2.38  \\
\hline

2.241 & 0.338 & 0.787 & 63 & 37.6 $\pm$ 2.27 $\pm$ 1.02  \\
\hline

2.240 & 0.338 & 0.788 & 81 & 35.7 $\pm$ 3.71 $\pm$ 1.38  \\
\hline

2.240 & 0.337 & 0.790 & 99 & 26.6 $\pm$ 4.93 $\pm$ 3.07  \\
\hline

2.242 & 0.338 & 0.787 & 117 & 32.7 $\pm$ 4.12 $\pm$ 6.67  \\
\hline

2.241 & 0.338 & 0.782 & 135 & 32.8 $\pm$ 3.27 $\pm$ 2.35  \\
\hline

2.242 & 0.338 & 0.780 & 153 & 29.4 $\pm$ 2.46 $\pm$ 3.16  \\
\hline

2.247 & 0.338 & 0.780 & 171 & 29.0 $\pm$ 3.46 $\pm$ 3.72  \\
\hline

2.243 & 0.338 & 0.782 & 189 & 20.0 $\pm$ 2.04 $\pm$ 3.44  \\
\hline

2.243 & 0.338 & 0.778 & 207 & 33.3 $\pm$ 3.13 $\pm$ 3.86  \\
\hline

2.242 & 0.338 & 0.782 & 225 & 35.7 $\pm$ 2.62 $\pm$ 3.81  \\
\hline

2.244 & 0.338 & 0.785 & 243 & 37.1 $\pm$ 3.45 $\pm$ 4.20  \\
\hline

2.241 & 0.338 & 0.788 & 261 & 43.3 $\pm$ 9.02 $\pm$ 2.40  \\
\hline

2.241 & 0.337 & 0.790 & 279 & 44.9 $\pm$ 5.33 $\pm$ 1.44  \\
\hline

2.242 & 0.338 & 0.787 & 297 & 36.7 $\pm$ 2.00 $\pm$ 1.56  \\
\hline

2.240 & 0.338 & 0.785 & 315 & 29.4 $\pm$ 1.38 $\pm$ 0.81  \\
\hline

2.242 & 0.338 & 0.783 & 333 & 29.0 $\pm$ 1.75 $\pm$ 2.49  \\
\hline

2.242 & 0.338 & 0.781 & 351 & 24.1 $\pm$ 3.38 $\pm$ 3.90  \\
\hline

2.243 & 0.339 & 1.224 & 9 & 13.2 $\pm$ 3.31 $\pm$ 1.35  \\
\hline

2.241 & 0.339 & 1.222 & 27 & 12.3 $\pm$ 0.90 $\pm$ 0.47  \\
\hline

2.242 & 0.339 & 1.221 & 45 & 14.3 $\pm$ 1.04 $\pm$ 0.84  \\
\hline

2.243 & 0.339 & 1.221 & 63 & 18.5 $\pm$ 1.99 $\pm$ 0.61  \\
\hline

2.241 & 0.339 & 1.223 & 81 & 25.5 $\pm$ 3.84 $\pm$ 0.91  \\
\hline

2.241 & 0.339 & 1.220 & 99 & 21.1 $\pm$ 1.65 $\pm$ 1.11  \\
\hline

2.244 & 0.339 & 1.221 & 117 & 25.1 $\pm$ 2.11 $\pm$ 1.93  \\
\hline

2.242 & 0.339 & 1.222 & 135 & 20.5 $\pm$ 2.50 $\pm$ 0.70  \\
\hline

2.243 & 0.339 & 1.222 & 153 & 19.2 $\pm$ 1.89 $\pm$ 2.35  \\
\hline

2.245 & 0.339 & 1.224 & 171 & 11.9 $\pm$ 2.04 $\pm$ 0.46  \\
\hline

2.247 & 0.339 & 1.221 & 189 & 13.4 $\pm$ 1.62 $\pm$ 2.38  \\
\hline

2.244 & 0.339 & 1.222 & 207 & 20.6 $\pm$ 2.29 $\pm$ 3.25  \\
\hline

2.241 & 0.339 & 1.221 & 225 & 22.1 $\pm$ 1.88 $\pm$ 0.57  \\
\hline

2.241 & 0.339 & 1.223 & 243 & 21.7 $\pm$ 2.69 $\pm$ 0.78  \\
\hline

2.241 & 0.339 & 1.219 & 261 & 24.3 $\pm$ 2.55 $\pm$ 3.33  \\
\hline

2.241 & 0.339 & 1.222 & 279 & 17.9 $\pm$ 3.90 $\pm$ 0.18  \\
\hline

2.240 & 0.339 & 1.221 & 297 & 17.1 $\pm$ 1.74 $\pm$ 0.65  \\
\hline

2.242 & 0.339 & 1.221 & 315 & 15.7 $\pm$ 1.04 $\pm$ 0.85  \\
\hline

2.242 & 0.339 & 1.221 & 333 & 12.7 $\pm$ 1.05 $\pm$ 0.44  \\
\hline

2.243 & 0.339 & 1.223 & 351 & 6.63 $\pm$ 2.97 $\pm$ 0.61  \\
\hline

2.246 & 0.340 & 1.723 & 9 & 3.59 $\pm$ 0.61 $\pm$ 0.21  \\
\hline

2.246 & 0.340 & 1.726 & 27 & 5.00 $\pm$ 0.59 $\pm$ 0.37  \\
\hline

2.243 & 0.339 & 1.721 & 45 & 6.03 $\pm$ 1.10 $\pm$ 0.58  \\
\hline

2.243 & 0.340 & 1.720 & 63 & 14.2 $\pm$ 4.74 $\pm$ 1.25  \\
\hline

2.241 & 0.340 & 1.719 & 81 & 12.2 $\pm$ 1.10 $\pm$ 0.98  \\
\hline

2.246 & 0.341 & 1.719 & 99 & 11.1 $\pm$ 0.87 $\pm$ 0.68  \\
\hline

2.245 & 0.340 & 1.723 & 117 & 12.1 $\pm$ 1.29 $\pm$ 0.77  \\
\hline

2.243 & 0.340 & 1.723 & 135 & 11.9 $\pm$ 2.03 $\pm$ 1.23  \\
\hline

2.244 & 0.340 & 1.725 & 153 & 10.6 $\pm$ 1.88 $\pm$ 1.02  \\
\hline

2.246 & 0.339 & 1.727 & 171 & 8.21 $\pm$ 2.74 $\pm$ 1.61  \\
\hline

2.241 & 0.339 & 1.722 & 189 & 5.60 $\pm$ 1.45 $\pm$ 1.31  \\
\hline

2.245 & 0.339 & 1.725 & 207 & 4.14 $\pm$ 1.31 $\pm$ 0.84  \\
\hline

2.245 & 0.340 & 1.721 & 225 & 11.2 $\pm$ 1.49 $\pm$ 1.37  \\
\hline

2.242 & 0.340 & 1.721 & 243 & 10.7 $\pm$ 1.99 $\pm$ 1.64  \\
\hline

2.242 & 0.340 & 1.720 & 261 & 8.14 $\pm$ 0.99 $\pm$ 0.93  \\
\hline

2.243 & 0.340 & 1.720 & 279 & 10.7 $\pm$ 1.06 $\pm$ 0.58  \\
\hline

2.243 & 0.341 & 1.723 & 297 & 13.1 $\pm$ 3.64 $\pm$ 1.05  \\
\hline

2.243 & 0.340 & 1.721 & 315 & 7.65 $\pm$ 1.28 $\pm$ 0.30  \\
\hline

2.240 & 0.340 & 1.721 & 333 & 5.01 $\pm$ 0.68 $\pm$ 1.01  \\
\hline

2.243 & 0.340 & 1.725 & 351 & 2.90 $\pm$ 0.58 $\pm$ 0.59  \\
\hline

2.334 & 0.400 & 0.257 & 9 & 65.4 $\pm$ 16.9 $\pm$ 6.22  \\
\hline

2.331 & 0.400 & 0.256 & 27 & 87.5 $\pm$ 21.2 $\pm$ 9.82  \\
\hline

2.332 & 0.400 & 0.257 & 45 & 112. $\pm$ 31.0 $\pm$ 7.18  \\
\hline

2.334 & 0.400 & 0.257 & 63 & 80.8 $\pm$ 30.5 $\pm$ 8.55  \\
\hline

2.334 & 0.400 & 0.255 & 99 & 67.0 $\pm$ 29.9 $\pm$ 31.0  \\
\hline

2.333 & 0.399 & 0.255 & 261 & 62.5 $\pm$ 23.6 $\pm$ 35.2  \\
\hline

2.330 & 0.400 & 0.258 & 279 & 64.9 $\pm$ 18.0 $\pm$ 10.5  \\
\hline

2.329 & 0.400 & 0.257 & 297 & 127. $\pm$ 34.1 $\pm$ 16.9  \\
\hline

2.338 & 0.400 & 0.257 & 315 & 66.4 $\pm$ 27.1 $\pm$ 4.41  \\
\hline

2.334 & 0.400 & 0.257 & 333 & 66.4 $\pm$ 23.5 $\pm$ 13.9  \\
\hline

2.331 & 0.400 & 0.256 & 351 & 47.1 $\pm$ 16.7 $\pm$ 7.57  \\
\hline

2.342 & 0.403 & 0.349 & 9 & 68.2 $\pm$ 10.2 $\pm$ 15.8  \\
\hline

2.338 & 0.403 & 0.350 & 27 & 77.3 $\pm$ 11.4 $\pm$ 4.27  \\
\hline

2.337 & 0.403 & 0.348 & 45 & 120. $\pm$ 21.5 $\pm$ 17.7  \\
\hline

2.345 & 0.403 & 0.350 & 63 & 118. $\pm$ 48.1 $\pm$ 10.2  \\
\hline

2.344 & 0.404 & 0.349 & 81 & 94.2 $\pm$ 42.1 $\pm$ 4.31  \\
\hline

2.335 & 0.403 & 0.349 & 99 & 108. $\pm$ 25.5 $\pm$ 9.58  \\
\hline

2.341 & 0.403 & 0.349 & 117 & 56.5 $\pm$ 15.7 $\pm$ 8.47  \\
\hline

2.341 & 0.403 & 0.350 & 225 & 97.1 $\pm$ 30.7 $\pm$ 26.7  \\
\hline

2.342 & 0.403 & 0.349 & 243 & 83.7 $\pm$ 18.7 $\pm$ 8.32  \\
\hline

2.341 & 0.404 & 0.350 & 261 & 87.7 $\pm$ 23.4 $\pm$ 6.07  \\
\hline

2.341 & 0.404 & 0.349 & 279 & 64.0 $\pm$ 21.3 $\pm$ 13.0  \\
\hline

2.344 & 0.403 & 0.350 & 297 & 86.6 $\pm$ 32.7 $\pm$ 29.9  \\
\hline

2.344 & 0.403 & 0.349 & 315 & 57.7 $\pm$ 12.9 $\pm$ 15.5  \\
\hline

2.339 & 0.404 & 0.349 & 333 & 55.1 $\pm$ 10.4 $\pm$ 10.3  \\
\hline

2.342 & 0.403 & 0.349 & 351 & 89.6 $\pm$ 12.3 $\pm$ 1.71  \\
\hline

2.342 & 0.403 & 0.498 & 9 & 68.7 $\pm$ 5.22 $\pm$ 4.57  \\
\hline

2.342 & 0.404 & 0.499 & 27 & 66.7 $\pm$ 5.55 $\pm$ 2.17  \\
\hline

2.343 & 0.403 & 0.498 & 45 & 83.3 $\pm$ 8.99 $\pm$ 3.65  \\
\hline

2.340 & 0.403 & 0.499 & 63 & 54.4 $\pm$ 15.1 $\pm$ 1.47  \\
\hline

2.341 & 0.403 & 0.497 & 99 & 80.0 $\pm$ 17.9 $\pm$ 11.7  \\
\hline

2.345 & 0.404 & 0.498 & 117 & 126. $\pm$ 20.2 $\pm$ 9.79  \\
\hline

2.343 & 0.403 & 0.497 & 135 & 69.1 $\pm$ 14.1 $\pm$ 4.54  \\
\hline

2.342 & 0.404 & 0.495 & 207 & 96.4 $\pm$ 34.1 $\pm$ 5.76  \\
\hline

2.345 & 0.404 & 0.499 & 225 & 75.2 $\pm$ 8.80 $\pm$ 10.6  \\
\hline

2.343 & 0.404 & 0.498 & 243 & 82.5 $\pm$ 9.93 $\pm$ 11.1  \\
\hline

2.343 & 0.403 & 0.497 & 261 & 68.8 $\pm$ 15.8 $\pm$ 9.97  \\
\hline

2.343 & 0.403 & 0.498 & 297 & 80.8 $\pm$ 16.5 $\pm$ 8.24  \\
\hline

2.342 & 0.403 & 0.501 & 315 & 66.9 $\pm$ 7.26 $\pm$ 2.33  \\
\hline

2.343 & 0.404 & 0.498 & 333 & 71.5 $\pm$ 6.64 $\pm$ 3.03  \\
\hline

2.340 & 0.403 & 0.499 & 351 & 70.2 $\pm$ 6.13 $\pm$ 6.32  \\
\hline

2.344 & 0.404 & 0.784 & 9 & 40.5 $\pm$ 3.23 $\pm$ 2.44  \\
\hline

2.344 & 0.404 & 0.789 & 27 & 50.2 $\pm$ 3.13 $\pm$ 1.42  \\
\hline

2.345 & 0.403 & 0.791 & 45 & 60.9 $\pm$ 4.63 $\pm$ 3.20  \\
\hline

2.340 & 0.403 & 0.787 & 63 & 69.1 $\pm$ 10.7 $\pm$ 5.88  \\
\hline

2.340 & 0.403 & 0.792 & 99 & 67.1 $\pm$ 8.33 $\pm$ 7.37  \\
\hline

2.342 & 0.404 & 0.792 & 117 & 91.7 $\pm$ 12.4 $\pm$ 8.26  \\
\hline

2.341 & 0.403 & 0.788 & 135 & 68.6 $\pm$ 7.93 $\pm$ 6.92  \\
\hline

2.346 & 0.404 & 0.780 & 153 & 57.0 $\pm$ 9.02 $\pm$ 5.17  \\
\hline

2.343 & 0.404 & 0.783 & 207 & 47.1 $\pm$ 9.07 $\pm$ 7.66  \\
\hline

2.342 & 0.404 & 0.787 & 225 & 68.5 $\pm$ 5.38 $\pm$ 7.67  \\
\hline

2.345 & 0.404 & 0.793 & 243 & 65.0 $\pm$ 6.12 $\pm$ 5.33  \\
\hline

2.343 & 0.404 & 0.794 & 261 & 67.2 $\pm$ 11.0 $\pm$ 2.50  \\
\hline

2.342 & 0.404 & 0.791 & 297 & 57.3 $\pm$ 8.84 $\pm$ 2.93  \\
\hline

2.342 & 0.404 & 0.789 & 315 & 63.2 $\pm$ 4.50 $\pm$ 2.54  \\
\hline

2.343 & 0.404 & 0.786 & 333 & 39.1 $\pm$ 3.19 $\pm$ 1.82  \\
\hline

2.345 & 0.403 & 0.781 & 351 & 33.5 $\pm$ 3.24 $\pm$ 4.13  \\
\hline

2.344 & 0.404 & 1.225 & 9 & 24.1 $\pm$ 5.04 $\pm$ 6.89  \\
\hline

2.342 & 0.404 & 1.226 & 27 & 20.9 $\pm$ 1.98 $\pm$ 0.60  \\
\hline

2.344 & 0.404 & 1.227 & 45 & 23.4 $\pm$ 2.83 $\pm$ 2.34  \\
\hline

2.343 & 0.404 & 1.223 & 63 & 24.7 $\pm$ 8.22 $\pm$ 0.89  \\
\hline

2.344 & 0.404 & 1.230 & 81 & 36.6 $\pm$ 4.76 $\pm$ 1.45  \\
\hline

2.341 & 0.404 & 1.230 & 99 & 36.0 $\pm$ 3.35 $\pm$ 5.20  \\
\hline

2.344 & 0.404 & 1.224 & 117 & 37.1 $\pm$ 5.09 $\pm$ 3.89  \\
\hline

2.346 & 0.404 & 1.225 & 135 & 42.4 $\pm$ 5.58 $\pm$ 2.19  \\
\hline

2.346 & 0.404 & 1.223 & 153 & 28.8 $\pm$ 7.99 $\pm$ 4.27  \\
\hline

2.345 & 0.404 & 1.228 & 207 & 61.3 $\pm$ 11.8 $\pm$ 2.05  \\
\hline

2.344 & 0.404 & 1.223 & 225 & 33.2 $\pm$ 3.62 $\pm$ 0.70  \\
\hline

2.344 & 0.404 & 1.230 & 243 & 45.7 $\pm$ 5.66 $\pm$ 1.80  \\
\hline

2.344 & 0.404 & 1.231 & 261 & 45.2 $\pm$ 5.11 $\pm$ 4.42  \\
\hline

2.345 & 0.404 & 1.231 & 279 & 36.7 $\pm$ 5.60 $\pm$ 0.73  \\
\hline

2.345 & 0.404 & 1.230 & 297 & 19.9 $\pm$ 6.28 $\pm$ 2.57  \\
\hline

2.342 & 0.404 & 1.226 & 315 & 30.0 $\pm$ 3.28 $\pm$ 1.68  \\
\hline

2.343 & 0.404 & 1.224 & 333 & 17.3 $\pm$ 2.01 $\pm$ 1.49  \\
\hline

2.344 & 0.404 & 1.229 & 351 & 6.13 $\pm$ 2.74 $\pm$ 1.39  \\
\hline

2.345 & 0.404 & 1.728 & 9 & 7.17 $\pm$ 2.07 $\pm$ 0.81  \\
\hline

2.345 & 0.404 & 1.729 & 27 & 9.55 $\pm$ 1.53 $\pm$ 1.98  \\
\hline

2.346 & 0.405 & 1.726 & 45 & 7.80 $\pm$ 3.49 $\pm$ 0.38  \\
\hline

2.344 & 0.405 & 1.723 & 63 & 14.6 $\pm$ 5.53 $\pm$ 1.56  \\
\hline

2.344 & 0.404 & 1.724 & 81 & 14.3 $\pm$ 1.73 $\pm$ 0.90  \\
\hline

2.345 & 0.404 & 1.722 & 99 & 20.2 $\pm$ 2.11 $\pm$ 1.03  \\
\hline

2.345 & 0.404 & 1.721 & 117 & 17.7 $\pm$ 3.09 $\pm$ 2.65  \\
\hline

2.343 & 0.404 & 1.725 & 135 & 23.2 $\pm$ 5.07 $\pm$ 1.83  \\
\hline

2.344 & 0.404 & 1.726 & 225 & 16.0 $\pm$ 3.35 $\pm$ 1.46  \\
\hline

2.346 & 0.405 & 1.725 & 243 & 19.6 $\pm$ 3.85 $\pm$ 2.90  \\
\hline

2.345 & 0.405 & 1.723 & 261 & 12.4 $\pm$ 1.91 $\pm$ 0.87  \\
\hline

2.346 & 0.404 & 1.730 & 279 & 17.4 $\pm$ 1.94 $\pm$ 1.63  \\
\hline

2.345 & 0.404 & 1.724 & 297 & 10.2 $\pm$ 3.41 $\pm$ 0.34  \\
\hline

2.343 & 0.405 & 1.725 & 315 & 10.3 $\pm$ 3.91 $\pm$ 0.59  \\
\hline

2.345 & 0.404 & 1.725 & 333 & 8.23 $\pm$ 1.68 $\pm$ 2.24  \\
\hline

2.590 & 0.289 & 0.249 & 45 & 33.6 $\pm$ 15.1 $\pm$ 11.7  \\
\hline

2.587 & 0.289 & 0.249 & 63 & 20.6 $\pm$ 9.21 $\pm$ 3.01  \\
\hline

2.590 & 0.289 & 0.248 & 81 & 14.1 $\pm$ 6.31 $\pm$ 10.4  \\
\hline

2.585 & 0.289 & 0.249 & 171 & 36.3 $\pm$ 14.8 $\pm$ 0.71  \\
\hline

2.584 & 0.289 & 0.251 & 261 & 39.1 $\pm$ 11.8 $\pm$ 6.23  \\
\hline

2.586 & 0.289 & 0.248 & 279 & 27.8 $\pm$ 11.4 $\pm$ 6.20  \\
\hline

2.593 & 0.289 & 0.248 & 297 & 62.4 $\pm$ 17.3 $\pm$ 23.1  \\
\hline

2.589 & 0.289 & 0.350 & 63 & 51.4 $\pm$ 13.3 $\pm$ 7.82  \\
\hline

2.591 & 0.289 & 0.350 & 81 & 39.8 $\pm$ 11.0 $\pm$ 7.95  \\
\hline

2.583 & 0.289 & 0.351 & 99 & 20.7 $\pm$ 7.33 $\pm$ 1.66  \\
\hline

2.585 & 0.289 & 0.348 & 261 & 36.1 $\pm$ 11.4 $\pm$ 3.46  \\
\hline

2.584 & 0.290 & 0.349 & 297 & 20.0 $\pm$ 8.16 $\pm$ 0.61  \\
\hline

2.586 & 0.289 & 0.494 & 45 & 23.0 $\pm$ 7.69 $\pm$ 14.0  \\
\hline

2.585 & 0.289 & 0.498 & 63 & 18.6 $\pm$ 4.98 $\pm$ 1.49  \\
\hline

2.588 & 0.290 & 0.497 & 81 & 20.4 $\pm$ 5.10 $\pm$ 3.23  \\
\hline

2.593 & 0.290 & 0.497 & 99 & 28.1 $\pm$ 6.46 $\pm$ 1.55  \\
\hline

2.587 & 0.289 & 0.500 & 261 & 23.5 $\pm$ 6.79 $\pm$ 3.22  \\
\hline

2.588 & 0.289 & 0.496 & 279 & 30.3 $\pm$ 7.36 $\pm$ 0.35  \\
\hline

2.589 & 0.289 & 0.496 & 297 & 21.6 $\pm$ 5.39 $\pm$ 1.33  \\
\hline

2.587 & 0.289 & 0.495 & 315 & 13.1 $\pm$ 5.35 $\pm$ 1.02  \\
\hline

2.584 & 0.289 & 0.779 & 45 & 6.47 $\pm$ 2.29 $\pm$ 1.95  \\
\hline

2.588 & 0.290 & 0.777 & 63 & 19.9 $\pm$ 3.76 $\pm$ 3.66  \\
\hline

2.587 & 0.290 & 0.781 & 81 & 19.4 $\pm$ 3.74 $\pm$ 4.34  \\
\hline

2.587 & 0.289 & 0.773 & 99 & 22.7 $\pm$ 5.51 $\pm$ 1.12  \\
\hline

2.585 & 0.289 & 0.777 & 261 & 16.5 $\pm$ 5.22 $\pm$ 2.53  \\
\hline

2.589 & 0.289 & 0.779 & 279 & 17.9 $\pm$ 3.91 $\pm$ 0.53  \\
\hline

2.584 & 0.290 & 0.782 & 297 & 10.7 $\pm$ 2.38 $\pm$ 1.66  \\
\hline

2.589 & 0.290 & 0.782 & 315 & 14.3 $\pm$ 2.98 $\pm$ 2.44  \\
\hline

2.585 & 0.289 & 1.216 & 9 & 15.7 $\pm$ 7.02 $\pm$ 2.35  \\
\hline

2.589 & 0.289 & 1.224 & 27 & 8.40 $\pm$ 2.33 $\pm$ 0.70  \\
\hline

2.590 & 0.290 & 1.205 & 45 & 5.32 $\pm$ 1.77 $\pm$ 1.17  \\
\hline

2.586 & 0.290 & 1.218 & 63 & 5.71 $\pm$ 2.02 $\pm$ 2.17  \\
\hline

2.584 & 0.289 & 1.219 & 81 & 18.0 $\pm$ 6.79 $\pm$ 2.85  \\
\hline

2.590 & 0.290 & 1.219 & 297 & 5.19 $\pm$ 1.84 $\pm$ 3.17  \\
\hline

2.589 & 0.290 & 1.217 & 315 & 6.84 $\pm$ 1.71 $\pm$ 1.17  \\
\hline

2.592 & 0.290 & 1.211 & 333 & 6.11 $\pm$ 2.31 $\pm$ 1.72  \\
\hline

2.711 & 0.336 & 0.178 & 9 & 23.3 $\pm$ 8.25 $\pm$ 1.72  \\
\hline

2.713 & 0.335 & 0.178 & 27 & 25.4 $\pm$ 7.33 $\pm$ 5.05  \\
\hline

2.710 & 0.336 & 0.177 & 45 & 39.2 $\pm$ 8.76 $\pm$ 2.81  \\
\hline

2.710 & 0.336 & 0.178 & 63 & 33.1 $\pm$ 9.55 $\pm$ 2.60  \\
\hline

2.712 & 0.336 & 0.178 & 81 & 49.8 $\pm$ 13.3 $\pm$ 1.44  \\
\hline

2.713 & 0.337 & 0.178 & 99 & 25.7 $\pm$ 8.12 $\pm$ 5.07  \\
\hline

2.708 & 0.336 & 0.177 & 153 & 51.4 $\pm$ 23.0 $\pm$ 12.0  \\
\hline

2.711 & 0.336 & 0.178 & 243 & 43.4 $\pm$ 12.5 $\pm$ 5.41  \\
\hline

2.710 & 0.337 & 0.177 & 261 & 41.9 $\pm$ 10.8 $\pm$ 4.53  \\
\hline

2.712 & 0.336 & 0.178 & 279 & 44.8 $\pm$ 12.4 $\pm$ 2.16  \\
\hline

2.705 & 0.337 & 0.178 & 297 & 14.7 $\pm$ 5.99 $\pm$ 1.93  \\
\hline

2.706 & 0.336 & 0.178 & 315 & 34.5 $\pm$ 8.14 $\pm$ 6.80  \\
\hline

2.706 & 0.336 & 0.178 & 333 & 27.4 $\pm$ 8.66 $\pm$ 9.29  \\
\hline

2.715 & 0.342 & 0.249 & 9 & 33.9 $\pm$ 5.66 $\pm$ 1.94  \\
\hline

2.714 & 0.341 & 0.249 & 27 & 38.0 $\pm$ 5.08 $\pm$ 4.34  \\
\hline

2.713 & 0.342 & 0.249 & 45 & 34.6 $\pm$ 5.22 $\pm$ 7.14  \\
\hline

2.711 & 0.342 & 0.249 & 63 & 42.4 $\pm$ 6.32 $\pm$ 4.35  \\
\hline

2.714 & 0.342 & 0.248 & 81 & 34.4 $\pm$ 6.09 $\pm$ 0.35  \\
\hline

2.711 & 0.342 & 0.249 & 99 & 41.6 $\pm$ 5.56 $\pm$ 5.49  \\
\hline

2.710 & 0.343 & 0.248 & 117 & 35.6 $\pm$ 5.50 $\pm$ 2.45  \\
\hline

2.717 & 0.342 & 0.250 & 135 & 33.2 $\pm$ 5.97 $\pm$ 4.96  \\
\hline

2.712 & 0.342 & 0.249 & 153 & 31.2 $\pm$ 5.21 $\pm$ 2.11  \\
\hline

2.714 & 0.343 & 0.250 & 171 & 42.8 $\pm$ 8.74 $\pm$ 2.51  \\
\hline

2.712 & 0.342 & 0.250 & 189 & 23.2 $\pm$ 6.00 $\pm$ 3.80  \\
\hline

2.712 & 0.342 & 0.249 & 207 & 45.7 $\pm$ 7.84 $\pm$ 3.86  \\
\hline

2.714 & 0.342 & 0.249 & 225 & 28.3 $\pm$ 5.78 $\pm$ 0.69  \\
\hline

2.717 & 0.342 & 0.249 & 243 & 42.4 $\pm$ 5.42 $\pm$ 2.61  \\
\hline

2.711 & 0.342 & 0.248 & 261 & 48.2 $\pm$ 7.18 $\pm$ 4.11  \\
\hline

2.711 & 0.342 & 0.250 & 279 & 44.8 $\pm$ 7.01 $\pm$ 1.23  \\
\hline

2.713 & 0.342 & 0.249 & 297 & 29.7 $\pm$ 4.96 $\pm$ 1.84  \\
\hline

2.715 & 0.342 & 0.248 & 315 & 32.3 $\pm$ 4.82 $\pm$ 4.32  \\
\hline

2.710 & 0.342 & 0.249 & 333 & 26.4 $\pm$ 4.82 $\pm$ 0.70  \\
\hline

2.712 & 0.341 & 0.249 & 351 & 24.2 $\pm$ 4.93 $\pm$ 5.90  \\
\hline

2.710 & 0.343 & 0.350 & 9 & 38.5 $\pm$ 5.80 $\pm$ 4.56  \\
\hline

2.712 & 0.342 & 0.349 & 27 & 30.6 $\pm$ 4.06 $\pm$ 4.18  \\
\hline

2.713 & 0.342 & 0.348 & 45 & 37.8 $\pm$ 4.45 $\pm$ 0.86  \\
\hline

2.712 & 0.342 & 0.350 & 63 & 44.4 $\pm$ 5.38 $\pm$ 5.15  \\
\hline

2.710 & 0.342 & 0.349 & 81 & 36.2 $\pm$ 5.87 $\pm$ 2.36  \\
\hline

2.712 & 0.342 & 0.350 & 99 & 52.3 $\pm$ 7.63 $\pm$ 3.17  \\
\hline

2.716 & 0.342 & 0.349 & 117 & 59.7 $\pm$ 8.81 $\pm$ 0.74  \\
\hline

2.709 & 0.342 & 0.349 & 135 & 30.8 $\pm$ 5.63 $\pm$ 1.89  \\
\hline

2.716 & 0.343 & 0.348 & 153 & 31.7 $\pm$ 5.61 $\pm$ 2.32  \\
\hline

2.714 & 0.343 & 0.348 & 171 & 51.3 $\pm$ 9.88 $\pm$ 3.95  \\
\hline

2.715 & 0.343 & 0.349 & 189 & 14.7 $\pm$ 4.89 $\pm$ 2.89  \\
\hline

2.710 & 0.342 & 0.349 & 207 & 34.7 $\pm$ 7.08 $\pm$ 4.54  \\
\hline

2.713 & 0.341 & 0.350 & 225 & 29.4 $\pm$ 5.66 $\pm$ 2.69  \\
\hline

2.714 & 0.342 & 0.350 & 243 & 35.7 $\pm$ 5.44 $\pm$ 2.58  \\
\hline

2.713 & 0.342 & 0.349 & 261 & 50.2 $\pm$ 8.49 $\pm$ 5.84  \\
\hline

2.713 & 0.342 & 0.350 & 279 & 35.1 $\pm$ 6.20 $\pm$ 2.22  \\
\hline

2.714 & 0.342 & 0.350 & 297 & 34.5 $\pm$ 4.69 $\pm$ 2.48  \\
\hline

2.715 & 0.343 & 0.350 & 315 & 41.4 $\pm$ 4.60 $\pm$ 1.02  \\
\hline

2.717 & 0.342 & 0.349 & 333 & 26.3 $\pm$ 4.45 $\pm$ 0.27  \\
\hline

2.710 & 0.342 & 0.349 & 351 & 41.5 $\pm$ 6.73 $\pm$ 2.71  \\
\hline

2.713 & 0.343 & 0.498 & 9 & 15.1 $\pm$ 3.15 $\pm$ 1.95  \\
\hline

2.713 & 0.342 & 0.498 & 27 & 28.9 $\pm$ 2.98 $\pm$ 3.67  \\
\hline

2.715 & 0.342 & 0.497 & 45 & 32.5 $\pm$ 2.76 $\pm$ 1.55  \\
\hline

2.712 & 0.342 & 0.498 & 63 & 40.7 $\pm$ 3.18 $\pm$ 4.01  \\
\hline

2.711 & 0.342 & 0.498 & 81 & 36.3 $\pm$ 3.81 $\pm$ 0.47  \\
\hline

2.711 & 0.342 & 0.497 & 99 & 29.6 $\pm$ 5.31 $\pm$ 3.14  \\
\hline

2.712 & 0.343 & 0.498 & 117 & 38.3 $\pm$ 7.23 $\pm$ 6.86  \\
\hline

2.715 & 0.342 & 0.497 & 135 & 38.1 $\pm$ 6.18 $\pm$ 4.34  \\
\hline

2.714 & 0.343 & 0.496 & 153 & 17.7 $\pm$ 4.06 $\pm$ 5.11  \\
\hline

2.714 & 0.343 & 0.495 & 171 & 24.9 $\pm$ 6.04 $\pm$ 5.34  \\
\hline

2.711 & 0.343 & 0.496 & 189 & 18.0 $\pm$ 4.37 $\pm$ 2.42  \\
\hline

2.712 & 0.343 & 0.495 & 207 & 26.5 $\pm$ 5.40 $\pm$ 3.56  \\
\hline

2.714 & 0.343 & 0.495 & 225 & 18.2 $\pm$ 4.42 $\pm$ 4.62  \\
\hline

2.716 & 0.342 & 0.496 & 243 & 40.2 $\pm$ 5.87 $\pm$ 4.25  \\
\hline

2.715 & 0.342 & 0.498 & 261 & 33.6 $\pm$ 6.25 $\pm$ 5.67  \\
\hline

2.714 & 0.343 & 0.499 & 279 & 31.4 $\pm$ 4.02 $\pm$ 1.19  \\
\hline

2.711 & 0.342 & 0.498 & 297 & 37.1 $\pm$ 2.95 $\pm$ 1.10  \\
\hline

2.711 & 0.342 & 0.498 & 315 & 30.5 $\pm$ 2.48 $\pm$ 1.89  \\
\hline

2.712 & 0.342 & 0.496 & 333 & 30.8 $\pm$ 3.66 $\pm$ 0.49  \\
\hline

2.712 & 0.342 & 0.497 & 351 & 34.9 $\pm$ 5.81 $\pm$ 6.37  \\
\hline

2.714 & 0.343 & 0.781 & 9 & 23.2 $\pm$ 7.75 $\pm$ 3.06  \\
\hline

2.712 & 0.343 & 0.782 & 27 & 12.5 $\pm$ 1.68 $\pm$ 0.34  \\
\hline

2.712 & 0.343 & 0.784 & 45 & 17.6 $\pm$ 1.38 $\pm$ 0.60  \\
\hline

2.712 & 0.343 & 0.784 & 63 & 21.4 $\pm$ 1.63 $\pm$ 2.03  \\
\hline

2.714 & 0.343 & 0.785 & 81 & 28.3 $\pm$ 2.89 $\pm$ 1.08  \\
\hline

2.713 & 0.343 & 0.787 & 99 & 20.3 $\pm$ 5.43 $\pm$ 0.95  \\
\hline

2.711 & 0.343 & 0.786 & 117 & 24.3 $\pm$ 5.06 $\pm$ 2.61  \\
\hline

2.714 & 0.343 & 0.780 & 135 & 15.1 $\pm$ 3.89 $\pm$ 2.19  \\
\hline

2.713 & 0.344 & 0.782 & 153 & 9.45 $\pm$ 2.85 $\pm$ 2.66  \\
\hline

2.716 & 0.344 & 0.781 & 171 & 11.5 $\pm$ 2.89 $\pm$ 1.52  \\
\hline

2.713 & 0.343 & 0.780 & 189 & 12.1 $\pm$ 2.10 $\pm$ 1.52  \\
\hline

2.711 & 0.343 & 0.780 & 207 & 14.7 $\pm$ 3.07 $\pm$ 2.68  \\
\hline

2.710 & 0.344 & 0.783 & 225 & 13.5 $\pm$ 3.27 $\pm$ 1.78  \\
\hline

2.711 & 0.343 & 0.786 & 243 & 26.5 $\pm$ 4.84 $\pm$ 2.97  \\
\hline

2.714 & 0.343 & 0.787 & 261 & 27.9 $\pm$ 7.21 $\pm$ 4.63  \\
\hline

2.713 & 0.343 & 0.786 & 279 & 24.5 $\pm$ 3.00 $\pm$ 0.68  \\
\hline

2.712 & 0.343 & 0.785 & 297 & 21.5 $\pm$ 1.54 $\pm$ 1.39  \\
\hline

2.712 & 0.344 & 0.783 & 315 & 17.3 $\pm$ 1.26 $\pm$ 1.06  \\
\hline

2.713 & 0.343 & 0.783 & 333 & 16.2 $\pm$ 2.19 $\pm$ 0.98  \\
\hline

2.712 & 0.344 & 1.221 & 27 & 9.06 $\pm$ 1.12 $\pm$ 1.63  \\
\hline

2.713 & 0.344 & 1.224 & 45 & 11.6 $\pm$ 1.08 $\pm$ 0.44  \\
\hline

2.712 & 0.344 & 1.223 & 63 & 15.2 $\pm$ 2.03 $\pm$ 0.29  \\
\hline

2.710 & 0.345 & 1.219 & 81 & 10.3 $\pm$ 3.43 $\pm$ 0.55  \\
\hline

2.715 & 0.345 & 1.219 & 99 & 12.6 $\pm$ 2.37 $\pm$ 1.06  \\
\hline

2.714 & 0.345 & 1.222 & 117 & 7.44 $\pm$ 1.86 $\pm$ 0.59  \\
\hline

2.714 & 0.344 & 1.222 & 135 & 8.13 $\pm$ 2.45 $\pm$ 1.36  \\
\hline

2.719 & 0.344 & 1.221 & 153 & 5.61 $\pm$ 1.87 $\pm$ 1.93  \\
\hline

2.713 & 0.343 & 1.223 & 171 & 5.29 $\pm$ 1.87 $\pm$ 0.98  \\
\hline

2.716 & 0.343 & 1.224 & 189 & 6.10 $\pm$ 1.36 $\pm$ 2.14  \\
\hline

2.716 & 0.344 & 1.223 & 207 & 3.14 $\pm$ 1.19 $\pm$ 1.15  \\
\hline

2.711 & 0.343 & 1.222 & 225 & 8.43 $\pm$ 2.04 $\pm$ 4.82  \\
\hline

2.713 & 0.345 & 1.224 & 243 & 7.35 $\pm$ 2.12 $\pm$ 1.19  \\
\hline

2.711 & 0.344 & 1.224 & 261 & 19.2 $\pm$ 4.66 $\pm$ 4.89  \\
\hline

2.709 & 0.345 & 1.222 & 279 & 9.59 $\pm$ 4.29 $\pm$ 0.37  \\
\hline

2.712 & 0.344 & 1.222 & 297 & 7.68 $\pm$ 1.34 $\pm$ 0.55  \\
\hline

2.710 & 0.344 & 1.222 & 315 & 7.87 $\pm$ 0.83 $\pm$ 0.50  \\
\hline

2.713 & 0.344 & 1.224 & 333 & 7.74 $\pm$ 1.11 $\pm$ 1.18  \\
\hline

2.713 & 0.345 & 1.718 & 9 & 3.17 $\pm$ 0.92 $\pm$ 0.22  \\
\hline

2.713 & 0.344 & 1.719 & 27 & 3.61 $\pm$ 0.81 $\pm$ 0.30  \\
\hline

2.712 & 0.345 & 1.723 & 63 & 4.88 $\pm$ 2.18 $\pm$ 0.30  \\
\hline

2.712 & 0.345 & 1.724 & 81 & 5.14 $\pm$ 1.21 $\pm$ 0.51  \\
\hline

2.718 & 0.345 & 1.722 & 99 & 6.21 $\pm$ 1.06 $\pm$ 1.61  \\
\hline

2.716 & 0.345 & 1.719 & 117 & 5.61 $\pm$ 1.17 $\pm$ 0.42  \\
\hline

2.713 & 0.344 & 1.723 & 135 & 10.0 $\pm$ 2.43 $\pm$ 3.27  \\
\hline

2.714 & 0.344 & 1.725 & 153 & 7.65 $\pm$ 1.91 $\pm$ 0.51  \\
\hline

2.717 & 0.344 & 1.728 & 171 & 4.41 $\pm$ 1.47 $\pm$ 0.60  \\
\hline

2.712 & 0.344 & 1.724 & 189 & 2.89 $\pm$ 0.87 $\pm$ 1.31  \\
\hline

2.722 & 0.344 & 1.723 & 207 & 4.57 $\pm$ 1.38 $\pm$ 0.39  \\
\hline

2.715 & 0.344 & 1.724 & 225 & 3.71 $\pm$ 1.31 $\pm$ 1.19  \\
\hline

2.712 & 0.345 & 1.721 & 243 & 8.38 $\pm$ 2.53 $\pm$ 1.59  \\
\hline

2.714 & 0.345 & 1.720 & 261 & 4.96 $\pm$ 1.50 $\pm$ 2.05  \\
\hline

2.709 & 0.346 & 1.721 & 279 & 4.91 $\pm$ 1.36 $\pm$ 1.64  \\
\hline

2.711 & 0.345 & 1.723 & 297 & 5.88 $\pm$ 2.22 $\pm$ 1.01  \\
\hline

2.718 & 0.344 & 1.724 & 315 & 4.70 $\pm$ 1.92 $\pm$ 0.47  \\
\hline

2.714 & 0.345 & 1.719 & 333 & 2.87 $\pm$ 0.87 $\pm$ 0.63  \\
\hline

2.728 & 0.406 & 0.262 & 9 & 45.5 $\pm$ 11.0 $\pm$ 12.7  \\
\hline

2.726 & 0.407 & 0.262 & 27 & 31.7 $\pm$ 7.93 $\pm$ 5.18  \\
\hline

2.728 & 0.406 & 0.261 & 45 & 51.8 $\pm$ 9.46 $\pm$ 5.07  \\
\hline

2.729 & 0.406 & 0.262 & 63 & 57.4 $\pm$ 12.5 $\pm$ 9.61  \\
\hline

2.728 & 0.407 & 0.262 & 81 & 42.6 $\pm$ 13.5 $\pm$ 8.44  \\
\hline

2.733 & 0.407 & 0.262 & 99 & 70.4 $\pm$ 23.5 $\pm$ 8.78  \\
\hline

2.735 & 0.406 & 0.261 & 279 & 63.6 $\pm$ 13.3 $\pm$ 4.28  \\
\hline

2.730 & 0.407 & 0.262 & 297 & 42.4 $\pm$ 8.49 $\pm$ 0.56  \\
\hline

2.732 & 0.406 & 0.262 & 315 & 24.7 $\pm$ 7.83 $\pm$ 5.17  \\
\hline

2.732 & 0.407 & 0.263 & 333 & 74.2 $\pm$ 15.5 $\pm$ 0.88  \\
\hline

2.734 & 0.407 & 0.262 & 351 & 62.7 $\pm$ 14.8 $\pm$ 0.64  \\
\hline

2.742 & 0.422 & 0.351 & 9 & 59.7 $\pm$ 8.71 $\pm$ 7.24  \\
\hline

2.745 & 0.422 & 0.350 & 27 & 43.9 $\pm$ 7.52 $\pm$ 2.30  \\
\hline

2.751 & 0.422 & 0.351 & 45 & 76.6 $\pm$ 13.3 $\pm$ 11.9  \\
\hline

2.745 & 0.421 & 0.350 & 63 & 26.7 $\pm$ 10.1 $\pm$ 5.98  \\
\hline

2.751 & 0.421 & 0.351 & 81 & 30.2 $\pm$ 8.71 $\pm$ 2.11  \\
\hline

2.748 & 0.422 & 0.351 & 99 & 57.6 $\pm$ 13.2 $\pm$ 2.35  \\
\hline

2.746 & 0.421 & 0.350 & 117 & 94.5 $\pm$ 26.2 $\pm$ 13.9  \\
\hline

2.749 & 0.422 & 0.351 & 243 & 57.2 $\pm$ 23.3 $\pm$ 8.85  \\
\hline

2.746 & 0.421 & 0.350 & 261 & 66.6 $\pm$ 15.7 $\pm$ 4.02  \\
\hline

2.748 & 0.422 & 0.351 & 279 & 53.7 $\pm$ 10.1 $\pm$ 8.66  \\
\hline

2.746 & 0.421 & 0.351 & 297 & 48.1 $\pm$ 10.2 $\pm$ 6.42  \\
\hline

2.742 & 0.422 & 0.350 & 315 & 43.1 $\pm$ 9.90 $\pm$ 7.72  \\
\hline

2.744 & 0.421 & 0.350 & 333 & 47.8 $\pm$ 8.58 $\pm$ 4.66  \\
\hline

2.750 & 0.421 & 0.350 & 351 & 49.7 $\pm$ 8.53 $\pm$ 1.77  \\
\hline

2.747 & 0.422 & 0.497 & 9 & 44.6 $\pm$ 3.68 $\pm$ 2.18  \\
\hline

2.749 & 0.422 & 0.499 & 27 & 44.5 $\pm$ 3.79 $\pm$ 2.91  \\
\hline

2.749 & 0.423 & 0.499 & 45 & 55.3 $\pm$ 5.53 $\pm$ 0.63  \\
\hline

2.746 & 0.422 & 0.498 & 63 & 49.2 $\pm$ 9.47 $\pm$ 10.8  \\
\hline

2.750 & 0.423 & 0.498 & 81 & 50.2 $\pm$ 12.5 $\pm$ 16.2  \\
\hline

2.748 & 0.422 & 0.497 & 99 & 58.4 $\pm$ 10.5 $\pm$ 4.55  \\
\hline

2.748 & 0.423 & 0.498 & 117 & 71.6 $\pm$ 13.3 $\pm$ 9.68  \\
\hline

2.749 & 0.423 & 0.498 & 135 & 48.0 $\pm$ 13.8 $\pm$ 5.65  \\
\hline

2.753 & 0.423 & 0.498 & 225 & 54.3 $\pm$ 9.91 $\pm$ 6.88  \\
\hline

2.751 & 0.423 & 0.499 & 243 & 57.8 $\pm$ 8.82 $\pm$ 4.34  \\
\hline

2.748 & 0.422 & 0.498 & 261 & 44.6 $\pm$ 9.97 $\pm$ 1.80  \\
\hline

2.748 & 0.423 & 0.498 & 279 & 48.9 $\pm$ 10.2 $\pm$ 7.94  \\
\hline

2.749 & 0.422 & 0.498 & 297 & 53.4 $\pm$ 9.29 $\pm$ 1.92  \\
\hline

2.747 & 0.422 & 0.497 & 315 & 63.7 $\pm$ 6.13 $\pm$ 3.19  \\
\hline

2.750 & 0.423 & 0.498 & 333 & 41.6 $\pm$ 4.20 $\pm$ 4.84  \\
\hline

2.747 & 0.423 & 0.498 & 351 & 43.5 $\pm$ 4.13 $\pm$ 3.24  \\
\hline

2.751 & 0.423 & 0.785 & 9 & 35.2 $\pm$ 2.45 $\pm$ 3.35  \\
\hline

2.750 & 0.424 & 0.789 & 27 & 34.5 $\pm$ 2.07 $\pm$ 0.92  \\
\hline

2.749 & 0.423 & 0.792 & 45 & 33.7 $\pm$ 2.53 $\pm$ 1.20  \\
\hline

2.750 & 0.423 & 0.791 & 63 & 40.2 $\pm$ 5.58 $\pm$ 2.21  \\
\hline

2.748 & 0.423 & 0.792 & 81 & 81.3 $\pm$ 16.3 $\pm$ 4.03  \\
\hline

2.749 & 0.423 & 0.789 & 99 & 48.4 $\pm$ 6.52 $\pm$ 3.74  \\
\hline

2.748 & 0.423 & 0.791 & 117 & 49.5 $\pm$ 7.56 $\pm$ 6.08  \\
\hline

2.751 & 0.424 & 0.788 & 135 & 45.3 $\pm$ 5.62 $\pm$ 6.22  \\
\hline

2.752 & 0.424 & 0.781 & 153 & 32.4 $\pm$ 5.25 $\pm$ 5.97  \\
\hline

2.751 & 0.424 & 0.779 & 189 & 25.5 $\pm$ 6.58 $\pm$ 8.90  \\
\hline

2.751 & 0.424 & 0.784 & 207 & 20.0 $\pm$ 4.86 $\pm$ 6.10  \\
\hline

2.750 & 0.424 & 0.788 & 225 & 40.2 $\pm$ 3.73 $\pm$ 2.94  \\
\hline

2.749 & 0.423 & 0.793 & 243 & 41.2 $\pm$ 4.27 $\pm$ 5.14  \\
\hline

2.749 & 0.423 & 0.792 & 261 & 51.3 $\pm$ 8.21 $\pm$ 8.77  \\
\hline

2.751 & 0.423 & 0.793 & 279 & 59.1 $\pm$ 13.6 $\pm$ 8.55  \\
\hline

2.751 & 0.423 & 0.789 & 297 & 28.9 $\pm$ 4.52 $\pm$ 4.81  \\
\hline

2.748 & 0.423 & 0.792 & 315 & 35.5 $\pm$ 2.65 $\pm$ 1.71  \\
\hline

2.751 & 0.423 & 0.788 & 333 & 37.1 $\pm$ 2.54 $\pm$ 1.22  \\
\hline

2.750 & 0.423 & 0.785 & 351 & 32.6 $\pm$ 2.62 $\pm$ 2.67  \\
\hline

2.750 & 0.425 & 1.226 & 9 & 12.8 $\pm$ 2.86 $\pm$ 1.51  \\
\hline

2.752 & 0.424 & 1.225 & 27 & 15.3 $\pm$ 1.36 $\pm$ 0.58  \\
\hline

2.751 & 0.424 & 1.226 & 45 & 19.4 $\pm$ 2.07 $\pm$ 1.47  \\
\hline

2.749 & 0.424 & 1.227 & 63 & 18.1 $\pm$ 6.86 $\pm$ 1.88  \\
\hline

2.749 & 0.425 & 1.231 & 81 & 24.6 $\pm$ 3.42 $\pm$ 1.94  \\
\hline

2.751 & 0.424 & 1.231 & 99 & 21.1 $\pm$ 2.27 $\pm$ 1.76  \\
\hline

2.751 & 0.424 & 1.230 & 117 & 25.8 $\pm$ 3.30 $\pm$ 3.45  \\
\hline

2.749 & 0.424 & 1.225 & 135 & 31.2 $\pm$ 3.85 $\pm$ 3.31  \\
\hline

2.751 & 0.424 & 1.227 & 153 & 22.4 $\pm$ 4.24 $\pm$ 1.79  \\
\hline

2.751 & 0.424 & 1.228 & 207 & 23.5 $\pm$ 5.14 $\pm$ 1.97  \\
\hline

2.749 & 0.425 & 1.227 & 225 & 28.9 $\pm$ 2.85 $\pm$ 1.55  \\
\hline

2.751 & 0.425 & 1.228 & 243 & 29.8 $\pm$ 3.42 $\pm$ 1.96  \\
\hline

2.748 & 0.425 & 1.230 & 261 & 20.9 $\pm$ 3.27 $\pm$ 2.75  \\
\hline

2.749 & 0.424 & 1.231 & 279 & 28.4 $\pm$ 4.38 $\pm$ 2.73  \\
\hline

2.749 & 0.424 & 1.227 & 297 & 20.1 $\pm$ 6.70 $\pm$ 2.25  \\
\hline

2.749 & 0.424 & 1.225 & 315 & 20.2 $\pm$ 2.15 $\pm$ 1.09  \\
\hline

2.751 & 0.424 & 1.226 & 333 & 16.3 $\pm$ 1.64 $\pm$ 1.06  \\
\hline

2.752 & 0.424 & 1.229 & 351 & 19.4 $\pm$ 3.97 $\pm$ 2.76  \\
\hline

2.751 & 0.425 & 1.730 & 9 & 9.24 $\pm$ 3.27 $\pm$ 0.54  \\
\hline

2.753 & 0.426 & 1.729 & 27 & 8.77 $\pm$ 1.63 $\pm$ 0.27  \\
\hline

2.751 & 0.425 & 1.725 & 63 & 18.8 $\pm$ 3.84 $\pm$ 2.23  \\
\hline

2.749 & 0.426 & 1.727 & 81 & 10.2 $\pm$ 1.30 $\pm$ 0.93  \\
\hline

2.749 & 0.426 & 1.724 & 99 & 11.1 $\pm$ 1.23 $\pm$ 1.01  \\
\hline

2.752 & 0.426 & 1.725 & 117 & 14.4 $\pm$ 2.18 $\pm$ 1.69  \\
\hline

2.754 & 0.425 & 1.726 & 135 & 13.3 $\pm$ 2.78 $\pm$ 1.07  \\
\hline

2.749 & 0.425 & 1.728 & 225 & 13.4 $\pm$ 2.15 $\pm$ 2.31  \\
\hline

2.752 & 0.425 & 1.727 & 243 & 10.0 $\pm$ 2.24 $\pm$ 1.27  \\
\hline

2.746 & 0.425 & 1.726 & 261 & 13.1 $\pm$ 1.76 $\pm$ 1.56  \\
\hline

2.750 & 0.426 & 1.728 & 279 & 11.2 $\pm$ 1.46 $\pm$ 0.93  \\
\hline

2.749 & 0.425 & 1.730 & 297 & 8.70 $\pm$ 2.11 $\pm$ 1.39  \\
\hline

2.751 & 0.426 & 1.729 & 315 & 13.8 $\pm$ 5.62 $\pm$ 1.26  \\
\hline

2.752 & 0.425 & 1.723 & 333 & 6.86 $\pm$ 1.58 $\pm$ 0.48  \\
\hline

3.118 & 0.362 & 0.248 & 45 & 48.6 $\pm$ 18.4 $\pm$ 4.17  \\
\hline

3.114 & 0.362 & 0.248 & 63 & 44.1 $\pm$ 15.6 $\pm$ 3.98  \\
\hline

3.115 & 0.362 & 0.249 & 81 & 30.9 $\pm$ 10.3 $\pm$ 1.55  \\
\hline

3.118 & 0.362 & 0.249 & 99 & 25.1 $\pm$ 7.93 $\pm$ 0.45  \\
\hline

3.121 & 0.362 & 0.252 & 117 & 28.9 $\pm$ 10.2 $\pm$ 5.34  \\
\hline

3.130 & 0.364 & 0.249 & 153 & 44.6 $\pm$ 18.2 $\pm$ 2.29  \\
\hline

3.117 & 0.363 & 0.249 & 243 & 16.6 $\pm$ 7.44 $\pm$ 4.84  \\
\hline

3.116 & 0.363 & 0.248 & 279 & 32.6 $\pm$ 10.9 $\pm$ 0.46  \\
\hline

3.117 & 0.362 & 0.249 & 297 & 36.9 $\pm$ 11.7 $\pm$ 8.34  \\
\hline

3.119 & 0.362 & 0.249 & 315 & 46.8 $\pm$ 14.8 $\pm$ 7.16  \\
\hline

3.122 & 0.362 & 0.351 & 45 & 37.6 $\pm$ 16.8 $\pm$ 2.65  \\
\hline

3.119 & 0.361 & 0.351 & 81 & 29.7 $\pm$ 13.3 $\pm$ 7.75  \\
\hline

3.125 & 0.362 & 0.349 & 99 & 26.8 $\pm$ 7.18 $\pm$ 5.67  \\
\hline

3.123 & 0.363 & 0.349 & 117 & 30.6 $\pm$ 8.48 $\pm$ 2.44  \\
\hline

3.123 & 0.363 & 0.350 & 135 & 32.3 $\pm$ 8.96 $\pm$ 1.80  \\
\hline

3.121 & 0.362 & 0.349 & 153 & 42.2 $\pm$ 10.2 $\pm$ 2.67  \\
\hline

3.116 & 0.362 & 0.349 & 171 & 29.4 $\pm$ 13.2 $\pm$ 16.5  \\
\hline

3.120 & 0.363 & 0.349 & 225 & 43.6 $\pm$ 15.4 $\pm$ 3.14  \\
\hline

3.128 & 0.363 & 0.349 & 243 & 34.3 $\pm$ 8.85 $\pm$ 2.65  \\
\hline

3.114 & 0.362 & 0.353 & 261 & 43.1 $\pm$ 11.1 $\pm$ 4.65  \\
\hline

3.122 & 0.363 & 0.350 & 279 & 132. $\pm$ 31.9 $\pm$ 17.0  \\
\hline

3.115 & 0.362 & 0.352 & 315 & 29.8 $\pm$ 13.3 $\pm$ 4.64  \\
\hline

3.122 & 0.363 & 0.497 & 45 & 24.3 $\pm$ 7.03 $\pm$ 3.82  \\
\hline

3.122 & 0.363 & 0.500 & 63 & 16.2 $\pm$ 7.24 $\pm$ 10.2  \\
\hline

3.121 & 0.363 & 0.500 & 81 & 84.3 $\pm$ 34.4 $\pm$ 8.07  \\
\hline

3.124 & 0.363 & 0.501 & 99 & 25.7 $\pm$ 6.87 $\pm$ 3.33  \\
\hline

3.121 & 0.362 & 0.497 & 117 & 27.0 $\pm$ 6.20 $\pm$ 2.13  \\
\hline

3.124 & 0.363 & 0.495 & 135 & 19.0 $\pm$ 5.27 $\pm$ 5.78  \\
\hline

3.120 & 0.363 & 0.499 & 153 & 25.4 $\pm$ 7.05 $\pm$ 3.67  \\
\hline

3.120 & 0.362 & 0.496 & 171 & 23.4 $\pm$ 10.5 $\pm$ 5.91  \\
\hline

3.125 & 0.363 & 0.494 & 189 & 27.9 $\pm$ 12.5 $\pm$ 10.4  \\
\hline

3.118 & 0.362 & 0.497 & 207 & 35.2 $\pm$ 11.1 $\pm$ 6.68  \\
\hline

3.123 & 0.363 & 0.496 & 225 & 29.6 $\pm$ 7.19 $\pm$ 3.63  \\
\hline

3.120 & 0.363 & 0.497 & 243 & 32.7 $\pm$ 5.78 $\pm$ 0.33  \\
\hline

3.120 & 0.362 & 0.497 & 261 & 32.6 $\pm$ 8.42 $\pm$ 0.40  \\
\hline

3.121 & 0.363 & 0.496 & 297 & 28.4 $\pm$ 7.58 $\pm$ 6.06  \\
\hline

3.119 & 0.363 & 0.496 & 315 & 31.6 $\pm$ 7.07 $\pm$ 4.47  \\
\hline

3.118 & 0.362 & 0.498 & 333 & 31.8 $\pm$ 13.0 $\pm$ 9.20  \\
\hline

3.119 & 0.362 & 0.782 & 45 & 17.2 $\pm$ 3.75 $\pm$ 6.43  \\
\hline

3.122 & 0.363 & 0.787 & 63 & 15.9 $\pm$ 4.25 $\pm$ 0.31  \\
\hline

3.122 & 0.363 & 0.784 & 81 & 53.3 $\pm$ 23.9 $\pm$ 12.0  \\
\hline

3.120 & 0.363 & 0.783 & 99 & 21.4 $\pm$ 5.04 $\pm$ 1.12  \\
\hline

3.118 & 0.363 & 0.785 & 117 & 24.1 $\pm$ 5.53 $\pm$ 3.24  \\
\hline

3.119 & 0.363 & 0.787 & 225 & 18.1 $\pm$ 8.11 $\pm$ 6.17  \\
\hline

3.122 & 0.363 & 0.781 & 243 & 18.8 $\pm$ 4.43 $\pm$ 2.68  \\
\hline

3.120 & 0.363 & 0.784 & 261 & 33.5 $\pm$ 7.50 $\pm$ 4.48  \\
\hline

3.117 & 0.363 & 0.785 & 297 & 10.5 $\pm$ 3.04 $\pm$ 2.29  \\
\hline

3.123 & 0.363 & 0.785 & 315 & 18.5 $\pm$ 3.50 $\pm$ 1.98  \\
\hline

3.121 & 0.363 & 1.228 & 45 & 6.00 $\pm$ 2.68 $\pm$ 0.83  \\
\hline

3.117 & 0.363 & 1.220 & 81 & 6.25 $\pm$ 2.79 $\pm$ 0.74  \\
\hline

3.124 & 0.363 & 1.225 & 99 & 13.1 $\pm$ 4.16 $\pm$ 1.09  \\
\hline

3.121 & 0.363 & 1.222 & 261 & 9.85 $\pm$ 4.02 $\pm$ 0.55  \\
\hline

3.118 & 0.363 & 1.226 & 315 & 6.98 $\pm$ 2.33 $\pm$ 2.33  \\
\hline

3.116 & 0.362 & 1.730 & 171 & 6.93 $\pm$ 3.10 $\pm$ 1.76  \\
\hline

3.123 & 0.364 & 1.727 & 279 & 7.84 $\pm$ 3.51 $\pm$ 2.31  \\
\hline

3.218 & 0.407 & 0.263 & 9 & 32.2 $\pm$ 8.05 $\pm$ 1.16  \\
\hline

3.224 & 0.406 & 0.263 & 27 & 44.0 $\pm$ 7.78 $\pm$ 3.43  \\
\hline

3.222 & 0.407 & 0.264 & 45 & 33.4 $\pm$ 6.43 $\pm$ 3.20  \\
\hline

3.222 & 0.407 & 0.264 & 63 & 32.2 $\pm$ 7.60 $\pm$ 6.66  \\
\hline

3.225 & 0.407 & 0.263 & 81 & 40.5 $\pm$ 11.2 $\pm$ 5.81  \\
\hline

3.215 & 0.407 & 0.264 & 99 & 46.6 $\pm$ 13.4 $\pm$ 0.47  \\
\hline

3.213 & 0.406 & 0.262 & 261 & 52.8 $\pm$ 16.7 $\pm$ 2.21  \\
\hline

3.217 & 0.407 & 0.264 & 279 & 37.3 $\pm$ 9.06 $\pm$ 10.1  \\
\hline

3.220 & 0.406 & 0.262 & 297 & 35.0 $\pm$ 7.01 $\pm$ 3.67  \\
\hline

3.221 & 0.407 & 0.263 & 315 & 13.3 $\pm$ 4.42 $\pm$ 3.43  \\
\hline

3.215 & 0.406 & 0.263 & 333 & 39.5 $\pm$ 8.83 $\pm$ 15.2  \\
\hline

3.216 & 0.406 & 0.263 & 351 & 27.3 $\pm$ 7.30 $\pm$ 1.75  \\
\hline

3.224 & 0.427 & 0.351 & 9 & 41.1 $\pm$ 7.15 $\pm$ 3.12  \\
\hline

3.222 & 0.427 & 0.352 & 27 & 36.5 $\pm$ 5.63 $\pm$ 3.29  \\
\hline

3.228 & 0.427 & 0.352 & 45 & 45.3 $\pm$ 6.01 $\pm$ 4.99  \\
\hline

3.226 & 0.427 & 0.351 & 63 & 37.9 $\pm$ 5.72 $\pm$ 3.58  \\
\hline

3.228 & 0.428 & 0.352 & 81 & 39.2 $\pm$ 5.84 $\pm$ 0.43  \\
\hline

3.229 & 0.427 & 0.351 & 99 & 38.3 $\pm$ 6.05 $\pm$ 1.67  \\
\hline

3.226 & 0.428 & 0.350 & 117 & 41.2 $\pm$ 9.22 $\pm$ 4.24  \\
\hline

3.230 & 0.429 & 0.352 & 135 & 46.5 $\pm$ 16.4 $\pm$ 1.34  \\
\hline

3.224 & 0.428 & 0.352 & 153 & 58.6 $\pm$ 26.2 $\pm$ 10.4  \\
\hline

3.227 & 0.428 & 0.352 & 225 & 57.8 $\pm$ 19.3 $\pm$ 12.6  \\
\hline

3.223 & 0.428 & 0.351 & 243 & 51.5 $\pm$ 10.1 $\pm$ 6.63  \\
\hline

3.224 & 0.428 & 0.351 & 261 & 50.6 $\pm$ 8.44 $\pm$ 0.74  \\
\hline

3.223 & 0.428 & 0.352 & 279 & 45.3 $\pm$ 5.80 $\pm$ 2.81  \\
\hline

3.223 & 0.427 & 0.351 & 297 & 26.7 $\pm$ 4.03 $\pm$ 2.87  \\
\hline

3.229 & 0.427 & 0.352 & 315 & 22.4 $\pm$ 4.68 $\pm$ 2.21  \\
\hline

3.224 & 0.428 & 0.350 & 333 & 40.0 $\pm$ 6.96 $\pm$ 3.57  \\
\hline

3.226 & 0.428 & 0.352 & 351 & 28.2 $\pm$ 6.02 $\pm$ 6.54  \\
\hline

3.222 & 0.430 & 0.498 & 9 & 30.1 $\pm$ 4.70 $\pm$ 2.88  \\
\hline

3.228 & 0.430 & 0.499 & 27 & 27.0 $\pm$ 4.12 $\pm$ 4.60  \\
\hline

3.229 & 0.430 & 0.498 & 45 & 36.6 $\pm$ 5.58 $\pm$ 4.69  \\
\hline

3.226 & 0.430 & 0.498 & 63 & 37.9 $\pm$ 5.26 $\pm$ 2.02  \\
\hline

3.229 & 0.430 & 0.498 & 81 & 46.3 $\pm$ 4.57 $\pm$ 5.85  \\
\hline

3.227 & 0.430 & 0.499 & 99 & 37.6 $\pm$ 4.20 $\pm$ 1.95  \\
\hline

3.229 & 0.430 & 0.500 & 117 & 38.7 $\pm$ 7.18 $\pm$ 3.66  \\
\hline

3.230 & 0.430 & 0.498 & 135 & 39.0 $\pm$ 10.4 $\pm$ 0.94  \\
\hline

3.226 & 0.431 & 0.497 & 153 & 25.2 $\pm$ 10.3 $\pm$ 5.72  \\
\hline

3.229 & 0.432 & 0.496 & 189 & 73.2 $\pm$ 25.9 $\pm$ 4.82  \\
\hline

3.227 & 0.431 & 0.497 & 225 & 26.3 $\pm$ 9.29 $\pm$ 8.19  \\
\hline

3.232 & 0.430 & 0.497 & 243 & 28.3 $\pm$ 5.17 $\pm$ 1.68  \\
\hline

3.228 & 0.430 & 0.497 & 261 & 29.9 $\pm$ 4.32 $\pm$ 1.69  \\
\hline

3.227 & 0.430 & 0.498 & 279 & 31.0 $\pm$ 3.65 $\pm$ 2.82  \\
\hline

3.225 & 0.430 & 0.498 & 297 & 33.7 $\pm$ 4.22 $\pm$ 3.50  \\
\hline

3.230 & 0.430 & 0.498 & 315 & 33.1 $\pm$ 5.24 $\pm$ 6.45  \\
\hline

3.227 & 0.430 & 0.497 & 333 & 34.8 $\pm$ 5.31 $\pm$ 2.83  \\
\hline

3.223 & 0.431 & 0.498 & 351 & 31.5 $\pm$ 5.33 $\pm$ 2.32  \\
\hline

3.226 & 0.431 & 0.785 & 9 & 17.8 $\pm$ 2.68 $\pm$ 0.52  \\
\hline

3.228 & 0.432 & 0.787 & 27 & 22.0 $\pm$ 2.32 $\pm$ 1.03  \\
\hline

3.228 & 0.431 & 0.790 & 45 & 21.9 $\pm$ 3.04 $\pm$ 1.90  \\
\hline

3.229 & 0.431 & 0.791 & 63 & 32.3 $\pm$ 5.99 $\pm$ 2.20  \\
\hline

3.229 & 0.431 & 0.791 & 81 & 31.2 $\pm$ 3.41 $\pm$ 0.54  \\
\hline

3.228 & 0.431 & 0.791 & 99 & 29.5 $\pm$ 3.58 $\pm$ 2.65  \\
\hline

3.228 & 0.432 & 0.789 & 117 & 28.7 $\pm$ 6.58 $\pm$ 2.15  \\
\hline

3.229 & 0.431 & 0.787 & 135 & 37.7 $\pm$ 7.12 $\pm$ 6.67  \\
\hline

3.230 & 0.432 & 0.782 & 153 & 11.0 $\pm$ 4.47 $\pm$ 4.18  \\
\hline

3.227 & 0.431 & 0.781 & 189 & 15.9 $\pm$ 5.62 $\pm$ 7.86  \\
\hline

3.227 & 0.432 & 0.786 & 225 & 17.7 $\pm$ 3.54 $\pm$ 2.12  \\
\hline

3.230 & 0.431 & 0.790 & 243 & 23.3 $\pm$ 4.05 $\pm$ 2.16  \\
\hline

3.224 & 0.432 & 0.791 & 261 & 23.0 $\pm$ 3.64 $\pm$ 2.84  \\
\hline

3.227 & 0.432 & 0.791 & 279 & 29.1 $\pm$ 3.48 $\pm$ 3.19  \\
\hline

3.228 & 0.431 & 0.791 & 297 & 29.1 $\pm$ 5.15 $\pm$ 3.60  \\
\hline

3.228 & 0.431 & 0.788 & 315 & 18.8 $\pm$ 2.72 $\pm$ 4.05  \\
\hline

3.227 & 0.431 & 0.788 & 333 & 21.4 $\pm$ 2.64 $\pm$ 3.34  \\
\hline

3.222 & 0.432 & 0.787 & 351 & 24.5 $\pm$ 3.36 $\pm$ 1.98  \\
\hline

3.226 & 0.432 & 1.228 & 27 & 10.3 $\pm$ 1.82 $\pm$ 0.47  \\
\hline

3.225 & 0.433 & 1.223 & 45 & 12.6 $\pm$ 3.64 $\pm$ 0.69  \\
\hline

3.224 & 0.433 & 1.226 & 63 & 14.4 $\pm$ 3.07 $\pm$ 1.70  \\
\hline

3.226 & 0.433 & 1.226 & 81 & 21.2 $\pm$ 2.72 $\pm$ 2.90  \\
\hline

3.224 & 0.433 & 1.227 & 99 & 17.8 $\pm$ 2.89 $\pm$ 1.57  \\
\hline

3.224 & 0.433 & 1.229 & 117 & 13.7 $\pm$ 3.14 $\pm$ 1.75  \\
\hline

3.227 & 0.433 & 1.226 & 135 & 14.8 $\pm$ 2.84 $\pm$ 2.78  \\
\hline

3.231 & 0.432 & 1.228 & 153 & 16.2 $\pm$ 3.73 $\pm$ 0.67  \\
\hline

3.230 & 0.432 & 1.226 & 171 & 5.46 $\pm$ 2.23 $\pm$ 1.75  \\
\hline

3.230 & 0.432 & 1.226 & 189 & 2.87 $\pm$ 1.17 $\pm$ 0.88  \\
\hline

3.227 & 0.432 & 1.228 & 207 & 9.30 $\pm$ 2.48 $\pm$ 1.52  \\
\hline

3.226 & 0.433 & 1.223 & 225 & 15.8 $\pm$ 2.23 $\pm$ 2.24  \\
\hline

3.225 & 0.433 & 1.225 & 243 & 16.2 $\pm$ 3.18 $\pm$ 2.28  \\
\hline

3.224 & 0.433 & 1.227 & 261 & 12.3 $\pm$ 3.18 $\pm$ 0.47  \\
\hline

3.228 & 0.433 & 1.229 & 279 & 14.9 $\pm$ 2.56 $\pm$ 0.88  \\
\hline

3.225 & 0.434 & 1.226 & 297 & 15.4 $\pm$ 2.86 $\pm$ 0.78  \\
\hline

3.226 & 0.433 & 1.226 & 315 & 9.14 $\pm$ 2.89 $\pm$ 0.78  \\
\hline

3.226 & 0.432 & 1.225 & 333 & 11.0 $\pm$ 2.20 $\pm$ 3.17  \\
\hline

3.225 & 0.434 & 1.728 & 45 & 12.2 $\pm$ 2.50 $\pm$ 2.80  \\
\hline

3.227 & 0.434 & 1.730 & 63 & 12.4 $\pm$ 1.85 $\pm$ 0.70  \\
\hline

3.227 & 0.434 & 1.726 & 81 & 6.70 $\pm$ 1.46 $\pm$ 0.45  \\
\hline

3.223 & 0.434 & 1.730 & 99 & 9.08 $\pm$ 1.45 $\pm$ 0.73  \\
\hline

3.225 & 0.434 & 1.728 & 117 & 4.77 $\pm$ 1.27 $\pm$ 0.92  \\
\hline

3.226 & 0.434 & 1.728 & 135 & 6.85 $\pm$ 1.90 $\pm$ 1.20  \\
\hline

3.224 & 0.432 & 1.729 & 153 & 6.78 $\pm$ 2.40 $\pm$ 1.10  \\
\hline

3.231 & 0.432 & 1.730 & 171 & 13.4 $\pm$ 4.22 $\pm$ 4.72  \\
\hline

3.228 & 0.432 & 1.734 & 207 & 10.2 $\pm$ 2.83 $\pm$ 4.17  \\
\hline

3.228 & 0.434 & 1.731 & 225 & 10.9 $\pm$ 2.06 $\pm$ 1.53  \\
\hline

3.225 & 0.434 & 1.728 & 243 & 7.49 $\pm$ 2.08 $\pm$ 0.83  \\
\hline

3.224 & 0.434 & 1.727 & 261 & 7.87 $\pm$ 1.86 $\pm$ 1.14  \\
\hline

3.225 & 0.434 & 1.725 & 279 & 10.3 $\pm$ 1.98 $\pm$ 0.29  \\
\hline

3.227 & 0.434 & 1.721 & 297 & 9.77 $\pm$ 1.44 $\pm$ 0.82  \\
\hline

3.224 & 0.433 & 1.726 & 315 & 12.4 $\pm$ 2.71 $\pm$ 2.44  \\
\hline

3.286 & 0.496 & 0.500 & 9 & 69.3 $\pm$ 13.3 $\pm$ 9.36  \\
\hline

3.283 & 0.495 & 0.500 & 27 & 65.0 $\pm$ 11.9 $\pm$ 4.99  \\
\hline

3.287 & 0.496 & 0.502 & 45 & 45.9 $\pm$ 10.3 $\pm$ 1.72  \\
\hline

3.288 & 0.496 & 0.501 & 63 & 97.9 $\pm$ 24.5 $\pm$ 1.00  \\
\hline

3.282 & 0.496 & 0.504 & 99 & 77.4 $\pm$ 34.6 $\pm$ 10.4  \\
\hline

3.283 & 0.496 & 0.503 & 261 & 87.7 $\pm$ 39.2 $\pm$ 18.1  \\
\hline

3.286 & 0.495 & 0.497 & 297 & 34.8 $\pm$ 10.5 $\pm$ 1.86  \\
\hline

3.288 & 0.496 & 0.499 & 315 & 52.5 $\pm$ 12.7 $\pm$ 4.25  \\
\hline

3.284 & 0.496 & 0.501 & 333 & 87.5 $\pm$ 18.3 $\pm$ 24.1  \\
\hline

3.288 & 0.497 & 0.503 & 351 & 62.0 $\pm$ 14.6 $\pm$ 11.3  \\
\hline

3.289 & 0.496 & 0.790 & 9 & 23.5 $\pm$ 5.71 $\pm$ 5.04  \\
\hline

3.288 & 0.497 & 0.790 & 27 & 43.4 $\pm$ 9.71 $\pm$ 5.30  \\
\hline

3.289 & 0.496 & 0.793 & 45 & 68.8 $\pm$ 20.8 $\pm$ 9.68  \\
\hline

3.287 & 0.497 & 0.797 & 63 & 45.6 $\pm$ 10.2 $\pm$ 7.71  \\
\hline

3.291 & 0.497 & 0.797 & 81 & 79.0 $\pm$ 23.8 $\pm$ 13.3  \\
\hline

3.288 & 0.496 & 0.795 & 117 & 40.0 $\pm$ 14.2 $\pm$ 6.53  \\
\hline

3.288 & 0.496 & 0.794 & 243 & 18.2 $\pm$ 8.12 $\pm$ 4.08  \\
\hline

3.288 & 0.496 & 0.791 & 261 & 68.1 $\pm$ 25.7 $\pm$ 12.6  \\
\hline

3.289 & 0.496 & 0.790 & 279 & 36.9 $\pm$ 12.3 $\pm$ 10.3  \\
\hline

3.289 & 0.496 & 0.791 & 297 & 33.3 $\pm$ 8.07 $\pm$ 6.73  \\
\hline

3.284 & 0.496 & 0.793 & 315 & 76.1 $\pm$ 21.1 $\pm$ 22.2  \\
\hline

3.290 & 0.496 & 0.789 & 333 & 31.1 $\pm$ 9.84 $\pm$ 2.65  \\
\hline

3.285 & 0.496 & 0.788 & 351 & 44.2 $\pm$ 9.21 $\pm$ 3.89  \\
\hline

3.290 & 0.497 & 1.229 & 9 & 12.4 $\pm$ 4.68 $\pm$ 1.05  \\
\hline

3.285 & 0.496 & 1.234 & 27 & 15.4 $\pm$ 5.82 $\pm$ 4.23  \\
\hline

3.288 & 0.496 & 1.233 & 63 & 27.5 $\pm$ 8.31 $\pm$ 0.80  \\
\hline

3.288 & 0.497 & 1.234 & 81 & 36.0 $\pm$ 12.0 $\pm$ 4.48  \\
\hline

3.287 & 0.497 & 1.238 & 99 & 18.1 $\pm$ 5.72 $\pm$ 2.56  \\
\hline

3.287 & 0.496 & 1.233 & 117 & 36.7 $\pm$ 11.1 $\pm$ 15.5  \\
\hline

3.291 & 0.497 & 1.226 & 135 & 39.2 $\pm$ 14.8 $\pm$ 4.38  \\
\hline

3.284 & 0.497 & 1.230 & 225 & 20.3 $\pm$ 7.19 $\pm$ 2.30  \\
\hline

3.287 & 0.497 & 1.233 & 243 & 30.5 $\pm$ 7.19 $\pm$ 7.35  \\
\hline

3.285 & 0.496 & 1.235 & 297 & 32.6 $\pm$ 9.42 $\pm$ 1.60  \\
\hline

3.287 & 0.496 & 1.233 & 351 & 18.8 $\pm$ 7.10 $\pm$ 0.28  \\
\hline

3.292 & 0.497 & 1.728 & 63 & 14.2 $\pm$ 5.02 $\pm$ 1.04  \\
\hline

3.283 & 0.496 & 1.729 & 81 & 25.2 $\pm$ 5.94 $\pm$ 2.46  \\
\hline

3.292 & 0.497 & 1.736 & 99 & 17.4 $\pm$ 4.35 $\pm$ 1.23  \\
\hline

3.288 & 0.496 & 1.737 & 117 & 17.0 $\pm$ 5.37 $\pm$ 0.70  \\
\hline

3.296 & 0.497 & 1.732 & 243 & 18.1 $\pm$ 5.73 $\pm$ 3.44  \\
\hline

3.285 & 0.496 & 1.739 & 261 & 12.7 $\pm$ 5.19 $\pm$ 0.69  \\
\hline

3.287 & 0.496 & 1.728 & 279 & 18.3 $\pm$ 5.29 $\pm$ 3.35  \\
\hline

3.291 & 0.497 & 1.723 & 297 & 15.3 $\pm$ 4.85 $\pm$ 1.25  \\
\hline

3.292 & 0.497 & 1.737 & 315 & 13.1 $\pm$ 5.37 $\pm$ 1.32  \\
\hline

3.599 & 0.425 & 0.277 & 27 & 67.1 $\pm$ 30.1 $\pm$ 5.41  \\
\hline

3.591 & 0.424 & 0.275 & 297 & 116. $\pm$ 51.8 $\pm$ 8.35  \\
\hline

3.582 & 0.423 & 0.274 & 351 & 107. $\pm$ 47.8 $\pm$ 10.6  \\
\hline

3.666 & 0.448 & 0.353 & 9 & 27.6 $\pm$ 7.37 $\pm$ 3.94  \\
\hline

3.668 & 0.448 & 0.356 & 27 & 24.6 $\pm$ 7.09 $\pm$ 9.26  \\
\hline

3.663 & 0.448 & 0.353 & 45 & 44.5 $\pm$ 10.2 $\pm$ 1.26  \\
\hline

3.672 & 0.448 & 0.355 & 63 & 24.8 $\pm$ 9.39 $\pm$ 1.17  \\
\hline

3.665 & 0.448 & 0.354 & 81 & 69.5 $\pm$ 19.3 $\pm$ 17.1  \\
\hline

3.667 & 0.448 & 0.354 & 99 & 32.8 $\pm$ 14.7 $\pm$ 3.24  \\
\hline

3.667 & 0.448 & 0.355 & 261 & 46.5 $\pm$ 19.0 $\pm$ 4.83  \\
\hline

3.669 & 0.447 & 0.353 & 279 & 42.5 $\pm$ 11.4 $\pm$ 6.62  \\
\hline

3.676 & 0.448 & 0.355 & 297 & 31.6 $\pm$ 7.66 $\pm$ 4.59  \\
\hline

3.667 & 0.447 & 0.353 & 315 & 18.5 $\pm$ 6.19 $\pm$ 3.58  \\
\hline

3.660 & 0.447 & 0.354 & 351 & 20.8 $\pm$ 6.94 $\pm$ 3.29  \\
\hline

3.674 & 0.450 & 0.498 & 9 & 15.7 $\pm$ 5.55 $\pm$ 2.64  \\
\hline

3.673 & 0.450 & 0.497 & 27 & 24.3 $\pm$ 5.31 $\pm$ 1.26  \\
\hline

3.674 & 0.450 & 0.497 & 45 & 30.9 $\pm$ 5.55 $\pm$ 5.30  \\
\hline

3.681 & 0.451 & 0.498 & 63 & 27.2 $\pm$ 4.66 $\pm$ 0.29  \\
\hline

3.676 & 0.450 & 0.498 & 81 & 32.5 $\pm$ 5.13 $\pm$ 1.42  \\
\hline

3.674 & 0.450 & 0.497 & 99 & 34.4 $\pm$ 6.00 $\pm$ 2.37  \\
\hline

3.673 & 0.452 & 0.500 & 117 & 30.0 $\pm$ 8.67 $\pm$ 1.72  \\
\hline

3.676 & 0.450 & 0.499 & 243 & 34.9 $\pm$ 8.48 $\pm$ 5.87  \\
\hline

3.674 & 0.450 & 0.500 & 261 & 29.5 $\pm$ 6.16 $\pm$ 2.73  \\
\hline

3.678 & 0.451 & 0.496 & 279 & 38.3 $\pm$ 5.59 $\pm$ 4.17  \\
\hline

3.677 & 0.450 & 0.497 & 297 & 22.3 $\pm$ 3.57 $\pm$ 2.29  \\
\hline

3.671 & 0.449 & 0.499 & 315 & 28.7 $\pm$ 5.08 $\pm$ 2.20  \\
\hline

3.674 & 0.450 & 0.497 & 333 & 33.0 $\pm$ 8.00 $\pm$ 3.46  \\
\hline

3.677 & 0.451 & 0.498 & 351 & 22.5 $\pm$ 6.77 $\pm$ 5.70  \\
\hline

3.674 & 0.450 & 0.790 & 45 & 16.7 $\pm$ 6.33 $\pm$ 3.85  \\
\hline

3.675 & 0.451 & 0.789 & 63 & 18.8 $\pm$ 3.13 $\pm$ 2.91  \\
\hline

3.676 & 0.451 & 0.790 & 81 & 21.9 $\pm$ 2.93 $\pm$ 1.24  \\
\hline

3.675 & 0.451 & 0.793 & 99 & 31.3 $\pm$ 4.42 $\pm$ 1.71  \\
\hline

3.677 & 0.452 & 0.788 & 117 & 42.5 $\pm$ 10.6 $\pm$ 2.35  \\
\hline

3.675 & 0.451 & 0.789 & 243 & 21.7 $\pm$ 6.87 $\pm$ 3.21  \\
\hline

3.677 & 0.451 & 0.793 & 261 & 15.6 $\pm$ 3.32 $\pm$ 2.21  \\
\hline

3.676 & 0.451 & 0.786 & 279 & 24.1 $\pm$ 3.14 $\pm$ 1.98  \\
\hline

3.679 & 0.451 & 0.792 & 297 & 23.4 $\pm$ 3.13 $\pm$ 0.86  \\
\hline

3.676 & 0.451 & 0.789 & 315 & 22.8 $\pm$ 6.88 $\pm$ 1.05  \\
\hline

3.674 & 0.451 & 1.228 & 45 & 12.4 $\pm$ 4.69 $\pm$ 2.78  \\
\hline

3.677 & 0.452 & 1.230 & 63 & 10.9 $\pm$ 1.99 $\pm$ 0.90  \\
\hline

3.676 & 0.452 & 1.228 & 81 & 14.3 $\pm$ 2.54 $\pm$ 1.53  \\
\hline

3.672 & 0.451 & 1.228 & 99 & 9.93 $\pm$ 3.51 $\pm$ 1.18  \\
\hline

3.674 & 0.451 & 1.226 & 135 & 16.3 $\pm$ 6.64 $\pm$ 1.80  \\
\hline

3.678 & 0.451 & 1.226 & 225 & 10.5 $\pm$ 4.70 $\pm$ 1.60  \\
\hline

3.673 & 0.451 & 1.230 & 261 & 27.3 $\pm$ 7.29 $\pm$ 1.10  \\
\hline

3.676 & 0.451 & 1.229 & 279 & 12.0 $\pm$ 2.32 $\pm$ 0.44  \\
\hline

3.676 & 0.452 & 1.226 & 297 & 19.4 $\pm$ 2.52 $\pm$ 0.37  \\
\hline

3.677 & 0.451 & 1.230 & 315 & 9.35 $\pm$ 4.18 $\pm$ 1.34  \\
\hline

3.678 & 0.452 & 1.726 & 45 & 8.19 $\pm$ 1.79 $\pm$ 0.55  \\
\hline

3.672 & 0.451 & 1.739 & 63 & 5.93 $\pm$ 1.44 $\pm$ 0.86  \\
\hline

3.679 & 0.452 & 1.731 & 99 & 12.2 $\pm$ 4.30 $\pm$ 1.84  \\
\hline

3.675 & 0.452 & 1.731 & 117 & 11.7 $\pm$ 4.13 $\pm$ 0.34  \\
\hline

3.685 & 0.451 & 1.729 & 189 & 13.4 $\pm$ 5.99 $\pm$ 4.26  \\
\hline

3.680 & 0.453 & 1.730 & 225 & 6.85 $\pm$ 2.59 $\pm$ 1.58  \\
\hline

3.678 & 0.453 & 1.731 & 279 & 9.02 $\pm$ 3.19 $\pm$ 0.48  \\
\hline

3.681 & 0.452 & 1.722 & 297 & 9.62 $\pm$ 1.67 $\pm$ 1.13  \\
\hline

3.680 & 0.452 & 1.724 & 315 & 3.98 $\pm$ 1.20 $\pm$ 1.22  \\
\hline

3.672 & 0.451 & 1.732 & 333 & 6.91 $\pm$ 3.09 $\pm$ 1.43  \\
\hline

3.745 & 0.509 & 0.507 & 9 & 20.7 $\pm$ 3.91 $\pm$ 4.53  \\
\hline

3.743 & 0.510 & 0.508 & 27 & 36.3 $\pm$ 4.77 $\pm$ 1.12  \\
\hline

3.745 & 0.509 & 0.509 & 45 & 39.5 $\pm$ 5.53 $\pm$ 4.66  \\
\hline

3.741 & 0.509 & 0.510 & 63 & 36.8 $\pm$ 6.73 $\pm$ 2.53  \\
\hline

3.749 & 0.510 & 0.510 & 81 & 33.1 $\pm$ 8.84 $\pm$ 5.40  \\
\hline

3.745 & 0.509 & 0.508 & 99 & 28.3 $\pm$ 11.5 $\pm$ 0.84  \\
\hline

3.742 & 0.509 & 0.509 & 261 & 26.7 $\pm$ 12.0 $\pm$ 3.11  \\
\hline

3.749 & 0.509 & 0.507 & 279 & 39.0 $\pm$ 7.00 $\pm$ 0.53  \\
\hline

3.751 & 0.509 & 0.511 & 297 & 31.5 $\pm$ 5.11 $\pm$ 7.32  \\
\hline

3.749 & 0.509 & 0.508 & 315 & 44.4 $\pm$ 6.55 $\pm$ 0.45  \\
\hline

3.742 & 0.510 & 0.508 & 333 & 34.2 $\pm$ 5.78 $\pm$ 0.61  \\
\hline

3.741 & 0.510 & 0.510 & 351 & 36.3 $\pm$ 5.82 $\pm$ 3.66  \\
\hline

3.755 & 0.513 & 0.788 & 9 & 29.4 $\pm$ 5.05 $\pm$ 5.33  \\
\hline

3.753 & 0.512 & 0.790 & 27 & 26.9 $\pm$ 3.66 $\pm$ 2.19  \\
\hline

3.755 & 0.513 & 0.794 & 45 & 37.6 $\pm$ 3.79 $\pm$ 2.93  \\
\hline

3.755 & 0.513 & 0.793 & 63 & 37.7 $\pm$ 3.79 $\pm$ 3.04  \\
\hline

3.759 & 0.512 & 0.794 & 81 & 28.1 $\pm$ 4.90 $\pm$ 0.82  \\
\hline

3.755 & 0.513 & 0.794 & 99 & 30.0 $\pm$ 10.0 $\pm$ 6.26  \\
\hline

3.756 & 0.513 & 0.793 & 117 & 43.8 $\pm$ 17.9 $\pm$ 5.97  \\
\hline

3.756 & 0.513 & 0.791 & 243 & 29.1 $\pm$ 11.0 $\pm$ 6.19  \\
\hline

3.758 & 0.512 & 0.796 & 261 & 56.2 $\pm$ 14.5 $\pm$ 9.39  \\
\hline

3.757 & 0.514 & 0.794 & 279 & 30.0 $\pm$ 4.52 $\pm$ 1.90  \\
\hline

3.756 & 0.513 & 0.791 & 297 & 35.1 $\pm$ 3.04 $\pm$ 0.46  \\
\hline

3.757 & 0.513 & 0.793 & 315 & 32.6 $\pm$ 3.50 $\pm$ 1.45  \\
\hline

3.752 & 0.513 & 0.790 & 333 & 35.7 $\pm$ 5.05 $\pm$ 1.57  \\
\hline

3.756 & 0.513 & 0.789 & 351 & 38.4 $\pm$ 6.41 $\pm$ 4.64  \\
\hline

3.756 & 0.514 & 1.227 & 27 & 19.4 $\pm$ 6.15 $\pm$ 1.75  \\
\hline

3.755 & 0.514 & 1.231 & 45 & 22.6 $\pm$ 2.92 $\pm$ 1.10  \\
\hline

3.753 & 0.514 & 1.234 & 63 & 21.6 $\pm$ 2.70 $\pm$ 0.48  \\
\hline

3.753 & 0.514 & 1.234 & 81 & 24.0 $\pm$ 5.65 $\pm$ 3.39  \\
\hline

3.751 & 0.513 & 1.232 & 99 & 28.8 $\pm$ 8.00 $\pm$ 5.86  \\
\hline

3.756 & 0.513 & 1.235 & 117 & 22.5 $\pm$ 6.79 $\pm$ 6.57  \\
\hline

3.751 & 0.513 & 1.231 & 135 & 19.9 $\pm$ 8.13 $\pm$ 3.96  \\
\hline

3.750 & 0.513 & 1.228 & 225 & 22.3 $\pm$ 5.97 $\pm$ 1.49  \\
\hline

3.753 & 0.513 & 1.237 & 243 & 19.7 $\pm$ 4.52 $\pm$ 0.30  \\
\hline

3.756 & 0.514 & 1.236 & 261 & 24.8 $\pm$ 9.39 $\pm$ 3.84  \\
\hline

3.754 & 0.514 & 1.236 & 279 & 18.5 $\pm$ 4.62 $\pm$ 4.54  \\
\hline

3.752 & 0.514 & 1.235 & 297 & 22.0 $\pm$ 2.36 $\pm$ 2.99  \\
\hline

3.755 & 0.514 & 1.230 & 315 & 21.4 $\pm$ 2.94 $\pm$ 1.32  \\
\hline

3.754 & 0.513 & 1.232 & 333 & 16.7 $\pm$ 6.83 $\pm$ 2.28  \\
\hline

3.754 & 0.514 & 1.728 & 27 & 14.5 $\pm$ 2.78 $\pm$ 0.85  \\
\hline

3.756 & 0.514 & 1.729 & 45 & 11.0 $\pm$ 1.69 $\pm$ 0.86  \\
\hline

3.749 & 0.514 & 1.731 & 63 & 10.7 $\pm$ 2.40 $\pm$ 0.73  \\
\hline

3.751 & 0.514 & 1.736 & 81 & 17.5 $\pm$ 4.51 $\pm$ 1.80  \\
\hline

3.753 & 0.514 & 1.735 & 99 & 14.4 $\pm$ 3.86 $\pm$ 4.20  \\
\hline

3.753 & 0.514 & 1.734 & 117 & 10.2 $\pm$ 2.73 $\pm$ 1.25  \\
\hline

3.757 & 0.514 & 1.726 & 243 & 8.34 $\pm$ 2.64 $\pm$ 3.18  \\
\hline

3.750 & 0.514 & 1.731 & 261 & 15.6 $\pm$ 4.72 $\pm$ 2.59  \\
\hline

3.755 & 0.514 & 1.735 & 279 & 10.2 $\pm$ 3.60 $\pm$ 1.52  \\
\hline

3.754 & 0.514 & 1.732 & 297 & 10.0 $\pm$ 2.05 $\pm$ 1.04  \\
\hline

3.752 & 0.514 & 1.736 & 315 & 13.8 $\pm$ 1.91 $\pm$ 0.32  \\
\hline

3.754 & 0.513 & 1.730 & 333 & 3.74 $\pm$ 1.67 $\pm$ 2.02  \\
\hline

4.180 & 0.525 & 0.527 & 9 & 24.7 $\pm$ 7.12 $\pm$ 1.98  \\
\hline

4.188 & 0.526 & 0.527 & 27 & 21.5 $\pm$ 5.97 $\pm$ 2.29  \\
\hline

4.180 & 0.525 & 0.526 & 45 & 30.6 $\pm$ 7.91 $\pm$ 1.78  \\
\hline

4.185 & 0.525 & 0.527 & 63 & 60.9 $\pm$ 15.7 $\pm$ 10.8  \\
\hline

4.184 & 0.526 & 0.528 & 81 & 24.4 $\pm$ 10.9 $\pm$ 4.80  \\
\hline

4.180 & 0.527 & 0.529 & 279 & 51.1 $\pm$ 14.2 $\pm$ 7.30  \\
\hline

4.185 & 0.526 & 0.527 & 297 & 21.8 $\pm$ 6.57 $\pm$ 2.66  \\
\hline

4.179 & 0.525 & 0.528 & 315 & 11.3 $\pm$ 5.06 $\pm$ 1.36  \\
\hline

4.182 & 0.525 & 0.526 & 333 & 26.9 $\pm$ 8.11 $\pm$ 2.01  \\
\hline

4.180 & 0.526 & 0.528 & 351 & 11.5 $\pm$ 5.15 $\pm$ 1.66  \\
\hline

4.224 & 0.538 & 0.786 & 9 & 22.9 $\pm$ 3.45 $\pm$ 1.31  \\
\hline

4.221 & 0.537 & 0.787 & 27 & 17.4 $\pm$ 2.59 $\pm$ 0.18  \\
\hline

4.228 & 0.539 & 0.792 & 45 & 26.7 $\pm$ 3.48 $\pm$ 4.56  \\
\hline

4.227 & 0.538 & 0.792 & 63 & 29.3 $\pm$ 4.02 $\pm$ 2.42  \\
\hline

4.223 & 0.538 & 0.793 & 81 & 32.9 $\pm$ 5.64 $\pm$ 2.63  \\
\hline

4.230 & 0.539 & 0.796 & 99 & 29.3 $\pm$ 7.84 $\pm$ 2.46  \\
\hline

4.227 & 0.538 & 0.789 & 117 & 68.7 $\pm$ 28.0 $\pm$ 0.70  \\
\hline

4.227 & 0.538 & 0.793 & 261 & 24.6 $\pm$ 6.83 $\pm$ 1.02  \\
\hline

4.229 & 0.539 & 0.794 & 279 & 31.7 $\pm$ 4.62 $\pm$ 6.71  \\
\hline

4.225 & 0.538 & 0.793 & 297 & 25.6 $\pm$ 3.18 $\pm$ 0.82  \\
\hline

4.224 & 0.538 & 0.791 & 315 & 26.5 $\pm$ 3.48 $\pm$ 1.67  \\
\hline

4.227 & 0.538 & 0.788 & 333 & 22.2 $\pm$ 3.28 $\pm$ 2.30  \\
\hline

4.224 & 0.538 & 0.789 & 351 & 26.5 $\pm$ 3.79 $\pm$ 1.10  \\
\hline

4.232 & 0.540 & 1.233 & 9 & 19.1 $\pm$ 4.38 $\pm$ 3.91  \\
\hline

4.231 & 0.539 & 1.231 & 27 & 14.7 $\pm$ 2.49 $\pm$ 2.75  \\
\hline

4.230 & 0.539 & 1.232 & 45 & 15.5 $\pm$ 2.29 $\pm$ 1.76  \\
\hline

4.224 & 0.539 & 1.235 & 63 & 22.6 $\pm$ 2.94 $\pm$ 2.16  \\
\hline

4.228 & 0.539 & 1.232 & 81 & 21.1 $\pm$ 4.73 $\pm$ 0.47  \\
\hline

4.225 & 0.539 & 1.233 & 243 & 40.4 $\pm$ 18.1 $\pm$ 5.78  \\
\hline

4.223 & 0.539 & 1.233 & 279 & 29.1 $\pm$ 4.72 $\pm$ 0.91  \\
\hline

4.224 & 0.539 & 1.236 & 297 & 16.3 $\pm$ 2.16 $\pm$ 1.19  \\
\hline

4.222 & 0.539 & 1.232 & 315 & 16.3 $\pm$ 2.38 $\pm$ 2.41  \\
\hline

4.229 & 0.539 & 1.228 & 333 & 13.0 $\pm$ 2.65 $\pm$ 0.30  \\
\hline

4.225 & 0.539 & 1.234 & 351 & 9.98 $\pm$ 3.53 $\pm$ 1.12  \\
\hline

4.230 & 0.540 & 1.734 & 27 & 7.70 $\pm$ 1.92 $\pm$ 0.38  \\
\hline

4.226 & 0.539 & 1.737 & 45 & 8.82 $\pm$ 1.76 $\pm$ 0.95  \\
\hline

4.222 & 0.539 & 1.735 & 63 & 16.0 $\pm$ 2.70 $\pm$ 0.70  \\
\hline

4.228 & 0.539 & 1.733 & 279 & 9.68 $\pm$ 4.33 $\pm$ 0.57  \\
\hline

4.230 & 0.539 & 1.733 & 297 & 14.1 $\pm$ 2.39 $\pm$ 0.63  \\
\hline

4.221 & 0.538 & 1.734 & 315 & 12.3 $\pm$ 2.10 $\pm$ 0.35  \\
\hline

4.229 & 0.539 & 1.727 & 333 & 13.0 $\pm$ 2.84 $\pm$ 1.51  \\
\hline
\end{longtable}
\end{center}

